Harnessing Contrastive Learning and Neural Transformation for Time Series Anomaly Detection

Time series anomaly detection (TSAD) plays a vital role in many industrial applications. While contrastive learning has gained momentum in the time series domain for its prowess in extracting meaningful representations from unlabeled data, its straightforward application to anomaly detection is not without hurdles. Firstly, contrastive learning typically requires negative sampling to avoid the representation collapse issue, where the encoder converges to a constant solution. However, drawing from the same dataset for dissimilar samples is ill-suited for TSAD as most samples are ``normal'' in the training dataset. Secondly, conventional contrastive learning focuses on instance discrimination, which may overlook anomalies that are detectable when compared to their temporal context. In this study, we propose a novel approach, CNT, that incorporates a window-based contrastive learning strategy fortified with learnable transformations. This dual configuration focuses on capturing temporal anomalies in local regions while simultaneously mitigating the representation collapse issue. Our theoretical analysis validates the effectiveness of CNT in circumventing constant encoder solutions. Through extensive experiments on diverse real-world industrial datasets, we show the superiority of our framework by outperforming various baselines and model variants.

==> subtexes/abstract_v2.tex <==
Time series anomaly detection (TSAD) is vital for critical sectors such as industrial monitoring and cybersecurity, where accurate anomaly identification can have significant implications. Contrastive learning, despite its success in other domains, struggles with TSAD because of the context-dependent nature of anomalies, data-specific augmentation techniques, and the unsuitability of negative selection among normal instances. In this study, we propose CNT, an anomaly detection method that implements a temporal-wise contrasting framework fortified with learnable data augmentations by combining a contextual contrastive loss (CCL) with a discriminative contrastive loss (DCL) from NeuTralAD. Deviating from NeuTralAD's instance-level focus, CNT applies transformations within the latent space and performs contrastion between future and past windows, which sharpens the model's detection of temporal anomalies. Theoretical analysis confirms that CNT effectively prevents representation collapse without the need for negative samples by incorporating DCL into CCL. Empirical validation across various real-world industrial datasets shows that CNT consistently outperforms a variety of common benchmark models in terms of F1 scores. 

==> subtexes/abstract_v3.tex <==
Time series anomaly detection (TSAD) is vital for critical sectors such as industrial monitoring and cybersecurity, where accurate anomaly identification can have significant implications. Contrastive learning, despite its success in other domains, struggles with TSAD because of the context-dependent nature of anomalies, data-specific augmentation techniques, and the unsuitability of negative selection among normal instances. In this study, we propose CNT, an anomaly detection method that implements a temporal-wise contrasting framework fortified with learnable data augmentations by combining a contextual contrastive loss (CCL) with a discriminative contrastive loss (DCL) from NeuTralAD. Deviating from NeuTralAD's instance-level focus, CNT applies transformations within the latent space and performs contrastion between future and past windows, which sharpens the model's detection of temporal anomalies. Theoretical analysis confirms that CNT effectively prevents representation collapse without the need for negative samples by incorporating DCL into CCL. Empirical validation across various real-world industrial datasets shows that CNT consistently outperforms a variety of common benchmark models in terms of F1 scores. 

==> subtexes/abstract_v4.tex <==
Time series anomaly detection (TSAD) is crucial for IoT applications, where accurate anomaly identification can have significant implications for device reliability and data security. Contrastive learning, despite its success in other domains, struggles with TSAD because of the context-dependent nature of anomalies, data-specific augmentation techniques, and the unsuitability of negative selection among normal instances. In this work, we propose CNT, a simple and efficient anomaly detection framework that implements a temporal-wise contrasting framework fortified with learnable data augmentations. Specifically, CNT applies neural transformations to data instances, aligning these diverse but semantically related, transformed instances with their historical counterparts through contrastive learning. Thereby, anomalies can be identified based on inconsistencies highlighted between future projections and past observations. Furthermore, we prove through theoretical analysis that the combination of neural transformations with temporal-wise contrasting effectively circumvents the issue of representation collapse, eliminating the dependency on negative samples. Extensive experiments across five benchmark real-world industrial datasets showcase the effectiveness of CNT in TSAD in comparison to existing benchmarks.



% Specifically, CNT applies learnable transformations on data instances and aligns those diverse and semantic-related transformations with their past window through contrastive learning. Thereby, anomalies can be identified based on inconsistency between the future and the past. Additionally, theoretical analysis confirms that the combination of neural transformations and temporal-wise contrasting can effectively prevent representation collapse without the need for negative samples. Empirical validation across five benchmark real-world industrial datasets shows that CNT consistently outperforms various TSAD models in terms of F1 scores. 

% CNT aligns the future window of a time series with its past window through contrastive learning, thereby anomalies can be identified based on inconsistency highlighted by the temporal relationship. Additionally, we augment the temporal contrast with learnable neural transformations on data instances to avoid the need to define data-specific augmentations, this is backed up by our theoretical analysis. Empirical validation across various real-world industrial datasets shows that CNT consistently outperforms a variety of common benchmark models in terms of F1 scores. 

% Specifically, CNT applies learnable transformations within the latent space and performs contrastion between future and past windows, which sharpens the model's detection of temporal anomalies. Theoretical analysis confirms that CNT effectively prevents representation collapse without the need for negative samples by incorporating DCL into CCL. Empirical validation across various real-world industrial datasets shows that CNT consistently outperforms a variety of common benchmark models in terms of F1 scores. 

==> subtexes/ethecal.tex <==
\section{Ethics}
As authors of this submission on time series anomaly detection, we recognize the potential impact of our work on individuals and society, and we are committed to conducting our research in an ethical and responsible manner. We acknowledge the potential benefits and risks associated with the use of our methods in areas such as finance, healthcare, and security, and we are committed to engaging in ongoing dialogue with stakeholders to ensure that our methods are used ethically and responsibly.

We believe that transparency and accountability are key components of ethical research. We are committed to providing clear and transparent descriptions of our methods and results, and to engaging with stakeholders to receive feedback and address concerns. Additionally, we are committed to staying up-to-date with the latest ethical developments in our field and to incorporating ethical considerations into all aspects of our work.

% By conducting our research in an ethical manner, we believe that we can contribute to a more just and equitable society.

==> subtexes/experiments.tex <==
%\section{Experiment}
\subsection{Datasets}

In this work,  real-world benchmark datasets are used for the evaluation of time series anomaly detection methods: SWaT~\cite{mathur2016swat}. WADI~\cite{ahmed2017wadi}, HAI~\cite{hai21.03}, and MSL~\cite{lstm-ndt}. The SWaT dataset is collected from a scaled-down, secure water treatment testbed, featuring a 51-dimensional multivariate time series from 11 days of continuous operation. The first 7 days reflect normal operations and the last 4 days contain cyber attack data. Similarly, the WADI dataset, collected from a small-scale water distribution network, includes 123 sensor and actuator time series from a 16-day run, with normal operations in the first 14 days and cyber attacks in the last 2. Similar to~\cite{gdn}, both these datasets have been down-sampled to 10-second intervals using median values. Additionally, SWaT and WADI are released by iTrust Center~\footnote{\url{https://itrust.sutd.edu.sg/itrust-labs_datasets/dataset_info/}} to support research in cybersecurity. MSL, published by NASA, contains telemetry anomaly data from Mars Science Laboratory rover. The data includes telemetry values and one-hot commands. Lastly, the HAI dataset derives from an Industrial Control System testbed enriched with a Hardware-In-the-Loop simulator, featuring processes like boiler, turbine, water treatment, and steam-turbine power generation. 
The statistics of data are summarized in Table~\ref{tab:data_statistics}:
\begin{table}[H]
\small
    \setlength{\abovecaptionskip}{0cm}
    %\setlength{\belowcaptionskip}{-0.1cm}
    \centering
    \caption{Summary statistics for datasets used in experiments} 
    \begin{tabular}{ccccc}\\ \toprule
               \textbf{Dataset} & \textbf{\# Channels} & \textbf{\# training} & \textbf{\# test} & \textbf{\% anomalies} \\ \midrule
   SWaT  &  51         &  47440   & 44993 & 12.13       \\
   WADI       &  123         &  78458    & 17281 & 5.77     \\  
         SMAP       &   25        & 135183 & 427617 & 12.79     \\  

      MSL       &   55        & 58317 & 73729 & 10.53     \\
    SMD       & 38         &  25300   & 25300 & 4.21    \\  

   HAI       & 79         &  92163   & 27003 & 1.93    \\  
    TODS  & 1   & 33333 & 16667 & 2.74 \\
   \bottomrule
    \end{tabular}
    \label{tab:data_statistics}
    %\vspace{-0.8cm}
\end{table}

% \subsection{Model Configurations}
% Our model is trained with an Adam optimizer~\cite{kingma2014adam} at a learning rate of 0.001 for 50 epochs. $20\%$ of the training set is selected as a validation set where the best epoch is stored based on the validation loss. The hidden dimension $d$ is set to 32, and the number of TCN layers is set to 8. The temperature $\tau$ and the number of transformations for DCL loss are set to 0.1 and 6, respectively. The suspect window size $w$ is set to 5, and the sequence length is 50 for WADI, HAI, SMAP, and 30 for MSL, SWaT, SMD respectively. 


\subsection{Experimental Setup and Evaluation Metric}
Our model is trained with an Adam optimizer~\cite{kingma2014adam} at a learning rate of 0.001 for 30 epochs. $20\%$ of the training set is selected as a validation set where the best epoch is stored based on the validation loss. We employ early stopping with a patience of 10. The hidden dimension $d$ is set to 32, and the number of TCN blocks is set to 8. The temperature $\tau$ and the number of transformations for DCL loss are set to 0.1 and 6, respectively. The suspect window size $w$ is set to 5, and the sequence length is set to 30 for all datasets.  
%The sequence length $l$ is 30 for SWaT and MSL, and 50 for WADI, HAI, SMAP respectively. 

%\subsection{Evaluation Metrics}
F1-score is used as a performance metric to evaluate the performance of anomaly detection. The threshold for each model is chosen as the one which achieves the best F1 over the test sets. In addition, we follow the point-adjusting strategy suggested in \cite{omnianomaly}, which labels a whole anomaly segment as 1 as long as one of the points within the segment is detected as an anomaly. Since our primary contribution is not the development of a new thresholding method, we adopt this well-established practice to eliminate potential bias arising from selecting a specific thresholding method. This choice of reporting F1 scores ensures a fair and consistent comparison across all methods.

\subsection{Baseline Methods}
We compare our framework with the most commonly used baseline methods selected from two categories: 1. General deep learning-based anomaly detection algorithms: Deep SVDD~\cite{deepSVDD}, and DAGMM~\cite{zong2018deep}. 2. Deep learning-based anomaly detection algorithms that are tailored to temporal sequences: LSTM-VAE~\cite{park2018multimodal}, MAD-GAN~\cite{mad-gan}, USAD~\cite{usad}, MSCRED~\cite{mscred}, MTAD-GAT~\cite{mtad-gat}, GDN~\cite{gdn}, and LNT~\cite{lnt}.


\begin{table*}[t]
%\small
    \setlength{\abovecaptionskip}{0cm}
    %\setlength{\belowcaptionskip}{-0.1cm}
    \centering
        % \caption{Performance comparison (F1-scores (\%)) on real-world datasets. The best performance is highlighted in bold.} 
        \caption{Performance comparison (F1 (\%)) on real-world datasets. The best performance is highlighted in bold.}
    %\begin{adjustbox}{width=\columnwidth,center}
    %\setlength{\tabcolsep}{1.65mm}{
    \begin{tabular}{ccccccc}\\ \toprule
    \textbf{Methods}  &  \textbf{SWaT} & \textbf{WADI} & \textbf{SMAP} & \textbf{MSL} & \textbf{HAI} & \textbf{SMD}  \\ \midrule
   DeepSVDD   & 82.87  & 67.33  & 69.67 & 85.01  & 44.25 & 86.30 \\
   DAGMM       &81.83  & 44.34  & 71.05  & 70.07  & 38.27 & 70.94\\
  % LSTM-ED     & 83.58  &     65.56 &  \\
   LSTM-VAE    & 84.95  & 67.52  & 72.74  & 90.58  & 67.07 & 78.42 \\ 
   MAD-GAN     & 86.53  & 70.51  & 88.14  & 91.38  & 28.70 & 47.85 \\ 
   USAD        & 84.60  & 57.25  & 86.34 & 92.72  & 69.41  & 94.63  \\ 
   %OMNI-Onomaly        & 85.28  & 41.02  & 84.34 & 89.89 & 82.33 &\\ 
   MSCRED       & 84.59  & 55.01 & 69.33   & 82.05    &  74.79 & 78.75  \\ 
   MTAD-GAT    & 85.50  & 67.94  & 90.13  & 90.84 & 78.91  & 92.72  \\ 
   GDN         & 89.57 & 71.54  &92.31  & 94.62  & 62.54 & 94.84  \\ 
   LNT         & 81.31& 32.63 & 82.65 & 91.82 &35.61 & 66.00 \\
   NCAD        & 91.06 &  75.95       &\textbf{94.50} &  \textbf{96.09}     & 82.36  & 81.53  \\ \midrule

   %LNT         & & & & &  \\\midrule
   Ours         & \textbf{92.01} & \textbf{82.04} & 92.27 & 90.51 & \textbf{85.73} & \textbf{95.33} \\
   \bottomrule
    \end{tabular}
    %}
    %\end{adjustbox}
    \label{tab:comparison_result}
    %\vspace{-0.8cm}
\end{table*}


\subsection{Comparison Study}

% Table~\ref{tab:comparison_result} presents the performance results of several models, with our model achieving the highest F1 scores for most datasets. Nonetheless, it is worth noting that our model's performance falls short on the MSL and SMAP datasets. This could be attributed to the fact that the majority of features (except the first dimension which contains telemetry value) in these datasets are one-hot encoding commands, with the majority of entries set to 0. Consequently, temporal encoding of sequences using simple TCN layers can be challenging, as these layers tend to mix all features through simple sum aggregation.  Conversely, graph-based models like GDN, which explicitly learn the relationship between features, have performed well on these datasets.

Table~\ref{tab:comparison_result} shows our model achieving the highest F1 scores for most datasets. However, our model's performance falls short on MSL and SMAP. This could be due to the majority of features in these datasets being one-hot encoded commands, making temporal encoding of sequences challenging for simple TCN layers that tend to mix all features through simple sum aggregation. On the other hand, graph-based models like GDN, which explicitly learn the relationship between features, have performed well on these datasets.

Additionally, NCAD currently holds state-of-the-arts performance on MSL and SMAP due to its semi-supervised classification training schemes based on synthetic anomalies. While supervised training is known to be more effective when the underlying distribution of synthetic anomalies is similar to that of the true anomalies in the dataset, we can see that NCAD performed relatively worse in WADI, HAI, and SMD compared to our methods, suggesting potential overfitting due to these datasets having a variety of different anomaly types beyond the injected ones.

% On the other hand, LNT, a model similar to ours, exhibited substantially lower performance compared to ours. The core idea of LNT is to pull the transformation of future predictions close to the context window while simultaneously pulling them away among themselves using same distance measures. However, the similarity between the context window and future instances may not be related in the same way as among the transformations of future predictions themselves. In contrast, our model leverages a Euclidean metric to pull together the suspect sequence and context sequence, while using cosine similarity to perform a contrasting operation between the suspect sequence and their transformations. 

ON the other hand, LNT, a similar model to ours, showed inferior performance compared to our model, possibly because it attempts to minimize the distance between the transformation of point-wise future predictions and the context window, which may not have identical semantic meanings. In contrast, our model employs a sequence-to-sequence comparison, where the suspect and context sequences share semantically meaningful features due to their overlap and shared feature encoder.
% our model follows the original approach of Neutral AD, which minimizes the distance between the transformation of the suspect sequence and the suspect sequence itself. This approach is more intuitive, as both the transformation and suspect sequence share the same input features.
% LNT tries to bring the transformation of future predictions closer to the context window while keeping them apart from each other using the same distance measure. However, the similarity between the context window and future instances may not be related in the same way as among the transformations of future predictions themselves. In contrast, our model uses Euclidean metric to bring together the suspect and context sequences and cosine similarity to contrast the suspect sequence with its transformations.

% This enables the model to learn salient features of normal instances from different angles.

% Table~\ref{tab:comparison_result} presents the performance results for all models. Notably, our model achieves the best F1 for the majority of datasets. However, we still under perform in MSL and SMAP datasets. We suspect there are two possible reasons. First, the majority of features in MSL and SMAP are one-hot encoding commands with the majority of entries set to 0, only the first dimension, which is the telemetry values, contains temporal information, which can make the temporal encoding of sequences harder if we use simple TCN layers that tend to mix all features through simple sum aggregation. In contrast, GDN and MTAD-GAT have achieved well performance on these datasets. The reason is that they explicitly learn the relationship between features, thus if the information is unrelated (it is possible as the majority of one-hot embeddings are empty), it can learn to decouple the main time series  from them, thus the temporal information within the main time series can be largely unaffected by other columns. On the other hand, NCAD has the current state-of-the-art results on MSL and SMAP, which can be attributed to its semi-supervised classification training schemes based on synthetic anomalies. If the underlying distribution of the anomalies is very similar to that of the true anomalies for datasets, it is known that super-vised training will be much more powerful than unsupervised or semi-supervised training as it helps to create a discriminative boundary between normal and abnormal instances. However, we can also see that NCAE performs relatively worse in WADI, HAI and SMD compared to our methods, indicating that these datasets may have many different types of anomalies than the injected one, leading to the overfitting problem. Additionally, LNT is another model similar to our solution, but its performance is significantly lower compared to us. we suspect the reason might be that LNT is trained in a way that the transformation of future predictions is similar to its context window as well as makes them self apart from each other through the same distance function, which may be added too many regularizations since the similarity between context window and future instances are not actually related in the same way the transformations to themselves.

% Table~\ref{tab:comparison_result} presents the performance results for all models. Notebly, our model achieves the best F1 for the majority of datasets (except MSL and SMAP). NCAD has the current state-of-the-arts results on MSL and SMAP, which can be attributed to its semi-supervised classification training schemes based on synthetic anomalies. However, NCAD still underperforms in other datasets , in particular, WADI, HAI, and SMD compared to our model, one possible reason is that the synthetic anomalies cannot cover all kinds of types of anomalies, and it may lead to underperformed performance if the underlying distribution of abnormal instances is sustantially different from the injected anomalies. Another reason that we are underperformed for MSL and SMAP might be due to the data itself. For instance, he majority of features in MSL and SMAP are one-hot encodding commands, which can make the encoding of sequences harder if we use a simple TCN layers which tends to mix all features through simple aggregation. In contrast, GDN has achieved well performance on this datasets, which deals with the inter-series relationship through graph neural network, thus the information between each feature dimension can be nicely decoupled and aggregated in a data-driven way.  LNT is another model similar to our solution, but its performance is significantly lower compared to us. we suspect the reason might be that LNT is trained in a way that the transformation of future predictions is similar to its context window as well as makes them self apart from each other through the same distance function, which may be add too much regularizations since the similarity between context window and future instances are not actually related in the same way the the transformations to themselves.


% In general, models that utilize a specialized neural network, such as LSTM and TCN, as a base encoder for encoding temporal data outperform models that neglect the temporal dependencies within the data, such as DeepSVDD and DAGMM. Notably, our 

% Notably, NCAD achieves well performance among the majority of datasets, which can be attributed to the reason that the model include synthetic anomalies. 

% Notably, GDN achieves well performance on the majority of datasets, which can be attributed to the design of its base encoder for capturing the inter-series relationships among time series. Specifically, GDN employs graph neural networks to learn inter-series relationships, whereas our base model uses the TCN and models inter-series relationships through a fully connected neural network. Despite the relative simplicity of our base model, it outperforms all baseline methods on four datasets and performs reasonably well on MSL. This is likely due to the fact that most existing methods rely on either reconstruction-based or forecasting-based errors to identify anomalies. In contrast, our model leverages two contrastive losses, which are more suitable for learning the differences in latent representations between adjacent sequences, rather than capturing low-level details within the original time series data  through the process of time series forecasting or reconstruction.

% \begin{table*}[t]
% %\small
%     \setlength{\abovecaptionskip}{0cm}
%     %\setlength{\belowcaptionskip}{-0.1cm}
%     \centering
%         % \caption{Performance comparison (F1-scores (\%)) on real-world datasets. The best performance is highlighted in bold.} 
%         \caption{Performance comparison (F1 (\%)) on real-world datasets. The best performance is highlighted in bold. The results of baseline models are partially from~\protect\cite{su2019robust},~\protect\cite{audibert2020usad} and~\protect\cite{zhao2020multivariate}.}
%     %\begin{adjustbox}{width=\columnwidth,center}
%     %\setlength{\tabcolsep}{1.65mm}{
%     \begin{tabular}{cccccccc}\\ \toprule
%     \textbf{Methods}  &  \textbf{SWaT} & \textbf{WADI} & \textbf{SMAP} & \textbf{MSL} & \textbf{HAI\_1} & \textbf{HAI\_2} & \textbf{HAI\_3}   \\ \midrule
%    DeepSVDD   & 82.87  & 67.33  & 69.67 & 85.01  &   \\
%    DAGMM       &81.83  & 44.34  & 71.05  & 70.07  &  \\
%   % LSTM-ED     & 83.58  &     65.56 &  \\
%    LSTM-VAE    & 84.95  & 67.52  & 72.74  & 90.58  &  \\ 
%    MAD-GAN     & 86.53  & 70.51  & 88.14  & 91.38  &  \\ 
%    USAD        & 84.60  & 57.25  & 86.34 & 92.72  &   \\ 
%    OMNI-Onomaly        & 85.28  & 41.02  & 84.34 & 89.89 &  \\ 
%    MSCRED       & 84.59  & 55.01 & 69.33   & 82.05    &   \\ 
%    MTAD-GAT    & 85.50  & 67.94  & 90.13  & 90.84 &   \\ 
%    NCAD        &  91.06 &  75.95       &\textbf{93.37} &  \textbf{95.60}&        \\
%    %GDN         & 89.57 & 71.54  &92.31  & \textbf{94.62}  & 62.54 \\ 
%    %LNT         & & & & &  \\\midrule
%    Ours         & \textbf{91.48} & \textbf{82.04} & 93.25 & 90.60 & \textbf{85.73} \\
%    \bottomrule
%     \end{tabular}
%     %}
%     %\end{adjustbox}
%     \label{tab:comparison_result}
%     %\vspace{-0.8cm}
% \end{table*}




\subsection{Ablation Study}
\label{section: ablation}
% In addition, we also include the scenario for which our base feature encoder is trained under the setting of DeepSVDD, where the latent representations of normal instances are pulled toward a fixed center. 
% As our proposed solution is based on a combination of contextual contrastive loss and discriminative contrastive loss, we want to see whether combining them can generate superior performance than using them separately. We also include several other variants of our model. More specifically, we provide the following variations of our model:
In this section, we compare different possible variants of our proposed framework against our default setting, with the details presented as follows: 1. DCL: The feature encoder network $g(\cdot)$ is trained purely under the discriminative contrastive loss (Eq.~\eqref{eq. contextual discriminative contrastive loss}). 2. CCL: The feature encoder network $g(\cdot)$ is trained purely under the contextual contrastive loss (Eq.~\eqref{eq. raw contextual one-class objective}). 3. CCL + reg: The encoder network $g(\cdot)$ is trained under the contextual contrastive loss, with a regularization term to enforce the variance of the latent representations of suspect and context sequences within a batch to be larger than zero. This setting is inspired by~\cite{coca}~\cite{vicreg}, which is a more intuitive approach to addressing the constant encoder solution. Specifically, it is defined as: 
\begin{align}
    &\LL_{\text{ccl+reg}} = \LL_{\text{ccl}} + v(\{S^{t}\}_{t\in B}) + v(\{C^{t}\}_{t\in B}) \\
    & v(\{S^{t}\}_{t \in B}) = \frac{1}{d} \sum_{j=1}^d \max(0, \gamma - \sqrt{\text{Var}(\{g(S^t)_j\}_{t \in B}) + \epsilon}) \label{eq: regularization on ccl}
\end{align}
where $B$ denotes an arbitrary mini-batch of samples containing $X^t$, $\gamma$ is set to 1 as in~\cite{vicreg}, and $\epsilon$ is a small scaler value to prevent numerical instabilities. The variance in Eq.~\eqref{eq: regularization on ccl} is calculated over the encoder outputs within the mini-batch $B$ during training. During inference, only $\LL_{\text{ccl}}$ is used as an anomaly score for a given test instance.
\begin{itemize}
    \item DCL: The feature encoder network $g(\cdot)$ is trained purely under the discriminative contrastive loss (Eq.~\eqref{eq. contextual discriminative contrastive loss}). 
    %The same loss is used as an anomaly score for each test instance.
    \item CCL: The feature encoder network $g(\cdot)$ is trained purely under the contextual contrastive loss (Eq.~\eqref{eq. raw contextual one-class objective}).
    %The same loss is used as an anomaly score for each test instance.
    \item OCC: The feature encoder network is trained under the one-class classification loss from DeepSVDD in a semi-supervised setting, with the training objective to map the latent representations of all normal instances into a hypersphere with minimum volume. 
    %During inference, the anomaly score for an instance is its distance from the hypersphere center.
    \item CCL + reg: The encoder network $g(\cdot)$ is trained under the contextual contrastive loss, with a regularization term to enforce the variance of the latent representations of suspect and context sequences within a batch to be larger than zero. This setting is inspired by~\cite{coca}~\cite{vicreg}, which is a more intuitive approach to addressing the constant encoder solution. Specifically, it is defined as:
    \begin{align}
        &\LL_{\text{ccl+reg}} = \LL_{\text{ccl}} + v(\{S^{t}\}_{t\in B}) + v(\{C^{t}\}_{t\in B}) \\
        & v(\{S^{t}\}_{t \in B}) = \frac{1}{d} \sum_{j=1}^d \max(0, \gamma - \sqrt{\text{Var}(\{g(S^t)_j\}_{t \in B}) + \epsilon}) \label{eq: regularization on ccl}
    \end{align}
    where $B$ denotes an arbitrary mini-batch of samples containing $X^t$, $\gamma$ is set to 1 as in~\cite{vicreg}, and $\epsilon$ is a small scaler value to prevent numerical instabilities. The variance in Eq.~\eqref{eq: regularization on ccl} is calculated over the encoder outputs within the mini-batch $B$ during training. During inference, only $\LL_{\text{ccl}}$ is used as an anomaly score for a given test instance.

\end{itemize}

\begin{figure*}[t]
    \centering
   % \includesvg[width=1\linewidth]{figures/Framework.svg}
        %\includesvg[height=3.2cm]{figures/neural_contrast/contextualAD_ablation_study.svg}
        \includegraphics[height=3.2cm]{figures/neural_contrast/contextualAD_ablation_study.eps}
        \caption{Performance comparison (F1 (\%)) for different model variants.}
    \label{fig: ablation_result}
\end{figure*}


% The results are summarized in Table~\ref{tab:ablation_result}. As we can see from the table, our model is able to achieve consistently higher performance over the four settings (at least $10\%$ improvement over all of the different variants on average). OCC and DCL do not explicitly include the contextual nature of temporally similar sequences in their loss functions, thereby, they perform relatively worse compared to our default setting (we provide data visualizations in the next sections for further details). On the other hand, CCL is designed to assign similar representations to sequences in near neighbors, however, it still performs worse than our default setting, we doubt there might be two reasons behind this, one is that due to the representation collapse problem, this loss may lead the encoder to find the parameter spaces that are close to the constant encoder solution, which eventually may fail to learn the rich semantic information of the input sequences. On the other hand, the combination of DCL and OCC actually performs the contextual contrastion between several different transformed versions of the suspect sequence and the context sequence, therefore it provides different angles in terms of normality to measure the similarity between suspect and context sequences. 
% \begin{table}[h!]
% \small
%     \setlength{\abovecaptionskip}{0cm}
%     %\setlength{\belowcaptionskip}{-0.1cm}
%     \centering
%     \caption{Performance comparison (F1 (\%)) for our method against different model variants} 
%     \begin{tabular}{ccccccc}\\ \toprule
%      \textbf{Settings}          &     \textbf{SWaT} &      \textbf{WADI} &     \textbf{MSL} &     \textbf{SMAP} &       \textbf{HAI}  \\ \midrule
%   % Default             &  91.99     &  \\ \midrule
% Ours     & \textbf{92.01} & \textbf{82.04} & \textbf{91.98} & \textbf{93.25} & \textbf{85.73} \\ \midrule
% OCC & 89.19 & 65.28 & 78.38 & 90.60 & 73.72 \\
% DCL      & 85.75 & 67.45 & 82.28 & 89.12 & 72.01 \\
% CCL      & 83.55 & 71.55 & 86.60 & 78.96 & 70.26 \\
% CCL+reg  & 91.64 & 59.39 & 86.52 & 89.44 & 53.98 \\ 
%    \bottomrule
%     \end{tabular}
%     \label{tab:ablation_result}
%     %\vspace{-0.8cm}
% \end{table}

Figure~\ref{fig: ablation_result} presents the results of our experiments. The findings indicate that our model consistently outperforms the four settings. Notably, the OCC and DCL settings do not consider the contextual nature of temporally similar sequences in their loss functions, resulting in relatively poorer performance. These findings are further supported by data visualizations in subsequent sections.
In contrast, the CCL setting is designed to assign similar representations to normal sequences in close proximity, but its performance falls short in comparison to our proposed approach. This can potentially be attributed to the representation collapse problem, wherein the loss function leads the encoder to converge to a parameter space that closely approximates the constant encoder solution. Consequently, the model may fail to capture the rich semantic information of normal sequences.
An alternative explanation for our improved performance over CCL is that the combination of DCL and OCC losses facilitates contextual contrastion between various transformed versions of the suspect and context sequences, thereby providing diverse perspectives on the normality of the sequences and allowing the measurement of similarity between two sequences from multiple angles.
% contextual contrastion between various transformed versions of the suspect and context sequences. This approach provides diverse perspectives on the normality of the sequences, allowing the measurement of similarity between suspect and context sequences from multiple angles.
% The performance of the CCL+reg setting, which incorporates a variance regularization term to enforce non-constant latent representations among training samples, does not outperform our default setting and even performs worse than the CCL setting for certain datasets. In contrast, the DCL loss in our default setting not only forces the transformations of suspect sequences to be semantically similar to the original sequences, but also effectively increases the diversity of the latent representations. 
This argument can be further inferred from the performance of the CCL+reg setting, wherein the addition of a variance regularization term to enforce non-constant latent representations among training samples does not outperform our default setting, and even performs worse than the CCL setting for certain datasets. In contrast, the incorporation of DCL loss in our framework not only increases the diversity of the latent representations, but also effectively forces the transformations of suspect sequences to be semantically similar to the original sequences.
%, but also effectively increases the diversity of the latent representations.



% The second argument can be kind of inferred from the performance of CCL+reg setting: Even if we add a variance regularization term to enforce the latent representations of training samples to be non-constant among themselves, the performance does not outperform our default setting, and sometimes can perform even worse than the CCL setting. In comparison to adding this variance regularization term which simply forces the latent representations of input sequences to be apart from each other, DCL loss has the additional effect of forcing the transformations of suspect sequences to be semantically similar to the original sequences. 


% \begin{table}[h!]
% \small
%     \setlength{\abovecaptionskip}{0cm}
%     %\setlength{\belowcaptionskip}{-0.1cm}
%     \centering
%     \caption{Performance comparison (F1 (\%)) for our base model trained under different losses} 
%     \begin{tabular}{ccccccc}\\ \toprule
%      \textbf{Settings}          &   \textbf{SWaT} & \textbf{WADI} & \textbf{SMAP} & \textbf{MSL} & \textbf{SMD}  \\ \midrule
%   % Default             &  91.99     &  \\ \midrule
%    Default & 92.49 & 0.74436 & 0.92137 & 0.94972 & 0.9673\\ \midrule
%    DCL & & & & & \\
%    CCL & & & & & \\
%    CCL + Reg & & & & & \\  
%    DeepSVDD loss  & 0.8914 & 0.6142 & 0.8639 & 0.8754
%  & \\ 
%    \bottomrule
%     \end{tabular}
%     \label{tab:ablation_result}
%     %\vspace{-0.8cm}
% \end{table}





\subsection{Data Visualization}
\begin{figure*}[t]
    \centering
   % \includesvg[width=1\linewidth]{figures/Framework.svg}
        %\includesvg[height=8cm, width=11.5cm]{figures/neural_contrast/showcases_tods.svg}
                \includegraphics[height=8cm, width=11.5cm]{figures/neural_contrast/showcases_tods.eps}

        \caption{The above figure showcases various types of anomalies present in the TODS dataset alongside the corresponding anomaly scores generated by our proposed method, as well as the DCL and OCC settings. The red lines denote the threshold values beyond which anomalies will be identified under different settings.}
    \label{fig: tods showcase}
%\vspace{0.5cm}
\end{figure*}
% To evaluate the effectiveness of our proposed framework in capturing contextual characteristics of anomalies in time series data, we conducted experiments on a univariate dataset (TODS) generated from rules outlined in \cite{tods}. The data adopts sinusoidal wave as the base shapelet to generate a univariate time series, with synthetic anomalies of various types injected, such as point anomalies, trend anomalies, seasonal anomalies, and pattern-wise anomalies (Examples of different types of anomalies are shown in Figure~\ref{fig: tods showcase}, and summary statistics of the data is shown in Table~\ref{tab:data_statistics}). We choose TODS specifically for data visualization as it offers clearly classified anomalies of different types, allowing for a better understanding of the performance of our model. Furthermore, the univariate nature of the dataset makes it easy to visualize the results directly from the plot. 

To evaluate the effectiveness of our proposed framework in capturing contextual characteristics of anomalies in time series data, we conducted experiments on a univariate dataset (TODS) generated from the rules outlined in~\cite{tods}. The TODS dataset adopts a sinusoidal wave as the base shapelet to generate a univariate time series, and synthetic anomalies of various types are injected using predefined rules. Examples of different types of anomalies are shown in Figure~\ref{fig: tods showcase}, and summary statistics of the data are shown in Table~\ref{tab:data_statistics}. TODS is specifically chosen for data visualization as it offers clearly classified anomalies of different types, enabling a better understanding of the performance of our model. Furthermore, the univariate nature of the dataset makes it easy to visualize the results directly from the plot.

We trained our model with three different loss functions: our default objective, the DCL setting, and the OCC setting. Figure \ref{fig: tods showcase} presents several showcases of different anomaly types, demonstrating the effectiveness of our proposed framework in identifying contextual anomalies. We observe that while global point anomalies are readily identifiable by all methods, OCC and DCL show relatively weaker performance in detecting other anomaly types that require contextual information. In contrast, our proposed method is capable of effectively identifying contextual anomalies by leveraging the deviation between the suspect and context window. This approach enables our method to be more sensitive to drastic changes in local context information.




% \begin{figure*}[t!]
% %\vspace{3pt}
% \begin{subfigure}[t]{0.49\textwidth}
%   \centering
%  % {{\small}}
%   %\includegraphics[width=.95\linewidth]{figures/Graph Encoder.pdf}  
% \includesvg[width=1\linewidth]{figures/swat_ts_unidentified_event3.svg}
%   \caption{An example for anomaly being identified by graph forecasting task (SwaT dataset)}
% \label{fig:swat_ts_unidentified}
% \end{subfigure}
% \hfill
% \begin{subfigure}[t]{0.49\textwidth}
%   \centering
%  % {{\small}}
% % \includegraphics[width=0.9\textwidth]{figures/target_performance_comparison.eps}
% \includesvg[width=1\linewidth]{figures/smd_machine-1-3_graph_unidentified_event2.svg}
%   \caption{An example for anomaly being identified by time series forecasting task (SMD dataset)}

% \label{fig:smd_graph_unidentified}
% \end{subfigure}
% %\newline
%   \caption{Examples for unidentified anomaly events by time-series forecasting task (a) and graph forecasting task (b). Examples (a) and (b) consist of six time-series segments selected from the SWaT dataset and the SMD dataset, respectively, where the anomalies are marked in yellow. The last three sub-figures of (a) and (b) are the error score for time-series forecasting, graph forecasting, and the combined score of them together with the red threshold line chosen according to the three scores.}
% \end{figure*}

% \begin{figure}[t!]
% \includesvg[width=1\linewidth]{figures/swat_event-6_graph_plus_real_data.svg}
%   \caption{A visual example for a list of learned inter-series graphs around the beginning of the yellow region where an anomaly resides on SWaT dataset.}
% \end{figure}

% \begin{figure}[t!]
% \includesvg[width=1\linewidth]{figures/swat_graph_deviation.svg}
%   \caption{A visual example showing the node degree deviation in abnormal and normal states.}
% \end{figure}

%\subsection{Sensitivity of hyper-parameters}


==> subtexes/experiments_IS.tex <==
\subsection{Datasets}
\begin{table}[h]
\small
    %\setlength{\abovecaptionskip}{0cm}
    %\setlength{\belowcaptionskip}{-0.1cm}
    \centering
    \caption{Summary statistics for datasets} 
    %\resizebox{\linewidth}{!}{
    \begin{tabular}{ccccc}\\ \toprule
               \textbf{Dataset} & \textbf{\# Channels} & \textbf{\# training} & \textbf{\# test} & \textbf{\% anomalies} \\ \midrule
   SWaT  &  51         &  495000   & 449919 & 12.14      \\
   WADI       &  123         &  784571    & 172801 & 5.77     \\  
SMAP       &   25        & 135183 & 427617 & 12.79     \\  
      MSL       &   55        & 58317 & 73729 & 10.53     \\
%    SMD       & 38         &  25300   & 25300 & 4.21    \\  

   HAI       & 79         &  921603   & 270003 & 1.93    \\  
%    TODS  & 1   & 40000 & 20000 & 2.50 \\
   \bottomrule
    \end{tabular}
    %}
    \label{tab:data_statistics}
    %\vspace{-0.8cm}
\end{table}
Five industrial real-world datasets, as shown in Table~\ref{tab:data_statistics}, are adopted for the evaluation of time series anomaly detection methods, which are 
 SWaT~\cite{mathur2016swat}, WADI~\cite{ahmed2017wadi}, HAI~\cite{hai21.03}, SMAP and MSL~\cite{lstm-ndt}. Each dataset has a unlabeled training set, and a separate test set with anomalies. SWaT and WADI are released by iTrust Center~\footnote{\url{https://itrust.sutd.edu.sg/itrust-labs_datasets/dataset_info/}} to support research in cybersecurity. The SWaT dataset is collected from a scaled-down, secure water treatment testbed. The WADI dataset is collected from a small-scale water distribution network. The HAI dataset derives from an Industrial Control System testbed enriched with a Hardware-In-the-Loop simulator. As a common pre-processing step similar to~\cite{gdn}, the training and test sets of the above three datasets have been down-sampled to 10-second intervals using median values with anomaly labels assigned 0 or 1 by taking the mode. MSL and SMAP, published by NASA, contain telemetry anomaly data from Mars Science Laboratory rover.




\subsection{Baseline Methods and Evaluation Metrics}
We compare our framework with common anomaly detection approaches as the baseline methods, including DeepSVDD~\cite{deepSVDD} and DAGMM~\cite{zong2018deep}, which are general anomaly detection deep learning-based models, and LSTM-VAE~\cite{lstm-vae}, MAD-GAN~\cite{mad-gan}, USAD~\cite{usad}, MSCRED~\cite{mscred}, MTAD-GAT~\cite{mtad-gat}, TranAD~\cite{tranAD}, NeuTralAD~\cite{neuralAD},  AnomalyTransformer~\cite{anomalyTransformer}, COCA~\cite{coca}, and DCdetector~\cite{yang2023dcdetector}, which are recent anomaly detection methods tailored specifically to time series data.

In line with previous studies~\cite{mtad-gat,omnianomaly,anomalyTransformer,tranAD}, we use the best F1-score as the main performance metric to evaluate the performance of anomaly detection. We follow the point-adjusting strategy suggested in \cite{omnianomaly}, which labels a whole anomaly segment as 1 as long as one of the points within the segment is detected as an anomaly. Since our primary contribution is not the development of a new thresholding method, we adopt this well-established practice to eliminate potential bias arising from selecting a specific thresholding method. This choice of reporting F1 scores ensures a fair and consistent comparison across all methods. However, acknowledging recent debates
about the point-adjusted F1 measure~\cite{kim2022towards}, we also provide the performance evaluated under the point-wise F1 (basically without the point-adjusting strategy), another widely used metric in the literature~\cite{gdn,fusagnet}. We believe a more rigorous performance evaluation of TSAD approaches would achieve consistently high performance across both metrics. In our experiments, we denote the point-adjusted F1 as F1*, and point-wise F1 as F1, respectively.

\subsection{Experimental Setting}
Our model is trained with an Adam optimizer~\cite{kingma2014adam} at a learning rate of 0.001 for 30 epochs. The 20$\%$ of the training set is selected as a validation set where the best epoch is stored based on the validation loss. Note that each input sample is a consecutive time window. Each sample is extracted by sliding the multivariate time series along the time dimension with stride 1. We employ early stopping with a patience of 10 epochs. The hidden dimension $d$ is set to 64, and the maximum number of TCN blocks is set to 8. The temperature $\tau$ and the number of transformations $K$ for DCL loss are set to 0.1 and 6, respectively. The sequence length is set to 30 and the prediction window size $w$ is set to 5. In addition, all performance results are averaged over five independent runs. 

% Regarding the selection of those parameters, we initially select $p$ from \{1, 5, 10\}, $K$ from \{6, 12\}, and $p$ from \{30, 50, 70, 90\} based on the loss of the $20\%$ of validation dataset. 

% The experiments conducted in the paper utilized an environment with Ubuntu 22.04.2 LTS operating system. The hardware configuration included an Nvidia RTX 4090 graphics card, equipped with CUDA version 12.0 and driver version 525.125.06. The CPU supporting the operations consisted of 4 cores and was complemented with 64GB of RAM. All implementations were done using Python 3.9. For the deep learning tasks, we employed the PyTorch framework, specifically version 2.0.1.


\subsection{Comparison Study}
The results are presented in Table~\ref{tab:comparison_result_f1}. First, both DAGMM and DeepSVDD display relatively lower performance due to their base model which does not account for temporal information. On the other hand, models such as MTAD-GAT, AnomalyTransformer, and DCdetector perform comparatively better in comparison to other methods, a testament to their effective utilization of GNNs to capture inter-series relationships or the global characteristics of time series through Transformers. Yet, CNT outperforms all others on average across all datasets (surpassing the best-performing baseline over 10\% in both F1* and F1), thus demonstrating the best balance between Recall and Precision. In comparison to these approaches, which utilize either time series forecasting or reconstruction-based methods, our approach utilizes the distance of latent representation between input instance and their contextual information as a criterion to identify anomalies, which are more robust to noise and less likely to overfit the data. 


% \begin{table*}[t!]
% %\small
%     \setlength{\abovecaptionskip}{0cm}
%     \centering
%         \caption{Performance comparison (F1 (\%)) on the benchmark datasets, precision (Pre (\%)) and recall (Rec (\%)) are attached. }
%     \begin{tabular}{cccccccccccccc}\\ \toprule
%                &   \multicolumn{3}{c}{\textbf{SWaT}} & \multicolumn{3}{c}{\textbf{MSL}} & \multicolumn{3}{c}{\textbf{WADI}} & \multicolumn{3}{c}{\textbf{HAI}} \\ \midrule
%                \textbf{Methods} & \textbf{F1} &  \textbf{Pre} & \textbf{Rec} & \textbf{F1} &  \textbf{Pre} & \textbf{Rec} & \textbf{F1} &  \textbf{Pre} & \textbf{Rec}  & \textbf{F1} &  \textbf{Pre} & \textbf{Rec}    \\ \midrule
% DAGMM              &  82.3 &         90.6 &      75.8 &  81.0 &         77.0 &      85.7 &  43.7 &         53.5 &      38.4 &  34.3 &         41.3 &      39.0 \\
% DeepSVDD           &  86.4 &         96.7 &      78.2 &  80.3 &         75.6 &      87.0 &  47.8 &         82.0 &      33.7 &  37.0 &         29.9 &      61.8 \\
% LSTM-VAE           &  81.9 &         97.9 &      70.4 &  87.5 &         87.8 &      87.7 &  64.6 &         66.3 &      63.0 &  70.8 &         67.8 &      76.4 \\
% USAD               &  83.0 &         97.3 &      72.4 &  60.0 &         74.4 &      60.0 &  35.6 &         66.9 &      26.5 &  73.6 &         87.7 &      65.5 \\
% MAD-GAN            &  80.5 &         98.3 &      68.2 &  77.1 &         71.7 &      86.6 &  73.7 &         88.2 &      63.6 &  17.5 &         16.5 &      48.0 \\
% MTAD-GAT           &  83.2 &         94.4 &      74.5 &  88.4 &         87.1 &      89.8 &  46.3 &         50.1 &      44.2 &  78.0 &         90.8 &      71.0 \\
% TranAD             &  83.2 &         96.5 &      73.2 &  79.2 &         71.5 &      89.9 &  41.4 &         62.0 &      31.6 &  73.0 &         88.4 &      63.1 \\
% NeuTralAD          &  90.6 &         91.3 &      90.1 &  60.6 &         46.8 &      86.4 &  54.2 &         61.9 &      50.3 &  48.4 &         41.8 &      64.7 \\
% LNT                &  86.4 &  95.0 &  79.3 &  90.5 &  91.3 &  89.8 &  35.6 &  74.2 &  24.8 &  54.4 &  72.2 &  48.5 \\
% AnomalyTransformer &  89.7 &         92.1 &      87.5 &  93.9 &         91.8 &      96.1 &  69.5 &         74.9 &      64.9 &  57.4 &         61.0 &      56.6 \\
% \midrule
% CNT &  \textbf{91.7} & 96.5 & 87.3 & \textbf{95.1} & 96.1&	94.3&  \textbf{81.6}	& 82.4	& 81.2   & \textbf{84.0} & 81.5 & 87.8  \\
%    \bottomrule
%     \end{tabular}
%     \label{tab:comparison_result_f1}
% \end{table*}

% \begin{table*}[t!]
% %\small
%     \setlength{\abovecaptionskip}{0cm}
%     \centering
%         \caption{Performance comparison (F1 (\%)) on the benchmark datasets, precision (Pre (\%)) and recall (Rec (\%)) are attached. }
%         \resizebox{\linewidth}{!}{
%         %\setlength{\tabcolsep}{1.68mm}{
%     \begin{tabular}{ccccccccccccccccc}\\ \toprule
%                &   \multicolumn{3}{c}{\textbf{SWaT}}  & \multicolumn{3}{c}{\textbf{WADI}} & \multicolumn{3}{c}{\textbf{MSL}}& \multicolumn{3}{c}{\textbf{SMAP}}& \multicolumn{3}{c}{\textbf{HAI}} \\ \midrule
%                \textbf{Methods} & \textbf{F1} &  \textbf{Pre} & \textbf{Rec} & \textbf{F1} &  \textbf{Pre} & \textbf{Rec} & \textbf{F1} &  \textbf{Pre} & \textbf{Rec}  & \textbf{F1} &  \textbf{Pre} & \textbf{Rec} & \textbf{F1} &  \textbf{Pre} & \textbf{Rec}    \\ \midrule

% LSTM-VAE           &  81.88 &        97.89 &     70.42 &  64.60 &        66.32 &     62.99 &  87.50 &        87.80 &     87.73 &  69.45 &        95.12 &     54.70 &  70.79 &        67.76 &     76.45 \\USAD               &  83.02 &        97.30 &     72.44 &  35.61 &        66.91 &     26.52 &  59.97 &        74.37 &     59.99 &  25.41 &        21.21 &     37.23 &  73.58 &        87.69 &     65.49 \\MAD-GAN            &  80.55 &        98.34 &     68.23 &  63.43 &        86.02 &     53.46 &  77.08 &        71.66 &     86.62 &  67.45 &        87.59 &     55.55 &  17.49 &        16.49 &     47.98 \\MSCRED             &  82.94 &        94.86 &     73.68 &  50.61 &        45.84 &     60.52 &  81.12 &        90.89 &     73.38 &  63.16 &        83.73 &     51.19 &  70.98 &        75.13 &     68.67 \\MTAD-GAT           &  83.25 &        94.43 &     74.47 &  46.27 &        50.06 &     44.17 &  94.18 &        93.09 &     95.32 &  91.28 &        88.51 &     94.57 &  77.99 &        90.83 &     70.96 \\NeuTralAD          &  90.65 &        91.34 &     90.06 &  54.16 &        61.92 &     50.29 &  60.60 &        46.75 &     86.42 &  53.26 &        37.24 &     93.82 &  48.41 &        41.82 &     64.74 \\TranAD             &  83.24 &        96.47 &     73.23 &  38.96 &        55.11 &     31.55 &  79.19 &        71.45 &     89.94 &  67.40 &        67.27 &     77.81 &  72.96 &        88.37 &     63.07 \\AnomalyTransformer &  89.59 &        91.99 &     87.31 &  66.60 &        72.40 &     62.09 &  93.80 &        92.44 &     95.23 &  96.36 &        94.14 &     98.71 &  56.48 &        60.30 &     55.32 \\COCA               &  85.27 &        88.64 &     82.47 &  49.02 &        54.13 &     51.65 &  85.55 &        86.37 &     84.99 &  54.87 &        50.08 &     67.06 &  71.45 &        74.35 &     71.70 \\DCdetector         &  89.58 &        91.63 &     87.62 &  82.17 &       76.93 &     88.43 &  93.78 &        93.56 &     94.11 &  \textbf{96.58} &        95.06 &     98.16 &  19.22 &        21.68 &     31.79 \\\midrule
% CNT &  \textbf{91.68} & 96.50 & 87.33 &  \textbf{82.90}	& 83.15	& 82.65 & \textbf{95.13} & 96.06&	94.26 & 89.6&	93.5	& 86.1  & \textbf{83.95} & 81.48 & 87.75  \\
%    \bottomrule
%     \end{tabular}}
%     \label{tab:comparison_result_f1}
% \end{table*}




\begin{table*}[t!]
%\small
    \setlength{\abovecaptionskip}{0cm}
    \centering
        \caption{Performance comparison (F1* (\%) and F1 (\%)) on the benchmark datasets. }
       \resizebox{\linewidth}{!}{
            %\setlength{\tabcolsep}{1.3mm}{
    \begin{tabular}{cccccccccccc}\\ \toprule
               &   \multicolumn{2}{c}{\textbf{SWaT}}  & \multicolumn{2}{c}{\textbf{WADI}} & \multicolumn{2}{c}{\textbf{MSL}}& \multicolumn{2}{c}{\textbf{SMAP}}& \multicolumn{2}{c}{\textbf{HAI}} \\ \midrule
               \textbf{Methods} & \textbf{F1*}  & \textbf{F1} & \textbf{F1*}  & \textbf{F1} & \textbf{F1*}  & \textbf{F1}  & \textbf{F1*}  & \textbf{F1}& \textbf{F1*}  & \textbf{F1}   \\ \midrule
DeepSVDD           &  86.42 &  73.86 &  43.70 &  27.31 &  80.28 &  23.74 &  58.75 &  23.93 &  37.02 &  15.07 \\DAGMM              &  59.25 &  62.30 &  43.68 &  24.68 &  80.96 &  19.20 &  75.31 &  22.69 &  34.32 &  13.38 \\
% LSTM-VAE           &  81.88 &  77.22 &  64.60 &  36.56 &  87.50 &  20.05 &  69.45 &  22.71 &  70.79 &  33.62 \\
LSTM-VAE           &  81.88 &  77.22 &  64.60 &  36.56 &  87.50 &  20.05 &  69.45 &  22.71 &  70.79 &  33.62 
\\USAD               &  83.02 &  76.84 &  35.61 &  28.23 &  59.97 &  23.59 &  25.41 &  28.05 &  73.58 &  39.70 \\MAD-GAN            &  80.55 &  73.65 &  63.43 &  15.95 &  77.08 &  20.17 &  67.45 &  24.27 &  17.49 &   5.73 \\MSCRED             &  82.94 &  75.94 &  50.61 &  29.61 &  81.12 &  27.92 &  63.16 &  23.04 &  70.98 &  36.95 \\MTAD-GAT           &  83.25 &  76.43 &  46.27 &  30.34 &  94.18 &  29.67 &  91.28 &  28.97 &  77.99 &  43.75 \\NeuTralAD          &  90.65 &  76.11 &  54.16 &  30.36 &  60.60 &  21.03 &  53.26 &  23.16 &  48.41 &  31.99 \\TranAD             &  83.24 &  76.90 &  38.96 &  27.31 &  79.19 &  24.55 &  67.40 &  23.50 &  72.96 &  43.54 \\AnomalyTransformer &  89.59 &  12.92 &  66.60 &   4.99 &  93.80 &   8.93 &  96.36 &   8.29 &  56.48 &   5.29 \\COCA               &  85.27 &  67.89 &  49.02 &  20.62 &  85.55 &  22.92 &  54.87 &  24.92 &  71.45 &  32.34 \\DCdetector         &  89.58 &  21.90 &  82.17 &  11.02 &  93.78 &  19.25 &  \textbf{96.58} &  24.20 &  19.22 &   3.94 \\ \midrule
CNT        &  \textbf{91.68} &  \textbf{77.27} &  \textbf{82.90} &  \textbf{37.55} &  \textbf{95.13} &  \textbf{30.40} &  92.33 &  \textbf{34.41} &  \textbf{83.95} &  \textbf{55.29} \\
% CNT &   \textbf{77.5} &  58.3 &   73.0  &  \textbf{37.6} &  \textbf{39.8} &   \textbf{78.4} &  \textbf{30.4} &  24.7 &   \textbf{72.1}  &  \textbf{34.4} &  \textbf{24.9} &   \textbf{69.1}  &  \textbf{55.3} &  \textbf{46.9} &   \textbf{85.6} \\
% CNT &   \textbf{77.5}  &   73.0  &  \textbf{37.6}  &   \textbf{78.4} &  \textbf{30.4} &     \textbf{72.1}  &  \textbf{34.4}  &   \textbf{69.1}  &  \textbf{55.3}  &   \textbf{85.6} \\
   \bottomrule
    \end{tabular}}
    \label{tab:comparison_result_f1}
\end{table*}


It is worth noting that while CNT is built on top of NeuTralAD, it surpasses NeuTralAD in performance by a significant margin. One key contribution to this enhanced efficacy is that NeuTralAD and CNT diverge in their approach to transformation diversity and semantic relevance. Specifically, NeuTralAD aims to learn a diverse set of transformations semantically associated with a given input time window. In other words, it focuses more on capturing the characteristics of the whole window. This can sometimes dilute anomaly effects, especially when the dominant data trends within the window are normal. In contrast, CNT enforces semantic similarity among learned transformations relative to a context window. It concentrates more on deviations between a short prediction window and its historical observations. Additionally, CNT introduces a notable computational advantage. Unlike NeuTralAD, which requires multiple passes of the transformations over the raw time series data, CNT applies the feature encoder a single time to the latent space, creating transformations more efficiently (see the computational analysis in Section~\ref{sec: computation analysis}). 


% Lastly, the LNT model, though conceptually similar to CNT, lags in performance. LNT combines CPC loss with neural transformation learning, relying on negative sample selection which can bias the training due to the prevalence of normal samples. Our CNT model avoids this with a negative-free training strategy, leveraging discriminative contrastive loss to prevent representation collapse.


\subsection{Ablation Study}
\label{section: ablation}
In this section, we aim to verify whether each component does contribute to our final performance. Specifically, we test the following two settings: 
1) CCL: Here, $g(\cdot)$ is trained exclusively under the contextual contrastive loss in Eq.~\eqref{eq. raw contextual one-class objective}. 
2) DCL: The feature encoder network $g(\cdot)$ is trained purely under the discriminative contrastive loss in Eq.\eqref{eq. contextual discriminative contrastive loss}. It's akin to NeutralAD, but transformations are applied to the feature encoder output rather than the original sequence.

Table~\ref{tab:ablation_result} presents the results of our experiments. The CCL setting is designed to assign similar representations to normal sequences in close proximity, but its performance falls short in comparison to our proposed approach. This can potentially be attributed to the representation collapse problem, wherein the loss function leads the encoder to converge to a parameter space that closely approximates the constant encoder solution. Consequently, the model may fail to capture the rich semantic information of normal sequences. On the other hand, The DCL configuration primarily encourages similarity between an in
\begin{table}[t!]%{r}{6cm}
%\small
   %\vspace{-0.4cm}
    \setlength{\abovecaptionskip}{0cm}
    %\setlength{\belowcaptionskip}{-0.1cm}
    \centering
    \caption{Performance comparison (F1* (\%) and F1 (\%)) for ablation study.} 
           \resizebox{\linewidth}{!}{
    \begin{tabular}{cccccccccccc}\\ \toprule
               &   \multicolumn{2}{c}{\textbf{SWaT}}  & \multicolumn{2}{c}{\textbf{WADI}} & \multicolumn{2}{c}{\textbf{MSL}}& \multicolumn{2}{c}{\textbf{SMAP}}& \multicolumn{2}{c}{\textbf{HAI}} \\ \midrule
               \textbf{Methods} & \textbf{F1*}  & \textbf{F1} & \textbf{F1*}  & \textbf{F1} & \textbf{F1*}  & \textbf{F1}  & \textbf{F1*}  & \textbf{F1}& \textbf{F1*}  & \textbf{F1}   \\ \midrule
  % Default             &  91.99     &  \\ \midrule
% CNT    & \textbf{91.}  & \textbf{81.6} & \textbf{95.1} & & \textbf{84.0}\\ \midrule
% DCL     &  85.1 &  30.4  &  81.2 & &  67.5 \\
% CCL &  88.0  &  66.2 &  91.5 &  &64.2 \\
CNT        &  \textbf{91.68} &  \textbf{77.27} &  \textbf{82.90} &  \textbf{37.55} &  \textbf{95.13} &  \textbf{30.40} &  \textbf{92.33} &  \textbf{34.41} &  \textbf{83.95} &  \textbf{55.29} \\ \midrule
% CCL           &  88.01 &  66.22 &  91.49 &  91.14 &  64.24 \\
% DCL                &  85.06 &  30.36 &  81.21 &  91.17 &  67.50 \\
CCL           &  88.01 &  21.66 &  66.22 &  35.99 &  91.49 &  29.54 &  91.14 &  26.97 &  64.24 &  46.88 \\
DCL               &  85.06 &  74.13 &  30.36 &  26.55 &  81.21 &  20.31 &  91.17 &  34.38	 &  67.50 &  41.21 \\
   \bottomrule
    \end{tabular}}
    \label{tab:ablation_result}
    %\vspace{-0.3cm}
\end{table}
put time window and its corresponding transformed sequences, prioritizing the modeling of characteristics across the entire time window. Consequently, anomalies within short time spans may be overlooked, resulting in negligible distance scores between the time window and its transformations, particularly for longer time windows. In contrast, our default setting emphasizes the discrepancy between the prediction window and the context window, thereby enhancing accurate anomaly detection within the overlapping region.

\subsection{Comparison against different model variants}
In Section~\ref{sec: self-supervised-learning}, we list a couple of existing techniques for contrastive learning that can alleviate the representation collapse issue. In this section, we show that our proposed framework is still superior to those variants. First, here are the details of the variants that we aim to compare with:
(1) CCL + Neg: A straightforward adaptation of CCL loss is to introduce the negative samples into the contrastive framework. Following the settings in CPC~\cite{cpc}, for each prediction window, we sample a random set of context windows within the batch as negative samples, and the feature encoder is trained under the infoNCE loss with the distance function replaced by the $l_2$ distance similar to the CCL loss.
(2) CCL + Vicreg: Similar to~\cite{vicreg}, $g(\cdot)$ is trained under the contextual contrastive loss, supplemented with a regularization term to ensure non-zero variance of the latent representations within a batch, thereby ensuring non-constant encoder outputs. The operation is defined as:
\begin{align}
    &L_{\text{ccl+vicreg}} = L_{\text{ccl}} + v(\{S^{t}\}_{t\in B}) + v(\{C^{t}\}_{t\in B}) \\
    & v(\{S^{t}\}_{t \in B}) = \frac{1}{d} \sum_{j=1}^d \max(0, \gamma - \sqrt{\text{Var}(\{g(S^t)_j\}_{t \in B}) + \epsilon}) \label{eq: regularization on ccl}
\end{align}
where $B$ denotes an arbitrary mini-batch of samples containing $X^t$, $\gamma$ is set to 1 as in~\cite{vicreg}, and $\epsilon$ is a small scaler value to prevent numerical instabilities. The variance in Eq.\eqref{eq: regularization on ccl} is computed over the encoder outputs within the batch $B$. During inference, only $L_{\text{ccl}}$ is used as the anomaly score. 
(3) CCL+Simsiam: Following~\cite{simsiam}, we create unique feature encoders for the prediction and context sequences, and compute two CCL losses. Each loss applies the stopping criterion on the representation of one sequence, with the other remaining detached. During inference, the sum of the two losses serves as the anomaly scores. The essential idea of this setting is to incorporate continuous target changes in order to prevent constant encoder solutions.


Table~\ref{tab:variants} presents the results of our experiments. First, we can see that incorporating the negative samples did improve the performance of CCL on average. 
\begin{table}[t!]
%\small
   %\vspace{-0.4cm}
    \setlength{\abovecaptionskip}{0cm}
    %\setlength{\belowcaptionskip}{-0.1cm}
    \centering
    \caption{Performance comparison (F1* (\%) and F1 (\%)) against different model variants.} 
           \resizebox{\linewidth}{!}{
    \begin{tabular}{cccccccccccc}\\ \toprule
               &   \multicolumn{2}{c}{\textbf{SWaT}}  & \multicolumn{2}{c}{\textbf{WADI}} & \multicolumn{2}{c}{\textbf{MSL}}& \multicolumn{2}{c}{\textbf{SMAP}}& \multicolumn{2}{c}{\textbf{HAI}} \\ \midrule
               \textbf{Methods} & \textbf{F1*}  & \textbf{F1} & \textbf{F1*}  & \textbf{F1} & \textbf{F1*}  & \textbf{F1}  & \textbf{F1*}  & \textbf{F1}& \textbf{F1*}  & \textbf{F1}   \\ \midrule
  % Default             &  91.99     &  \\ \midrule
% CNT    & \textbf{91.7} & \textbf{81.6} & \textbf{84.0} & \textbf{95.1} \\ \midrule
% CCL+Neg & & & & \\
% CCL+Vicreg  & 89.0 & 54.3 & 50.3 & 87.5\\
% CCL+Simsiam & \textbf{91.8}	&66.3	&78.3 &	92.7 \\ 
CNT        &  91.68 &  \textbf{77.27} &  \textbf{82.90} &  \textbf{37.55} &  \textbf{95.13} &  \textbf{30.40} &  \textbf{92.33} &  \textbf{34.41} &  \textbf{83.95} &  \textbf{55.29} \\ \midrule
% CCL+Neg               &  89.5 &  90.5 &  78.5 &  65.9 \\
% CCL+Vicreg               &  89.0 &  87.5 &  54.3 &  50.3 \\
% CCL+Simsiam &  \textbf{91.8} &  92.7 &  66.3 &  78.3 \\

CCL+Neg               &  89.54 &  20.77 &  78.50 &   8.39 &  90.50 &  18.31 &  90.12 &  22.82 &  65.95 &   9.21 \\
CCL+Vicreg                &  89.00 &  21.65 &  54.33 &  27.52 &  87.50 &  38.00 &  85.60 &  24.75 &  50.29 &  32.95 \\
CCL+Simsiam &  \textbf{92.57} &	77.17 &  66.33 &  35.49 &  92.69 &  30.34	 &    92.20 &	26.94 &  78.26 &  54.39 \\

   \bottomrule
    \end{tabular}}
    \label{tab:variants}
    %\vspace{-0.3cm}
\end{table}
but still underperform than CNT. One of the reasons is that the negative samples are selected from a dataset that consists mostly the normal samples. This could make the model a bit confused to distinguish normal samples from abnormal samples based on a wrong classification bound. For the rest of the settings, recall that the goal of the CCL+Vicreg and CCL+Siamsam settings, the direct variants of the CCL setting, aim to prevent the representation collapse issue. Yet, our model still surpasses them on average across datasets. Distinguished 
from these two configurations, the incorporation of DCL loss ensures not only non-constant latent representations but also compels transformations of the prediction sequences to stay semantically akin to original sequences. This provides a diverse range of perspectives on sequence normality and enables multi-angular similarity measurement between sequences. 




%\section{Extended Investigations}
% \subsection{Data Visualization}
% \begin{figure}[h]
%     \centering
%    % \includesvg[width=1\linewidth]{figures/Framework.svg}
%         \includesvg[height=9.5cm]{figures/neural_contrast/tods_case_study_more.svg}
%         % \includegraphics[height=8cm, width=11.5cm]{figures/neural_contrast/showcases_tods.svg}

%         \caption{A visual comparison among CNT, DCL, and CCL Models based on the TODS dataset. The top row shows the original time series with anomalies. Subsequent rows illustrate the corresponding anomaly scores from the CNT, DCL, and CCL models.}
%     \label{fig: tods showcase}
% %\vspace{0.5cm}
% \end{figure}
% We further conducted experiments on a univariate dataset (TODS) generated from the rules outlined in~\cite{tods}. The TODS dataset adopts a sinusoidal wave as the base shapelet to generate a univariate time series, and synthetic anomalies of various types are injected using predefined rules. Examples of different types of anomalies are shown in Figure~\ref{fig: tods showcase}. TODS is specifically chosen for data visualization as it offers clearly classified anomalies of different types, enabling a better understanding of the performance of our method. Furthermore, the univariate nature of the dataset makes it easy to visualize the results directly from the plot.
% % , and summary statistics of the data are shown in Table~\ref{tab:data_statistics}

% Figure~\ref{fig: tods showcase} provides a visual comparative analysis of anomaly detection performances among the CNT, DCL, and CCL models. The first row reveals the original time series data, featuring various types of anomalies such as shapelet, seasonal, and trend-based disturbances, excluding point anomalies for their consistent detection across models. CNT distinguishes itself by generating distinctly elevated anomaly scores in areas of anomalies, demonstrating exceptional sensitivity to aberrant patterns. DCL, however, shows a reduction in performance, particularly with trend anomalies where its scores fail to capture the irregularities effectively, hinting at a potential under-detection of nuanced anomalies in predominantly normal data streams. CCL, while producing sharper scores than DCL, does not achieve the same level of discrimination as CNT, occasionally misidentifying normal regions as anomalous. This underperformance is likely a consequence of the representation collapse issue, wherein the feature encoder defaults to oversimplified representations that overlook temporal dynamics within the data. Overall, CNT demonstrates a superior capacity to detect a wide range of anomalies with its discriminative scoring, while the DCL and CCL models appear constrained by their focus on broader patterns and a vulnerability to representation collapse, respectively.


\subsection{Analysis Of Learning Situations}
In Section~\ref{sec:theoretical analysis}, we show that simply using 
$L_{\text{ccl}}$ could lead to the representation collapse issue, where the feature representations of the context window and the prediction window collapse to the same constant. Then we proved that under the assumption that $L_{\text{dcl}}<K\log{K}$, this situation does not apply to the case when we combine the CCL and DCL losses. 
Figure~\ref{fig: loss_decay} shows the loss values per epoch for our model training under purely $L_{\text{ccl}}$ loss or training under both $L_{\text{cncl}}$ and $L_{\text{dcl}}$ (the default setting). It is clear that $L_{\text{ccl}}$ decays quickly to 0 without the regularization of $L_{\text{dcl}}$, which agrees with Proposition~\ref{props: constant encoder}. In contrast, with the additional constraints of $L_{\text{dcl}}$, $L_{\text{cncl}}$ decays much slowly compared to the former. 
\begin{figure}[t!]%r}{6.5cm}
%\vspace{-0.4cm}
\centering
\includegraphics[width=0.7\textwidth]{figures/neural_contrast/loss_decay.eps}  
\caption{Provided the loss value per epoch with the model trained on the WADI dataset. The small window is the zooming region for loss values from 20 to 30 epochs.}
\label{fig: loss_decay}
\vspace{-0.3cm}
\end{figure}
This implies that $L_{\text{dcl}}$ does add additional complexity to the CCL task, preventing from learning trivial feature representations. This is also verified in our ablation study that the combination of both losses can obtain a much higher performance than using $L_{\text{ccl}}$ only. Furthermore, as shown in Figure~\ref{fig: loss_decay}, we can see that the loss value of $L_{\text{dcl}}$ quickly falls below $K\log K$, which is around 4.67 when $K=6$ (the default parameter setting used in our experiments). This verifies the assumption in Proposition~\ref{props: non-constant encoder} is empirically applicable. 

\subsection{Data Visualization}
\begin{figure*}[h]
    \centering
   % \includesvg[width=1\linewidth]{figures/Framework.svg}
        \includesvg[height=11cm]{figures/neural_contrast/tods_case_study_more.svg}
        % \includegraphics[height=8cm, width=11.5cm]{figures/neural_contrast/showcases_tods.svg}

        \caption{A visual comparison among CNT, DCL, and CCL Models based on the TODS dataset. The top row shows the original time series with anomalies. Subsequent rows illustrate the corresponding anomaly scores from the CNT, DCL, and CCL models.}
    \label{fig: tods showcase}
%\vspace{0.5cm}
\end{figure*}
We further conducted experiments on a univariate dataset (TODS) generated from the rules outlined in~\cite{tods}. The TODS dataset adopts a sinusoidal wave as the base shapelet to generate a univariate time series, and synthetic anomalies of various types are injected using predefined rules. Examples of different types of anomalies are shown in Figure~\ref{fig: tods showcase}. TODS is specifically chosen for data visualization as it offers clearly classified anomalies of different types, enabling a better understanding of the performance of our method. Furthermore, the univariate nature of the dataset makes it easy to visualize the results directly from the plot.
% , and summary statistics of the data are shown in Table~\ref{tab:data_statistics}

Figure~\ref{fig: tods showcase} provides a visual comparative analysis of anomaly detection performances among the CNT, DCL, and CCL models. The first row reveals the original time series data, featuring various types of anomalies such as shapelet, seasonal, and trend-based disturbances, excluding point anomalies for their consistent detection across models. CNT distinguishes itself by generating distinctly elevated anomaly scores in areas of anomalies, demonstrating exceptional sensitivity to aberrant patterns. DCL, however, shows a reduction in performance, particularly with trend anomalies where its scores fail to capture the irregularities effectively, hinting at a potential under-detection of nuanced anomalies in predominantly normal data streams. CCL, while producing sharper scores than DCL, does not achieve the same level of discrimination as CNT, occasionally misidentifying normal regions as anomalous. This underperformance is likely a consequence of the representation collapse issue, wherein the feature encoder defaults to oversimplified representations that overlook temporal dynamics within the data. Overall, CNT demonstrates a superior capacity to detect a wide range of anomalies with its discriminative scoring, while the DCL and CCL models appear constrained by their focus on broader patterns and a vulnerability to representation collapse, respectively.


\subsection{Sensitivity of Hyper-parameters}
\begin{figure*}[h]
\centering
\begin{subfigure}[b]{1\linewidth}
    \centering
    \includegraphics[height=0.7cm]{figures/neural_contrast/legend.eps}
\end{subfigure}
\newline
%\vspace{0.5cm}
\centering
\begin{subfigure}[b]{.32\linewidth}
    \centering
    % \includegraphics[height=3cm]{figures/neural_contrast/seq_len_results.eps}
    \includegraphics[height=2.5cm]{figures/neural_contrast/seq_len_results.eps}
    %\caption{F1 vs. sliding window size}
    \caption{F1* vs. sequence length}
        \label{fig: seq_len_results}
\end{subfigure}
\begin{subfigure}[b]{.32\linewidth}
    \centering
    \includegraphics[height=2.5cm]{figures/neural_contrast/win_size_results.eps} 
    \caption{F1* vs. prediction window}
    \label{fig: win_size_results}
\end{subfigure}
\begin{subfigure}[b]{.32\linewidth}
    \centering
    \includegraphics[height=2.5cm]{figures/neural_contrast/n_transformations_results.eps} 
    \caption{F1* vs. transformations}
    \label{fig: n_transformations_results}
\end{subfigure}
\caption{(a) F1* versus sliding window size $w$ from 20 to 70; (b) F1* versus prediction window size $p$ from 1 to 9; (c) F1* versus number of transformations $K$ from 4 to 12.}
\label{fig: sensitivity_results}
\end{figure*}
In this section we conduct the sensitivity analysis on three hyper-parameters, the sizes of the sliding window $w$, the prediction window $p$, and the number of transformations $K$, with each parameter setting result averaged over 5 runs. Figure~\ref{fig: seq_len_results} illustrates the F1* score’s correlation with the sliding window size, with the prediction window size held constant at 5. We can see a relatively higher performance when the sequence length lies below 60. This finding is consistent with the performance of the majority of other baseline models, which also obtain optimal performances by adopting a sequence length within this range. Figure~\ref{fig: win_size_results} explores the F1* score’s variability in response to different prediction window sizes, while maintaining the sliding window size as default. The model exhibits relatively stable performance across different window sizes. Figure~\ref{fig: n_transformations_results} portrays the F1* score's responsiveness to varying numbers of transformations. The optimal performance for different datasets are also different. For example, the peak performance for SMAP is when $K=10$, while the one for MSL is when $K=6$. Overall, the performance appears relatively stable across the number of transformations.

% The optimal performance is approximately $K=6$, with some performance fluctuations across other values. Overall F1 score appears relatively stable across the number of transformations. In our experiments, we initially select $p$ from \{1, 5\}, $K$ from \{6, 12\}, and $p$ from \{30, 40, 50\} based on the loss of the $20\%$ of validation dataset. Our hyper-parameter selection was informed by ranges commonly used in baseline models, recognizing that in unsupervised learning contexts, lower validation loss doesn't necessarily equate to superior performance. We also deliberately constrained our hyper-parameter space to mitigate the risk of overfitting.

\subsection{Computational Analysis}
\label{sec: computation analysis}
\begin{figure}[h]
\centering
%\vspace{-0.2cm}
\includesvg[height=5cm]{figures/neural_contrast/computation_time.svg}
\caption{The training time per epoch and inference time of each model based on the SWaT dataset.}
\label{fig: computation_time}
\end{figure}
Figure~\ref{fig: computation_time} provides a comparison of the computational demands for various models, including both training time per epoch and inference time, benchmarked on the SWaT dataset. To ensure consistency across models, we maintained the same batch size during the training and testing phases. CNT demonstrates a considerable reduction in both training and inference times relative to other models, particularly NeutralAD. The efficiency of CNT can be attributed to its approach of applying transformations to the hidden representations - outputs of a feature encoder - rather than operating directly on the input data. This design choice means that CNT requires only a single pass of the data through the feature encoder, irrespective of the number of transformations applied, in stark contrast to NeutralAD, which must repeatedly process the input data for each transformation, incurring high computational overhead. Additionally, the observed computational efficiency in models like USAD, DeepSVDD, and DAGMM can be rationalized by their reliance on simpler MLP-based feature encoders, which are inherently less computationally intensive than more complex architectures.





==> subtexes/experiments_bigdata.tex <==
\subsection{Datasets}
\begin{table}[h]
\small
    %\setlength{\abovecaptionskip}{0cm}
    %\setlength{\belowcaptionskip}{-0.1cm}
    \centering
    \caption{Summary statistics for datasets} 
    %\resizebox{\linewidth}{!}{
    \begin{tabular}{ccccc}\\ \toprule
               \textbf{Dataset} & \textbf{\# Channels} & \textbf{\# training} & \textbf{\# test} & \textbf{\% anomalies} \\ \midrule
   SWaT  &  51         &  495000   & 449919 & 12.14      \\
   WADI       &  123         &  784571    & 172801 & 5.77     \\  
SMAP       &   25        & 135183 & 427617 & 12.79     \\  
      MSL       &   55        & 58317 & 73729 & 10.53     \\
%    SMD       & 38         &  25300   & 25300 & 4.21    \\  

   HAI       & 79         &  921603   & 270003 & 1.93    \\  
%    TODS  & 1   & 40000 & 20000 & 2.50 \\
   \bottomrule
    \end{tabular}
    %}
    \label{tab:data_statistics}
    %\vspace{-0.8cm}
\end{table}
Five industrial real-world datasets, as shown in Table~\ref{tab:data_statistics}, are adopted for the evaluation of time series anomaly detection methods, which are 
 SWaT~\cite{mathur2016swat}, WADI~\cite{ahmed2017wadi}, HAI~\cite{hai21.03}, SMAP and MSL~\cite{lstm-ndt}. Each dataset has a unlabeled training set, and a separate test set with anomalies. SWaT and WADI are released by iTrust Center~\footnote{\url{https://itrust.sutd.edu.sg/itrust-labs_datasets/dataset_info/}} to support research in cybersecurity. The SWaT dataset is collected from a scaled-down, secure water treatment testbed. The WADI dataset is collected from a small-scale water distribution network. The HAI dataset derives from an Industrial Control System testbed enriched with a Hardware-In-the-Loop simulator. As a common pre-processing step similar to~\cite{gdn}, the training and test sets of the above three datasets have been down-sampled to 10-second intervals using median values with anomaly labels assigned 0 or 1 by taking the mode. MSL and SMAP, published by NASA, contain telemetry anomaly data from Mars Science Laboratory rover.




\subsection{Baseline Methods and Evaluation Metrics}
We compare our framework with common anomaly detection approaches as the baseline methods, including DeepSVDD~\cite{deepSVDD} and DAGMM~\cite{zong2018deep}, which are general anomaly detection deep learning-based models, and LSTM-VAE~\cite{lstm-vae}, MAD-GAN~\cite{mad-gan}, USAD~\cite{usad}, MSCRED~\cite{mscred}, MTAD-GAT~\cite{mtad-gat}, TranAD~\cite{tranAD}, NeuTralAD~\cite{neuralAD},  AnomalyTransformer~\cite{anomalyTransformer}, COCA~\cite{coca},  DCdetector~\cite{yang2023dcdetector} and CST-GL~\cite{zheng2023correlationaware}, which are recent anomaly detection methods tailored specifically to time series data.

In line with previous studies~\cite{mtad-gat}~\cite{omnianomaly}~\cite{anomalyTransformer}~\cite{tranAD}, we use the best F1-score as the main performance metric to evaluate the performance of anomaly detection. We follow the point-adjusting strategy suggested in \cite{omnianomaly}, which labels a whole anomaly segment as 1 as long as one of the points within the segment is detected as an anomaly. Since our primary contribution is not the development of a new thresholding method, we adopt this well-established practice to eliminate potential bias arising from selecting a specific thresholding method. This choice of reporting F1 scores ensures a fair and consistent comparison across all methods. However, acknowledging recent debates
about the point-adjusted F1 measure~\cite{kim2022towards}, we also provide the performance evaluated under the point-wise F1 (basically without the point-adjusting strategy), another widely used metric in the literature~\cite{gdn}~\cite{fusagnet}. We believe a more rigorous performance evaluation of TSAD approaches would achieve consistently high performance across both metrics. In our experiments, we denote the point-adjusted F1 as F1*, and point-wise F1 as F1, respectively.

\subsection{Experimental Setting}
Our model is trained with an Adam optimizer~\cite{kingma2014adam} at a learning rate of 0.001 for 30 epochs. The 20$\%$ of the training set is selected as a validation set where the best epoch is stored based on the validation loss. Note that each input sample is a consecutive time window. Each sample is extracted by sliding the multivariate time series along the time dimension with stride 1. We employ early stopping with a patience of 10 epochs. The hidden dimension $d$ is set to 64, and the maximum number of TCN blocks is set to 8. The temperature $\tau$ and the number of transformations $K$ for DCL loss are set to 0.1 and 6, respectively. The sequence length is set to 30 and the prediction window size $w$ is set to 5. In addition, all performance results are averaged over five independent runs. 

% Regarding the selection of those parameters, we initially select $p$ from \{1, 5, 10\}, $K$ from \{6, 12\}, and $p$ from \{30, 50, 70, 90\} based on the loss of the $20\%$ of validation dataset. 

% The experiments conducted in the paper utilized an environment with Ubuntu 22.04.2 LTS operating system. The hardware configuration included an Nvidia RTX 4090 graphics card, equipped with CUDA version 12.0 and driver version 525.125.06. The CPU supporting the operations consisted of 4 cores and was complemented with 64GB of RAM. All implementations were done using Python 3.9. For the deep learning tasks, we employed the PyTorch framework, specifically version 2.0.1.


\subsection{Comparison Study}
The results are presented in Table~\ref{tab:comparison_result_f1}. First, both DAGMM and DeepSVDD display relatively lower performance due to their base model which does not account for temporal information. On the other hand, models such as MTAD-GAT, AnomalyTransformer, and DCdetector perform comparatively better in comparison to other methods, a testament to their effective utilization of GNNs to capture inter-series relationships or the global characteristics of time series through Transformers. Yet, CNT outperforms all others on average across all datasets (surpassing the best-performing baseline over 10\% in both F1* and F1), thus demonstrating the best balance between Recall and Precision. In comparison to these approaches, which utilize either time series forecasting or reconstruction-based methods, our approach utilizes the distance of latent representation between input instance and their contextual information as a criterion to identify anomalies, which are more robust to noise and less likely to overfit the data. 


% \begin{table*}[t!]
% %\small
%     \setlength{\abovecaptionskip}{0cm}
%     \centering
%         \caption{Performance comparison (F1 (\%)) on the benchmark datasets, precision (Pre (\%)) and recall (Rec (\%)) are attached. }
%     \begin{tabular}{cccccccccccccc}\\ \toprule
%                &   \multicolumn{3}{c}{\textbf{SWaT}} & \multicolumn{3}{c}{\textbf{MSL}} & \multicolumn{3}{c}{\textbf{WADI}} & \multicolumn{3}{c}{\textbf{HAI}} \\ \midrule
%                \textbf{Methods} & \textbf{F1} &  \textbf{Pre} & \textbf{Rec} & \textbf{F1} &  \textbf{Pre} & \textbf{Rec} & \textbf{F1} &  \textbf{Pre} & \textbf{Rec}  & \textbf{F1} &  \textbf{Pre} & \textbf{Rec}    \\ \midrule
% DAGMM              &  82.3 &         90.6 &      75.8 &  81.0 &         77.0 &      85.7 &  43.7 &         53.5 &      38.4 &  34.3 &         41.3 &      39.0 \\
% DeepSVDD           &  86.4 &         96.7 &      78.2 &  80.3 &         75.6 &      87.0 &  47.8 &         82.0 &      33.7 &  37.0 &         29.9 &      61.8 \\
% LSTM-VAE           &  81.9 &         97.9 &      70.4 &  87.5 &         87.8 &      87.7 &  64.6 &         66.3 &      63.0 &  70.8 &         67.8 &      76.4 \\
% USAD               &  83.0 &         97.3 &      72.4 &  60.0 &         74.4 &      60.0 &  35.6 &         66.9 &      26.5 &  73.6 &         87.7 &      65.5 \\
% MAD-GAN            &  80.5 &         98.3 &      68.2 &  77.1 &         71.7 &      86.6 &  73.7 &         88.2 &      63.6 &  17.5 &         16.5 &      48.0 \\
% MTAD-GAT           &  83.2 &         94.4 &      74.5 &  88.4 &         87.1 &      89.8 &  46.3 &         50.1 &      44.2 &  78.0 &         90.8 &      71.0 \\
% TranAD             &  83.2 &         96.5 &      73.2 &  79.2 &         71.5 &      89.9 &  41.4 &         62.0 &      31.6 &  73.0 &         88.4 &      63.1 \\
% NeuTralAD          &  90.6 &         91.3 &      90.1 &  60.6 &         46.8 &      86.4 &  54.2 &         61.9 &      50.3 &  48.4 &         41.8 &      64.7 \\
% LNT                &  86.4 &  95.0 &  79.3 &  90.5 &  91.3 &  89.8 &  35.6 &  74.2 &  24.8 &  54.4 &  72.2 &  48.5 \\
% AnomalyTransformer &  89.7 &         92.1 &      87.5 &  93.9 &         91.8 &      96.1 &  69.5 &         74.9 &      64.9 &  57.4 &         61.0 &      56.6 \\
% \midrule
% CNT &  \textbf{91.7} & 96.5 & 87.3 & \textbf{95.1} & 96.1&	94.3&  \textbf{81.6}	& 82.4	& 81.2   & \textbf{84.0} & 81.5 & 87.8  \\
%    \bottomrule
%     \end{tabular}
%     \label{tab:comparison_result_f1}
% \end{table*}

% \begin{table*}[t!]
% %\small
%     \setlength{\abovecaptionskip}{0cm}
%     \centering
%         \caption{Performance comparison (F1 (\%)) on the benchmark datasets, precision (Pre (\%)) and recall (Rec (\%)) are attached. }
%         \resizebox{\linewidth}{!}{
%         %\setlength{\tabcolsep}{1.68mm}{
%     \begin{tabular}{ccccccccccccccccc}\\ \toprule
%                &   \multicolumn{3}{c}{\textbf{SWaT}}  & \multicolumn{3}{c}{\textbf{WADI}} & \multicolumn{3}{c}{\textbf{MSL}}& \multicolumn{3}{c}{\textbf{SMAP}}& \multicolumn{3}{c}{\textbf{HAI}} \\ \midrule
%                \textbf{Methods} & \textbf{F1} &  \textbf{Pre} & \textbf{Rec} & \textbf{F1} &  \textbf{Pre} & \textbf{Rec} & \textbf{F1} &  \textbf{Pre} & \textbf{Rec}  & \textbf{F1} &  \textbf{Pre} & \textbf{Rec} & \textbf{F1} &  \textbf{Pre} & \textbf{Rec}    \\ \midrule

% LSTM-VAE           &  81.88 &        97.89 &     70.42 &  64.60 &        66.32 &     62.99 &  87.50 &        87.80 &     87.73 &  69.45 &        95.12 &     54.70 &  70.79 &        67.76 &     76.45 \\USAD               &  83.02 &        97.30 &     72.44 &  35.61 &        66.91 &     26.52 &  59.97 &        74.37 &     59.99 &  25.41 &        21.21 &     37.23 &  73.58 &        87.69 &     65.49 \\MAD-GAN            &  80.55 &        98.34 &     68.23 &  63.43 &        86.02 &     53.46 &  77.08 &        71.66 &     86.62 &  67.45 &        87.59 &     55.55 &  17.49 &        16.49 &     47.98 \\MSCRED             &  82.94 &        94.86 &     73.68 &  50.61 &        45.84 &     60.52 &  81.12 &        90.89 &     73.38 &  63.16 &        83.73 &     51.19 &  70.98 &        75.13 &     68.67 \\MTAD-GAT           &  83.25 &        94.43 &     74.47 &  46.27 &        50.06 &     44.17 &  94.18 &        93.09 &     95.32 &  91.28 &        88.51 &     94.57 &  77.99 &        90.83 &     70.96 \\NeuTralAD          &  90.65 &        91.34 &     90.06 &  54.16 &        61.92 &     50.29 &  60.60 &        46.75 &     86.42 &  53.26 &        37.24 &     93.82 &  48.41 &        41.82 &     64.74 \\TranAD             &  83.24 &        96.47 &     73.23 &  38.96 &        55.11 &     31.55 &  79.19 &        71.45 &     89.94 &  67.40 &        67.27 &     77.81 &  72.96 &        88.37 &     63.07 \\AnomalyTransformer &  89.59 &        91.99 &     87.31 &  66.60 &        72.40 &     62.09 &  93.80 &        92.44 &     95.23 &  96.36 &        94.14 &     98.71 &  56.48 &        60.30 &     55.32 \\COCA               &  85.27 &        88.64 &     82.47 &  49.02 &        54.13 &     51.65 &  85.55 &        86.37 &     84.99 &  54.87 &        50.08 &     67.06 &  71.45 &        74.35 &     71.70 \\DCdetector         &  89.58 &        91.63 &     87.62 &  82.17 &       76.93 &     88.43 &  93.78 &        93.56 &     94.11 &  \textbf{96.58} &        95.06 &     98.16 &  19.22 &        21.68 &     31.79 \\\midrule
% CNT &  \textbf{91.68} & 96.50 & 87.33 &  \textbf{82.90}	& 83.15	& 82.65 & \textbf{95.13} & 96.06&	94.26 & 89.6&	93.5	& 86.1  & \textbf{83.95} & 81.48 & 87.75  \\
%    \bottomrule
%     \end{tabular}}
%     \label{tab:comparison_result_f1}
% \end{table*}




\begin{table*}[t!]
%\small
    \setlength{\abovecaptionskip}{0cm}
    \centering
        \caption{Performance comparison (F1* (\%) and F1 (\%)) on the benchmark datasets. }
       \resizebox{\linewidth}{!}{
            %\setlength{\tabcolsep}{1.3mm}{
    \begin{tabular}{cccccccccccc}\\ \toprule
               &   \multicolumn{2}{c}{\textbf{SWaT}}  & \multicolumn{2}{c}{\textbf{WADI}} & \multicolumn{2}{c}{\textbf{MSL}}& \multicolumn{2}{c}{\textbf{SMAP}}& \multicolumn{2}{c}{\textbf{HAI}} \\ \midrule
               \textbf{Methods} & \textbf{F1*}  & \textbf{F1} & \textbf{F1*}  & \textbf{F1} & \textbf{F1*}  & \textbf{F1}  & \textbf{F1*}  & \textbf{F1}& \textbf{F1*}  & \textbf{F1}   \\ \midrule
DeepSVDD           &  86.42 &  73.86 &  43.70 &  27.31 &  80.28 &  23.74 &  58.75 &  23.93 &  37.02 &  15.07 \\DAGMM              &  59.25 &  62.30 &  43.68 &  24.68 &  80.96 &  19.20 &  75.31 &  22.69 &  34.32 &  13.38 \\
% LSTM-VAE           &  81.88 &  77.22 &  64.60 &  36.56 &  87.50 &  20.05 &  69.45 &  22.71 &  70.79 &  33.62 \\
LSTM-VAE           &  81.88 &  77.22 &  64.60 &  36.56 &  87.50 &  20.05 &  69.45 &  22.71 &  70.79 &  33.62 
\\USAD               &  83.02 &  76.84 &  35.61 &  28.23 &  59.97 &  23.59 &  25.41 &  28.05 &  73.58 &  39.70 \\MAD-GAN            &  80.55 &  73.65 &  63.43 &  15.95 &  77.08 &  20.17 &  67.45 &  24.27 &  17.49 &   5.73 \\MSCRED             &  82.94 &  75.94 &  50.61 &  29.61 &  81.12 &  27.92 &  63.16 &  23.04 &  70.98 &  36.95 \\MTAD-GAT           &  83.25 &  76.43 &  46.27 &  30.34 &  94.18 &  29.67 &  91.28 &  28.97 &  77.99 &  43.75 \\NeuTralAD          &  90.65 &  76.11 &  54.16 &  30.36 &  60.60 &  21.03 &  53.26 &  23.16 &  48.41 &  31.99 \\TranAD             &  83.24 &  76.90 &  38.96 &  27.31 &  79.19 &  24.55 &  67.40 &  23.50 &  72.96 &  43.54 \\AnomalyTransformer &  89.59 &  12.92 &  66.60 &   4.99 &  93.80 &   8.93 &  96.36 &   8.29 &  56.48 &   5.29 \\COCA               &  85.27 &  67.89 &  49.02 &  20.62 &  85.55 &  22.92 &  54.87 &  24.92 &  71.45 &  32.34 \\DCdetector         &  89.58 &  21.90 &  82.17 &  11.02 &  93.78 &  19.25 &  \textbf{96.58} &  24.20 &  19.22 &   3.94 \\ 
CST-GL & 86.27 & 76.84 & 65.71 & 34.12 & 87.41 & 22.78 & 71.16 & 24.70 & 26.87 & 14.59 \\
\midrule
CNT (ours)        &  \textbf{91.68} &  \textbf{77.27} &  \textbf{82.90} &  \textbf{37.55} &  \textbf{95.13} &  \textbf{30.40} &  92.33 &  \textbf{34.41} &  \textbf{83.95} &  \textbf{55.29} \\
% CNT &   \textbf{77.5} &  58.3 &   73.0  &  \textbf{37.6} &  \textbf{39.8} &   \textbf{78.4} &  \textbf{30.4} &  24.7 &   \textbf{72.1}  &  \textbf{34.4} &  \textbf{24.9} &   \textbf{69.1}  &  \textbf{55.3} &  \textbf{46.9} &   \textbf{85.6} \\
% CNT &   \textbf{77.5}  &   73.0  &  \textbf{37.6}  &   \textbf{78.4} &  \textbf{30.4} &     \textbf{72.1}  &  \textbf{34.4}  &   \textbf{69.1}  &  \textbf{55.3}  &   \textbf{85.6} \\
   \bottomrule
    \end{tabular}}
    \label{tab:comparison_result_f1}
\end{table*}

\begin{table*}[t]%{r}{6cm}
%\small
   %\vspace{-0.4cm}
    \setlength{\abovecaptionskip}{0cm}
    %\setlength{\belowcaptionskip}{-0.1cm}
    \centering
    \caption{Performance comparison (F1* (\%) and F1 (\%)) for ablation study.} 
           \resizebox{\linewidth}{!}{
    \begin{tabular}{cccccccccccc}\\ \toprule
               &   \multicolumn{2}{c}{\textbf{SWaT}}  & \multicolumn{2}{c}{\textbf{WADI}} & \multicolumn{2}{c}{\textbf{MSL}}& \multicolumn{2}{c}{\textbf{SMAP}}& \multicolumn{2}{c}{\textbf{HAI}} \\ \midrule
               \textbf{Methods} & \textbf{F1*}  & \textbf{F1} & \textbf{F1*}  & \textbf{F1} & \textbf{F1*}  & \textbf{F1}  & \textbf{F1*}  & \textbf{F1}& \textbf{F1*}  & \textbf{F1}   \\ \midrule
  % Default             &  91.99     &  \\ \midrule
% CNT    & \textbf{91.}  & \textbf{81.6} & \textbf{95.1} & & \textbf{84.0}\\ \midrule
% DCL     &  85.1 &  30.4  &  81.2 & &  67.5 \\
% CCL &  88.0  &  66.2 &  91.5 &  &64.2 \\
CNT (ours)        &  \textbf{91.68} &  \textbf{77.27} &  \textbf{82.90} &  \textbf{37.55} &  \textbf{95.13} &  \textbf{30.40} &  \textbf{92.33} &  \textbf{34.41} &  \textbf{83.95} &  \textbf{55.29} \\ \midrule
% CCL           &  88.01 &  66.22 &  91.49 &  91.14 &  64.24 \\
% DCL                &  85.06 &  30.36 &  81.21 &  91.17 &  67.50 \\
CCL           &  88.01 &  21.66 &  66.22 &  35.99 &  91.49 &  29.54 &  91.14 &  26.97 &  64.24 &  46.88 \\
DCL               &  85.06 &  74.13 &  30.36 &  26.55 &  81.21 &  20.31 &  91.17 &  34.38	 &  67.50 &  41.21 \\
   \bottomrule
    \end{tabular}}
    \label{tab:ablation_result}
    %\vspace{-0.3cm}
\end{table*}


\begin{table*}[t!]
%\small
   %\vspace{-0.4cm}
    \setlength{\abovecaptionskip}{0cm}
    %\setlength{\belowcaptionskip}{-0.1cm}
    \centering
    \caption{Performance comparison (F1* (\%) and F1 (\%)) against different model variants.} 
           \resizebox{\linewidth}{!}{
    \begin{tabular}{cccccccccccc}\\ \toprule
               &   \multicolumn{2}{c}{\textbf{SWaT}}  & \multicolumn{2}{c}{\textbf{WADI}} & \multicolumn{2}{c}{\textbf{MSL}}& \multicolumn{2}{c}{\textbf{SMAP}}& \multicolumn{2}{c}{\textbf{HAI}} \\ \midrule
               \textbf{Methods} & \textbf{F1*}  & \textbf{F1} & \textbf{F1*}  & \textbf{F1} & \textbf{F1*}  & \textbf{F1}  & \textbf{F1*}  & \textbf{F1}& \textbf{F1*}  & \textbf{F1}   \\ \midrule
  % Default             &  91.99     &  \\ \midrule
% CNT    & \textbf{91.7} & \textbf{81.6} & \textbf{84.0} & \textbf{95.1} \\ \midrule
% CCL+Neg & & & & \\
% CCL+Vicreg  & 89.0 & 54.3 & 50.3 & 87.5\\
% CCL+Simsiam & \textbf{91.8}	&66.3	&78.3 &	92.7 \\ 
CNT (ours)         &  91.68 &  \textbf{77.27} &  \textbf{82.90} &  \textbf{37.55} &  \textbf{95.13} &  \textbf{30.40} &  \textbf{92.33} &  \textbf{34.41} &  \textbf{83.95} &  \textbf{55.29} \\ \midrule
% CCL+Neg               &  89.5 &  90.5 &  78.5 &  65.9 \\
% CCL+Vicreg               &  89.0 &  87.5 &  54.3 &  50.3 \\
% CCL+Simsiam &  \textbf{91.8} &  92.7 &  66.3 &  78.3 \\

CCL+Neg               &  89.54 &  20.77 &  78.50 &   8.39 &  90.50 &  18.31 &  90.12 &  22.82 &  65.95 &   9.21 \\
CCL+Vicreg                &  89.00 &  21.65 &  54.33 &  27.52 &  87.50 &  38.00 &  85.60 &  24.75 &  50.29 &  32.95 \\
CCL+Simsiam &  \textbf{92.57} &	77.17 &  66.33 &  35.49 &  92.69 &  30.34	 &    92.20 &	26.94 &  78.26 &  54.39 \\

   \bottomrule
    \end{tabular}}
    \label{tab:variants}
    %\vspace{-0.3cm}
\end{table*}


It is worth noting that while CNT is built on top of NeuTralAD, it surpasses NeuTralAD in performance by a significant margin. One key contribution to this enhanced efficacy is that NeuTralAD and CNT diverge in their approach to transformation diversity and semantic relevance. Specifically, NeuTralAD aims to learn a diverse set of transformations semantically associated with a given input time window. In other words, it focuses more on capturing the characteristics of the whole window. This can sometimes dilute anomaly effects, especially when the dominant data trends within the window are normal. In contrast, CNT enforces semantic similarity among learned transformations relative to a context window. It concentrates more on deviations between a short prediction window and its historical observations. Additionally, CNT introduces a notable computational advantage. Unlike NeuTralAD, which requires multiple passes of the transformations over the raw time series data, CNT applies the feature encoder a single time to the latent space, creating transformations more efficiently (see the computational analysis in Section~\ref{sec: computation analysis}). 


% Lastly, the LNT model, though conceptually similar to CNT, lags in performance. LNT combines CPC loss with neural transformation learning, relying on negative sample selection which can bias the training due to the prevalence of normal samples. Our CNT model avoids this with a negative-free training strategy, leveraging discriminative contrastive loss to prevent representation collapse.


\subsection{Ablation Study}
\label{section: ablation}
In this section, we aim to verify whether each component does contribute to our final performance. Specifically, we test the following two settings: 
1) CCL: Here, $g(\cdot)$ is trained exclusively under the contextual contrastive loss in Eq.~\eqref{eq. raw contextual one-class objective}. 
2) DCL: The feature encoder network $g(\cdot)$ is trained purely under the discriminative contrastive loss in Eq.\eqref{eq. contextual discriminative contrastive loss}. It's akin to NeutralAD, but transformations are applied to the feature encoder output rather than the original sequence.

Table~\ref{tab:ablation_result} presents the results of our experiments. The CCL setting is designed to assign similar representations to normal sequences in close proximity, but its performance falls short in comparison to our proposed approach. This can potentially be attributed to the representation collapse problem, wherein the loss function leads the encoder to converge to a parameter space that closely approximates the constant encoder solution. Consequently, the model may fail to capture the rich semantic information of normal sequences. On the other hand, The DCL configuration primarily encourages similarity between an in

put time window and its corresponding transformed sequences, prioritizing the modeling of characteristics across the entire time window. Consequently, anomalies within short time spans may be overlooked, resulting in negligible distance scores between the time window and its transformations, particularly for longer time windows. In contrast, our default setting emphasizes the discrepancy between the prediction window and the context window, thereby enhancing accurate anomaly detection within the overlapping region.

\subsection{Comparison against different model variants}
In Section~\ref{sec: self-supervised-learning}, we list a couple of existing techniques for contrastive learning that can alleviate the representation collapse issue. In this section, we show that our proposed framework is still superior to those variants. First, here are the details of the variants that we aim to compare with:
(1) CCL + Neg: A straightforward adaptation of CCL loss is to introduce the negative samples into the contrastive framework. Following the settings in CPC~\cite{cpc}, for each prediction window, we sample a random set of context windows within the batch as negative samples, and the feature encoder is trained under the infoNCE loss with the distance function replaced by the $l_2$ distance similar to the CCL loss.
(2) CCL + Vicreg: Similar to~\cite{vicreg}, $g(\cdot)$ is trained under the contextual contrastive loss, supplemented with a regularization term to ensure non-zero variance of the latent representations within a batch, thereby ensuring non-constant encoder outputs. The operation is defined as:
% \begin{align}
%     &
%     \resizebox{.85\hsize}{!}{L_{\text{ccl+vicreg}} = L_{\text{ccl}} + v(\{S^{t}\}_{t\in B}) + v(\{C^{t}\}_{t\in B})} \\
%     & 
% \resizebox{.85\hsize}{!}{v(\{S^{t}\}_{t \in B}) = \frac{1}{d} \sum_{j=1}^d \max(0, \gamma - \sqrt{\text{Var}(\{g(S^t)_j\}_{t \in B}) + \epsilon})} \label{eq: regularization on ccl}
% \end{align}
\begin{align}
& L_{\text{ccl+vicreg}} = L_{\text{ccl}} + v(\{S^{t}\}_{t\in B}) + v(\{C^{t}\}_{t\in B}) \\
& v(\{S^{t}\}_{t \in B}) = \frac{1}{d} \sum_{j=1}^d \max(0, \gamma - \sqrt{\text{Var}(\{g(S^t)_j\}_{t \in B}) + \epsilon} \label{eq: regularization on ccl}
\end{align}
where $B$ denotes an arbitrary mini-batch of samples containing $X^t$, $\gamma$ is set to 1 as in~\cite{vicreg}, and $\epsilon$ is a small scaler value to prevent numerical instabilities. The variance in Eq.\eqref{eq: regularization on ccl} is computed over the encoder outputs within the batch $B$. During inference, only $L_{\text{ccl}}$ is used as the anomaly score. 
(3) CCL+Simsiam: Following~\cite{simsiam}, we create unique feature encoders for the prediction and context sequences, and compute two CCL losses. Each loss applies the stopping criterion on the representation of one sequence, with the other remaining detached. During inference, the sum of the two losses serves as the anomaly scores. The essential idea of this setting is to incorporate continuous target changes in order to prevent constant encoder solutions.


Table~\ref{tab:variants} presents the results of our experiments. First, we can see that incorporating the negative samples did improve the performance of CCL on average. 
but still underperform than CNT. One of the reasons is that the negative samples are selected from a dataset that consists mostly the normal samples. This could make the model a bit confused to distinguish normal samples from abnormal samples based on a wrong classification bound. For the rest of the settings, recall that the goal of the CCL+Vicreg and CCL+Siamsam settings, the direct variants of the CCL setting, aim to prevent the representation collapse issue. Yet, our model still surpasses them on average across datasets. Distinguished 
from these two configurations, the incorporation of DCL loss ensures not only non-constant latent representations but also compels transformations of the prediction sequences to stay semantically akin to original sequences. This provides a diverse range of perspectives on sequence normality and enables multi-angular similarity measurement between sequences. 




%\section{Extended Investigations}
% \subsection{Data Visualization}
% \begin{figure}[h]
%     \centering
%    % \includesvg[width=1\linewidth]{figures/Framework.svg}
%         \includesvg[height=9.5cm]{figures/neural_contrast/tods_case_study_more.svg}
%         % \includegraphics[height=8cm, width=11.5cm]{figures/neural_contrast/showcases_tods.svg}

%         \caption{A visual comparison among CNT, DCL, and CCL Models based on the TODS dataset. The top row shows the original time series with anomalies. Subsequent rows illustrate the corresponding anomaly scores from the CNT, DCL, and CCL models.}
%     \label{fig: tods showcase}
% %\vspace{0.5cm}
% \end{figure}
% We further conducted experiments on a univariate dataset (TODS) generated from the rules outlined in~\cite{tods}. The TODS dataset adopts a sinusoidal wave as the base shapelet to generate a univariate time series, and synthetic anomalies of various types are injected using predefined rules. Examples of different types of anomalies are shown in Figure~\ref{fig: tods showcase}. TODS is specifically chosen for data visualization as it offers clearly classified anomalies of different types, enabling a better understanding of the performance of our method. Furthermore, the univariate nature of the dataset makes it easy to visualize the results directly from the plot.
% % , and summary statistics of the data are shown in Table~\ref{tab:data_statistics}

% Figure~\ref{fig: tods showcase} provides a visual comparative analysis of anomaly detection performances among the CNT, DCL, and CCL models. The first row reveals the original time series data, featuring various types of anomalies such as shapelet, seasonal, and trend-based disturbances, excluding point anomalies for their consistent detection across models. CNT distinguishes itself by generating distinctly elevated anomaly scores in areas of anomalies, demonstrating exceptional sensitivity to aberrant patterns. DCL, however, shows a reduction in performance, particularly with trend anomalies where its scores fail to capture the irregularities effectively, hinting at a potential under-detection of nuanced anomalies in predominantly normal data streams. CCL, while producing sharper scores than DCL, does not achieve the same level of discrimination as CNT, occasionally misidentifying normal regions as anomalous. This underperformance is likely a consequence of the representation collapse issue, wherein the feature encoder defaults to oversimplified representations that overlook temporal dynamics within the data. Overall, CNT demonstrates a superior capacity to detect a wide range of anomalies with its discriminative scoring, while the DCL and CCL models appear constrained by their focus on broader patterns and a vulnerability to representation collapse, respectively.


\subsection{Analysis Of Learning Situations}
In Section~\ref{sec:theoretical analysis}, we show that simply using 
$L_{\text{ccl}}$ could lead to the representation collapse issue, where the feature representations of the context window and the prediction window collapse to the same constant. Then we proved that under the assumption that $L_{\text{dcl}}<K\log{K}$, this situation does not apply to the case when we combine the CCL and DCL losses. 
Figure~\ref{fig: loss_decay} shows the loss values per epoch for our model training under purely $L_{\text{ccl}}$ loss or training under both $L_{\text{cncl}}$ and $L_{\text{dcl}}$ (the default setting). It is clear that $L_{\text{ccl}}$ decays quickly to 0 without the regularization of $L_{\text{dcl}}$, which agrees with Proposition~\ref{props: constant encoder}. In contrast, with the additional constraints of $L_{\text{dcl}}$, $L_{\text{cncl}}$ decays much slowly compared to the former. 
\begin{figure}[t!]%r}{6.5cm}
%\vspace{-0.4cm}
\centering
\includegraphics[width=0.6\linewidth]{figures/neural_contrast/loss_decay.eps}  
\caption{Provided the loss value per epoch with the model trained on the WADI dataset. The small window is the zooming region for loss values from 20 to 30 epochs.}
\label{fig: loss_decay}
\vspace{-0.3cm}
\end{figure}
This implies that $L_{\text{dcl}}$ does add additional complexity to the CCL task, preventing from learning trivial feature representations. This is also verified in our ablation study that the combination of both losses can obtain a much higher performance than using $L_{\text{ccl}}$ only. Furthermore, as shown in Figure~\ref{fig: loss_decay}, we can see that the loss value of $L_{\text{dcl}}$ quickly falls below $K\log K$, which is around 4.67 when $K=6$ (the default parameter setting used in our experiments). This verifies the assumption in Proposition~\ref{props: non-constant encoder} is empirically applicable. 

\begin{figure*}[t!]
    \centering
   % \includesvg[width=1\linewidth]{figures/Framework.svg}
        \includesvg[height=9cm]{figures/neural_contrast/tods_case_study_more.svg}
        % \includegraphics[height=8cm, width=11.5cm]{figures/neural_contrast/showcases_tods.svg}

        \caption{A visual comparison among CNT, DCL, and CCL Models based on the TODS dataset. The top row shows the original time series with anomalies. Subsequent rows illustrate the corresponding anomaly scores from the CNT, DCL, and CCL models.}
    \label{fig: tods showcase}
%\vspace{0.5cm}
\end{figure*}

\subsection{Data Visualization}

We further conducted experiments on a univariate dataset (TODS) generated from the rules outlined in~\cite{tods}. The TODS dataset adopts a sinusoidal wave as the base shapelet to generate a univariate time series, and synthetic anomalies of various types are injected using predefined rules. Examples of different types of anomalies are shown in Figure~\ref{fig: tods showcase}. TODS is specifically chosen for data visualization as it offers clearly classified anomalies of different types, enabling a better understanding of the performance of our method. Furthermore, the univariate nature of the dataset makes it easy to visualize the results directly from the plot.
% , and summary statistics of the data are shown in Table~\ref{tab:data_statistics}

Figure~\ref{fig: tods showcase} provides a visual comparative analysis of anomaly detection performances among the CNT, DCL, and CCL models. The first row reveals the original time series data, featuring various types of anomalies such as shapelet, seasonal, and trend-based disturbances, excluding point anomalies for their consistent detection across models. CNT distinguishes itself by generating distinctly elevated anomaly scores in areas of anomalies, demonstrating exceptional sensitivity to aberrant patterns. DCL, however, shows a reduction in performance, particularly with trend anomalies where its scores fail to capture the irregularities effectively, hinting at a potential under-detection of nuanced anomalies in predominantly normal data streams. CCL, while producing sharper scores than DCL, does not achieve the same level of discrimination as CNT, occasionally misidentifying normal regions as anomalous. This underperformance is likely a consequence of the representation collapse issue, wherein the feature encoder defaults to oversimplified representations that overlook temporal dynamics within the data. Overall, CNT demonstrates a superior capacity to detect a wide range of anomalies with its discriminative scoring, while the DCL and CCL models appear constrained by their focus on broader patterns and a vulnerability to representation collapse, respectively.

\begin{figure*}[t!]
\centering
\begin{subfigure}[b]{1\linewidth}
    \centering
    \includegraphics[height=0.7cm]{figures/neural_contrast/legend.eps}
\end{subfigure}
\newline
%\vspace{0.5cm}
\centering
\begin{subfigure}[b]{.32\linewidth}
    \centering
    % \includegraphics[height=3cm]{figures/neural_contrast/seq_len_results.eps}
    \includegraphics[height=2.5cm]{figures/neural_contrast/seq_len_results.eps}
    %\caption{F1 vs. sliding window size}
    \caption{F1* vs. sequence length}
        \label{fig: seq_len_results}
\end{subfigure}
\begin{subfigure}[b]{.32\linewidth}
    \centering
    \includegraphics[height=2.5cm]{figures/neural_contrast/win_size_results.eps} 
    \caption{F1* vs. prediction window}
    \label{fig: win_size_results}
\end{subfigure}
\begin{subfigure}[b]{.32\linewidth}
    \centering
    \includegraphics[height=2.5cm]{figures/neural_contrast/n_transformations_results.eps} 
    \caption{F1* vs. transformations}
    \label{fig: n_transformations_results}
\end{subfigure}
\caption{(a) F1* versus sliding window size $w$ from 20 to 70; (b) F1* versus prediction window size $p$ from 1 to 9; (c) F1* versus number of transformations $K$ from 4 to 12.}
\label{fig: sensitivity_results}
\end{figure*}
\subsection{Sensitivity of Hyper-parameters}

In this section we conduct the sensitivity analysis on three hyper-parameters, the sizes of the sliding window $w$, the prediction window $p$, and the number of transformations $K$, with each parameter setting result averaged over 5 runs. Figure~\ref{fig: seq_len_results} illustrates the F1* score’s correlation with the sliding window size, with the prediction window size held constant at 5. We can see a relatively higher performance when the sequence length lies below 60. This finding is consistent with the performance of the majority of other baseline models, which also obtain optimal performances by adopting a sequence length within this range. Figure~\ref{fig: win_size_results} explores the F1* score’s variability in response to different prediction window sizes, while maintaining the sliding window size as default. The model exhibits relatively stable performance across different window sizes. Figure~\ref{fig: n_transformations_results} portrays the F1* score's responsiveness to varying numbers of transformations. The optimal performance for different datasets are also different. For example, the peak performance for SMAP is when $K=10$, while the one for MSL is when $K=6$. Overall, the performance appears relatively stable across the number of transformations.



% \subsection{Computational Analysis}
% \label{sec: computation analysis}
% \begin{figure}[t!]
% \centering
% %\vspace{-0.2cm}
% \includesvg[width=0.7\linewidth]{figures/neural_contrast/computation_time.svg}
% \caption{The training time per epoch and inference time of each model based on the SWaT dataset.}
% \label{fig: computation_time}
% \end{figure}
% Figure~\ref{fig: computation_time} provides a comparison of the computational demands for various models, including both training time per epoch and inference time, benchmarked on the SWaT dataset. To ensure consistency across models, we maintained the same batch size during the training and testing phases. CNT demonstrates a considerable reduction in both training and inference times relative to other models, particularly NeutralAD. The efficiency of CNT can be attributed to its approach of applying transformations to the hidden representations - outputs of a feature encoder - rather than operating directly on the input data. This design choice means that CNT requires only a single pass of the data through the feature encoder, irrespective of the number of transformations applied, in stark contrast to NeutralAD, which must repeatedly process the input data for each transformation, incurring high computational overhead. Additionally, the observed computational efficiency in models like USAD, DeepSVDD, and DAGMM can be rationalized by their reliance on simpler MLP-based feature encoders, which are inherently less computationally intensive than more complex architectures.





==> subtexes/experiments_v2.tex <==
%\section{Experiment}
\subsection{Datasets}
\begin{table}[H]
\small
    %\setlength{\abovecaptionskip}{0cm}
    %\setlength{\belowcaptionskip}{-0.1cm}
    \centering
    \caption{Summary statistics for datasets} 
    \vspace{-0,3cm}
    \begin{tabular}{ccccc}\\ \toprule
               \textbf{Dataset} & \textbf{\# Channels} & \textbf{\# training} & \textbf{\# test} & \textbf{\% anomalies} \\ \midrule
   SWaT  &  51         &  495000   & 449919 & 12.14      \\
   WADI       &  123         &  784571    & 172801 & 5.77     \\  
%         SMAP       &   25        & 135183 & 427617 & 12.79     \\  

      MSL       &   55        & 58317 & 73729 & 10.53     \\
%    SMD       & 38         &  25300   & 25300 & 4.21    \\  

   HAI       & 79         &  921603   & 270003 & 1.93    \\  
%    TODS  & 1   & 40000 & 20000 & 2.50 \\
   \bottomrule
    \end{tabular}
    \label{tab:data_statistics}
    %\vspace{-0.8cm}
\end{table}
Four industrial real-world datasets, as shown in Table~\ref{tab:data_statistics},  are adopted for the evaluation of time series anomaly detection methods, which are SWaT~\cite{mathur2016swat}, WADI~\cite{ahmed2017wadi}, HAI~\cite{hai21.03}, and MSL~\cite{lstm-ndt}. Each dataset has a unlabeled training set, and a separate test set with anomalies. SWaT and WADI are released by iTrust Center~\footnote{\url{https://itrust.sutd.edu.sg/itrust-labs_datasets/dataset_info/}} to support research in cybersecurity. The SWaT dataset is collected from a scaled-down, secure water treatment testbed, featuring a 51-dimensional multivariate time series from 11 days of continuous operation. The first 7 days reflect normal operations (training set) and the last 4 days contain cyber attack data (test set). Similarly, the WADI dataset, collected from a small-scale water distribution network, includes 123 sensor and actuator time series from a 16-day run, with normal operations in the first 14 days (training set) and cyber attacks in the last 2 (test set). HAI dataset derives from an Industrial Control System testbed enriched with a Hardware-In-the-Loop simulator, featuring processes like boiler, turbine, water treatment, and steam-turbine power generation. As a common pre-processing step similar to~\cite{gdn}, the training and test sets of the above three datasets have been down-sampled to 10-second intervals using median values with anomaly labels assigned 0 or 1 by taking the mode. MSL, published by NASA, contains telemetry anomaly data from Mars Science Laboratory rover. The data contains multiple entities, which are concatenated into one time series for both training and testing.
% HAI contains three entities with each as a 79-dimensional multivariate time series. We train them separately and the performances are averaged over the three entities.


\begin{table*}[t!]
%\small
    \setlength{\abovecaptionskip}{0cm}
    %\setlength{\belowcaptionskip}{-0.1cm}
    \centering
        % \caption{Performance comparison (F1-scores (\%)) on real-world datasets. The best performance is highlighted in bold.} 
        \caption{Performance comparison (F1 (\%)) on the benchmark datasets, precision (Pre (\%)) and recall (Rec (\%)) are attached. }
    %\begin{adjustbox}{width=\columnwidth,center}
    %\setlength{\tabcolsep}{1.68mm}{
    \begin{tabular}{cccccccccccccc}\\ \toprule
               &   \multicolumn{3}{c}{\textbf{SWaT}} & \multicolumn{3}{c}{\textbf{WADI}} & \multicolumn{3}{c}{\textbf{HAI}} & \multicolumn{3}{c}{\textbf{MSL}} \\ \midrule
               \textbf{Methods} & \textbf{F1} &  \textbf{Pre} & \textbf{Rec} & \textbf{F1} &  \textbf{Pre} & \textbf{Rec} & \textbf{F1} &  \textbf{Pre} & \textbf{Rec}  & \textbf{F1} &  \textbf{Pre} & \textbf{Rec}    \\ \midrule
DAGMM              &  70.17 &  69.96 &  77.07 &  43.68 &  53.50 &  38.42 &  34.95 &  43.81 &  39.21 &  80.96 &  76.96 &  85.73 \\
DeepSVDD           &  86.41 &  96.68 &  78.16 &  45.37 &  77.44 &  34.30 &  35.36 &  31.08 &  50.39 &  81.03 &  76.99 &  86.87 \\
LSTM-VAE           &  81.90 &  97.95 &  70.42 &  64.70 &  66.53 &  62.99 &  69.41 &  64.90 &  77.46 &  88.40 &  87.55 &  89.70 \\
USAD               &  84.60 &  \textbf{98.70} &  74.02 &  61.74 &  84.49 &  48.65 &  74.93 &  83.48 &  68.43 &  92.72 &  88.10 &  \textbf{97.86} \\
MAD-GAN            &  80.44 &  97.31 &  68.77 &  74.09 &  \textbf{90.23} &  62.96 &  20.94 &  29.06 &  37.45 &  76.45 &  80.66 &  76.55 \\
MTAD-GAT           &  84.53 &  94.01 &  76.95 &  51.02 &  63.54 &  43.03 &  80.95 &  88.43 &  76.56 &  90.13 &	89.06	&91.23 \\
TranAD             &  83.17 &  97.39 &  72.61 &  41.05 &  69.83 &  29.91 &  73.93 &  \textbf{88.60} &  64.70 &  91.55 &  90.41 &  92.73 \\
LNT                &  86.36 &  94.95 &  79.34 &  35.55 &  74.20 &  24.77 &  54.43 &  72.23 &  48.51 &  90.50 &  91.28 &  89.84 \\
AnomalyTrans &  91.34 &  91.87 &  \textbf{90.82} &  69.00 &  75.41 &  63.59 &  58.02 &  63.33 &  55.26 &  93.97 &  92.75 &  95.25 \\
\midrule
CNT &  \textbf{91.68} & 96.50 & 87.33 &  \textbf{81.61}	& 82.39	& \textbf{81.19}   & \textbf{83.95} & 81.48 & \textbf{87.75} &  \textbf{95.13}&	\textbf{96.06}&	94.26 \\
   \bottomrule
    \end{tabular}
    %}
    %\end{adjustbox}
    \label{tab:comparison_result_f1}
    %\vspace{-0.8cm}
\end{table*}


% \begin{table*}[t!]
% %\small
%     \setlength{\abovecaptionskip}{0cm}
%     \centering
%         \caption{Performance comparison (VUS\_ROC (\%), VUS\_PR (\%)) on the benchmark datasets.}
%     \begin{tabular}{ccccccccc}\\ \toprule
%                &   \multicolumn{2}{c}{\textbf{SWaT}} & \multicolumn{2}{c}{\textbf{WADI}} & \multicolumn{2}{c}{\textbf{HAI}} & \multicolumn{2}{c}{\textbf{MSL}} \\ \midrule
%                \textbf{\textbf{Methods}}  & \textbf{VUS\_PR} & \textbf{VUS\_ROC}  & \textbf{VUS\_PR} & \textbf{VUS\_ROC} & \textbf{VUS\_PR} & \textbf{VUS\_ROC} & \textbf{VUS\_PR} & \textbf{VUS\_ROC}   \\ \midrule
% % DAGMM              &  43.02 &   63.80 &  20.88 &   57.85 &  18.95 &   66.50 &  15.22 &   58.76 \\
% % DeepSVDD           &  57.83 &   \textbf{84.37} &  26.60 &   54.66 &  25.01 &   74.93 &  19.71 &   66.50 \\
% LSTM-VAE           &  50.91 &   72.73 &  34.23 &   68.84 &  21.27 &   69.08 &  17.15 &   61.12 \\
% USAD               &  42.10 &   60.88 &  16.56 &   52.44 &  21.34 &   64.42 &  18.41 &   55.59 \\
% MAD-GAN            &  49.98 &   74.63 &  18.51 &   60.03 &  12.62 &   63.90 &  14.45 &   55.32 \\
% MTAD-GAT           &  49.06 &   67.24 &  22.12 &   62.97 &  27.31 &   71.09 &  19.83 &   65.60 \\
% TranAD             &  41.43 &   61.17 &  19.42 &   56.03 &  26.79 &   72.57 &  \textbf{31.84} &   67.00 \\
% LNT                &  54.73 &   \textbf{76.12} &  18.18 &   50.58 &  20.40 &   74.72 &  16.75 &   57.11 \\
% AnomalyTransformer &  20.22 &   53.24 &  10.72 &   51.64 &  12.38 &   54.16 &  14.33 &   51.39 \\


% \midrule
% CNT               &  \textbf{59.76} &   74.25 & \textbf{39.79} &   \textbf{78.38} &  \textbf{46.88} &   \textbf{85.64} &  23.87 &   \textbf{69.84} \\ 
%    \bottomrule
%     \end{tabular}
%     %}
%     %\end{adjustbox}
%     \label{tab:comparison_result_vus}
%     %\vspace{-0.8cm}
% \end{table*}


\subsection{Experimental Setup}
Our model is trained with an Adam optimizer~\cite{kingma2014adam} at a learning rate of 0.001 for 30 epochs. The 20$\%$ of the training set is selected as a validation set where the best epoch is stored based on the validation loss. Note that each input sample is a consecutive time window as stated in Section~\ref{sec: problem formulation}. We employ early stopping with a patience of 10 epochs. The hidden dimension $d$ is set to 64, and the maximum number of TCN blocks is set to 8. The temperature $\tau$ and the number of transformations $K$ for DCL loss are set to 0.1 and 6, respectively. The sequence length is set to 30 and the predict window size $w$ is set to 5. In addition, all performance results are averaged over five independent runs.
%The sequence length $l$ is 30 for SWaT and MSL, and 50 for WADI, HAI, SMAP respectively. 



\subsection{Baseline Methods and Evaluation Metrics}
We compare our framework with common anomaly detection approaches as the baseline methods, including Deep SVDD~\cite{deepSVDD} and DAGMM~\cite{zong2018deep}, which are general anomaly detection deep learning-based models, and LSTM-VAE~\cite{lstm-vae}, MAD-GAN~\cite{mad-gan}, USAD~\cite{usad}, MTAD-GAT~\cite{mtad-gat}, LNT~\cite{lnt}, TranAD~\cite{tranAD}, and AnomalyTransformer~\cite{anomalyTransformer}, which are state-of-the-art anomaly detection methods tailored specifically to time series data.

In line with previous studies~\cite{mtad-gat,omnianomaly,anomalyTransformer,tranAD}, we use F1-score as the main performance metric to evaluate the performance of anomaly detection, with the threshold for each model chosen as the one which achieves the best F1 over the test sets. In addition, we follow the point-adjusting strategy suggested in \cite{omnianomaly}, which labels a whole anomaly segment as 1 as long as one of the points within the segment is detected as an anomaly. Since our primary contribution is not the development of a new thresholding method, we adopt this well-established practice to eliminate potential bias arising from selecting a specific thresholding method. This choice of reporting F1 scores ensures a fair and consistent comparison across all methods. 

% Additionally, we provide the performance comparison based on two recent proposed metrics VUS-ROC and VUS-PR in~\cite{paparrizos2022volume}, which avoid the need to compute threshold and incorporate the concept of buffer regions that are designed for range-based contextual anomalies (anomaly event). Specifically, VUS\-ROC is the volume under the surfaces created based on ROC curve which is calculated by taking anomaly event into consideration, while VUS\-PR is the volume under the surfaces created based on PR curve. We think different evaluation metrics provide different views.
% We also present a performance comparison using two recently introduced metrics: VUS-ROC and VUS-PR, as detailed in \cite{paparrizos2022volume}. These metrics are designed to adapt traditional ROC and PR curves for time series anomalies, which tend to occur in consecutive sequences. Specifically, VUS-ROC measures the volume under the surfaces of the ROC curve while accounting for these consecutive anomaly sequences. In contrast, VUS-PR calculates the volume under the surfaces based on the PR curve. 

\subsection{Comparison Study}
The results are presented in Table~\ref{tab:comparison_result_f1}. First, both DAGMM and DeepSVDD display the lowest average performance among all models, likely due to their architectural design which does not account for temporal information. On the other hand, models such as MTAD-GAT and AnomalyTransformer perform comparatively better across all datasets in terms of F1 score, a testament to their effective utilization of GNNs to capture inter-series relationships or the global characteristics of time series through Transformers. Yet, CNT outperforms all others with the highest F1 score across all datasets, thus demonstrating the best balance between Recall and Precision. In comparison to these approaches, which utilize either time series forecasting or reconstruction-based methods, our approach utilizes the distance of latent representation between input instance and their contextual information as a criterion to identify anomalies, which are more robust to noise and less likely to overfit the data.

On the other hand, LNT, which is closest to ours, showed inferior performance compared to our approach. LNT fuses CPC loss with the objective of neural transformation learning, necessitating the selection of negative samples during the training stage. Since the majority of these negative samples are normal - as most samples in the training datasets are normal - this can introduce additional bias during the training process. To circumvent this, our approach applies a negative-free training scheme, with the representation collapse problem mitigated by incorporating the discriminative contrastive loss. 
% Both the sequence-level contrasting objective and the neural transformation learning objective can effectively collaborate to enhance anomaly detection performance. 

% Furthermore, we assessed model performance using VUS\_PR and VUS\_ROC metrics on recent state-of-the-art time series models. While the ranking of all models slightly shifts compared to the F1 score, our approach still maintains consistently high performance across the majority of datasets. (need to be modified)
%only falling behind TranAD on MSL datasets and LNT on SWaT. 

% This outcome could be attributed to our use of the TCN encoder, which may be less capable of capturing global characteristics compared to the Transformer used in TranAD. As such, the design of a more effective base feature encoder is a direction for our future research.

% This could be attributed to its strategy of minimizing the distance between the transformations of point-wise future predictions and the context window, a method that may fail to preserve identical semantic meanings. Conversely, our model leverages a sequence-to-sequence comparison where the suspect and context sequences share semantically meaningful features owing to their overlap and shared feature encoder.


% our model achieves the highest F1 for all datasets. In addition, Precision and Recall are also on average within the top 3. We also compare the performance based on recently proposed metrics, VUS\-ROC and VUS\-PR for the recent state-of-the-art methods, and the results show that our model outperforms them in the majority datasets while slightly falling behind LNT in terms of VUS\_ROC for swat.
% % However, our model's performance falls short on MSL and SMAP. This could be due to the majority of features in these datasets being one-hot encoded commands, making temporal encoding of sequences challenging for simple TCN layers that tend to mix all features through simple sum aggregation. On the other hand, graph-based models like GDN, which explicitly learn the relationship between features, have performed well on these datasets.

% Additionally, NCAD currently holds state-of-the-arts performance on MSL and SMAP due to its semi-supervised classification training schemes based on synthetic anomalies. While supervised training is known to be more effective when the underlying distribution of synthetic anomalies is similar to that of the true anomalies in the dataset, we can see that NCAD performed relatively worse in WADI, HAI, and SMD compared to our methods, suggesting potential overfitting due to these datasets having a variety of different anomaly types beyond the injected ones.

% ON the other hand, LNT, a similar model to ours, showed inferior performance compared to our model, possibly because it attempts to minimize the distance between the transformation of point-wise future predictions and the context window, which may not have identical semantic meanings. In contrast, our model employs a sequence-to-sequence comparison, where the suspect and context sequences share semantically meaningful features due to their overlap and shared feature encoder.


\subsection{Ablation Study}
\label{section: ablation}
In this section, we compare different possible variants of our proposed framework, with the details presented as follows: 
(1) CCL: Here, $g(\cdot)$ is trained exclusively under the contextual contrastive loss in Eq.~\eqref{eq. raw contextual one-class objective}.
(2) CCL + Vicreg: Similar to~\cite{vicreg}, $g(\cdot)$ is trained under the contextual contrastive loss, supplemented with a regularization term to ensure non-zero variance of the latent representations within a batch, thereby ensuring non-constant encoder outputs:
\begin{align}
    &L_{\text{ccl+vicreg}} = L_{\text{ccl}} + v(\{S^{t}\}_{t\in B}) + v(\{C^{t}\}_{t\in B}) \\
    & v(\{S^{t}\}_{t \in B}) = \frac{1}{d} \sum_{j=1}^d \max(0, \gamma - \sqrt{\text{Var}(\{g(S^t)_j\}_{t \in B}) + \epsilon}) \label{eq: regularization on ccl}
\end{align}
where $B$ denotes an arbitrary mini-batch of samples containing $X^t$, $\gamma$ is set to 1 as in~\cite{vicreg}, and $\epsilon$ is a small scaler value to prevent numerical instabilities. The variance in Eq.\eqref{eq: regularization on ccl} is computed over the encoder outputs within the batch $B$. During inference, only $L_{\text{ccl}}$ is used as the anomaly score. 
(3) CCL+Simsiam: Following ~\cite{simsiam}, we create unique feature encoders for the predict and context sequences, and compute two CCL losses. Each loss applies the stopping criterion on the representation of one sequence, with the other remaining detached. During inference, the sum of the two losses serves as the anomaly scores. The essential idea of this setting is to incorporate continuous target changes in order to prevent constant encoder solutions.
(4) DCL: The feature encoder network $g(\cdot)$ is trained purely under the discriminative contrastive loss in Eq.\eqref{eq. contextual discriminative contrastive loss}. It's akin to the approach in~\cite{neuralAD}, but transformations are applied to the feature encoder output rather than the original sequence. 

% The DCL setting processes features across a full sliding window, which may overlook anomalies using the loss at a single time step $t$. Thus, we aggregate scores over the entire window to determine the anomaly score for each $t$.



% /
\begin{table}[t!]
%\small
    \setlength{\abovecaptionskip}{0cm}
    %\setlength{\belowcaptionskip}{-0.1cm}
    \centering
    \caption{Performance comparison (F1 (\%)) for our method against different model variants.} 
    \begin{tabular}{ccccccc}\\ \toprule
     \textbf{Settings} & \textbf{SWaT} & \textbf{WADI}  & \textbf{HAI} & \textbf{MSL} & \textbf{Avg.}  \\ \midrule
  % Default             &  91.99     &  \\ \midrule
CNT    & 91.68 & \textbf{81.61} & \textbf{83.95} & \textbf{95.13}  & \textbf{88.10} \\ \midrule
DCL      & 85.06 & 30.36 & 67.50 & 81.21 & 66.03\\
CCL      & 88.01 & 66.22 & 64.24 & 91.49 & 77.49\\
CCL+Vicreg  & 89.00 & 54.33 & 50.29 & 87.50 & 70.28\\
CCL+Simsiam & \textbf{91.82}	&66.33	&78.26&	92.69 & 82.28 \\ 
   \bottomrule
    \end{tabular}
    \label{tab:ablation_result}
    %\vspace{-0.8cm}
\end{table}

\begin{figure}[t]
    \centering
   % \includesvg[width=1\linewidth]{figures/Framework.svg}
        \includesvg[height=6.5cm]{figures/neural_contrast/showcases_tods.svg}
        % \includegraphics[height=8cm, width=11.5cm]{figures/neural_contrast/showcases_tods.svg}

        \caption{The above figure showcases various types of anomalies present in the TODS dataset alongside the corresponding anomaly scores generated by our proposed method, as well as the other settings from Section~\ref{section: ablation}. The red lines denote the threshold values beyond which anomalies will be identified under different settings.}
    \label{fig: tods showcase}
%\vspace{0.5cm}
\end{figure}

Table~\ref{tab:ablation_result} presents the results of our experiments. First, the CCL setting is designed to assign similar representations to normal sequences in close proximity, but its performance falls short in comparison to our proposed approach. This can potentially be attributed to the representation collapse problem, wherein the loss function leads the encoder to converge to a parameter space that closely approximates the constant encoder solution. Consequently, the model may fail to capture the rich semantic information of normal sequences. 

The goal of the CCL+Vicreg and CCL+Siamsam settings, the direct variants of the CCL setting, aim to prevent the representation collapse issue. Yet, our model still surpasses them on average across datasets. Distinguished from these two configurations, our framework's incorporation of DCL loss ensures not only non-constant latent representations but also compels transformations of the predict sequences to stay semantically akin to original sequences. This provides a diverse range of perspectives on sequence normality and enables multi-angular similarity measurement between sequences.

% The CCL+Vicreg and CCL+Siamsam configurations, direct offshoots of the CCL model, aim to avert representation collapse. Yet, our model consistently surpasses them across datasets. Distinguished from these two configurations, our framework's incorporation of DCL loss ensures not only non-constant latent representations but also compels transformations of suspect sequences to stay semantically akin to original sequences. This provides a diverse range of perspectives on sequence normality and enables multi-angular similarity measurement between sequences.


% An alternative explanation for our improved performance over CCL is that the combination of DCL and CCL losses facilitates contextual contrastion between various transformed versions of the predict and context sequences, thereby providing diverse perspectives on the normality of the sequences and allowing the measurement of similarity between two sequences from multiple angles.

% The above argument can be further inferred from the performance of the CCL+Vicreg setting, wherein the addition of a variance regularization term to enforce non-constant latent representations among training samples does not outperform our default setting, and even performs worse than the CCL setting for certain datasets. In comparison to CCL+Vicreg setting, the CCL+Simsiam setting has relatively better performance, It's core idea is to make a continuous change in targets in order to prevent the model from collapsing to trivial solutions In comparison to the above two settings, the incorporation of DCL loss in our framework not only increases the diversity of the latent representations and prevent mode collapse, but also effectively forces the transformations of suspect sequences to be semantically similar to the original sequences, which forces the network to learn high level semantics. 




% \begin{figure*}[t!]
% \centering
% \begin{minipage}[b]{1\linewidth}
% %\vspace{-0.2cm}
% \begin{subfigure}[b]{1\linewidth}
%     \centering
%      % \includesvg[height=4.2cm]{figures/swat_ts_unidentified_event1.svg}
%     \includegraphics[height=0.5cm]{figures/neural_contrast/legend.eps}
%     %\caption{}
%    % \label{fig: win_size_results}
% \end{subfigure}
% \newline
% %\vspace{0.5cm}
% \centering
% \begin{subfigure}[b]{.33\linewidth}
%     \centering
%     \includegraphics[height=2cm]{figures/neural_contrast/seq_len_results.eps}
%     %\caption{F1 vs. sliding window size}
%     \label{fig: seq_len_results}
% \end{subfigure}
% \begin{subfigure}[b]{.33\linewidth}
%     \centering
%     \includegraphics[height=2cm]{figures/neural_contrast/win_size_results.eps} 
%     %\caption{F1 vs. predict window size}
%     \label{fig: win_size_results}
% \end{subfigure}
% \begin{subfigure}[b]{.33\linewidth}
%     \centering
%     \includegraphics[height=2cm]{figures/neural_contrast/n_transformations_results.eps} 
%     %\caption{F1 vs. \# transformations}
%     \label{fig: n_transformations_results}
% \end{subfigure}
% \end{minipage}
% % \hfill
% % \begin{minipage}[b]{0.46\linewidth}
% %     \begin{subfigure}[b]{1\linewidth}
% %     \centering
% % \includesvg[height=3.3cm]{figures/neural_contrast/computation_time.svg}
% % %\captionsetup[figure]{justification=centering}
% % \caption{Training/Inference time}
% % \label{fig: computation_time}
% % \end{subfigure}
% %\end{minipage}
% \caption{(a) Average F1 versus sliding window size $w$ from 20 to 100; (b) Average F1 versus predict window size $p$ from 1 to 11; (c) The training time per epoch and inference time of each model based on the SWaT dataset.}
% \label{fig: sensitivity_results}
% \end{figure*}

Lastly, The DCL configuration primarily encourages similarity between an input time window and its corresponding transformed sequences, prioritizing the modeling of characteristics across the entire time window. Consequently, anomalies within short time spans may be overlooked, resulting in negligible distance scores between the time window and its transformations, particularly for longer time windows. In contrast, our default setting emphasizes the discrepancy between the predict window and the context window, thereby enhancing accurate anomaly detection within the overlapping region.







\subsection{Data Visualization}

% To evaluate the effectiveness of our proposed framework in capturing contextual characteristics of anomalies in time series data, we conducted experiments on a univariate dataset (TODS) generated from rules outlined in \cite{tods}. The data adopts sinusoidal wave as the base shapelet to generate a univariate time series, with synthetic anomalies of various types injected, such as point anomalies, trend anomalies, seasonal anomalies, and pattern-wise anomalies (Examples of different types of anomalies are shown in Figure~\ref{fig: tods showcase}, and summary statistics of the data is shown in Table~\ref{tab:data_statistics}). We choose TODS specifically for data visualization as it offers clearly classified anomalies of different types, allowing for a better understanding of the performance of our model. Furthermore, the univariate nature of the dataset makes it easy to visualize the results directly from the plot. 

We further conducted experiments on a univariate dataset (TODS) generated from the rules outlined in~\cite{tods}. The TODS dataset adopts a sinusoidal wave as the base shapelet to generate a univariate time series, and synthetic anomalies of various types are injected using predefined rules. Examples of different types of anomalies are shown in Figure~\ref{fig: tods showcase}. TODS is specifically chosen for data visualization as it offers clearly classified anomalies of different types, enabling a better understanding of the performance of our method. Furthermore, the univariate nature of the dataset makes it easy to visualize the results directly from the plot.
% , and summary statistics of the data are shown in Table~\ref{tab:data_statistics}


We trained our model with all settings as in the previous Section. Figure \ref{fig: tods showcase} presents several showcases of different anomaly types, demonstrating the effectiveness of our proposed framework in identifying contextual anomalies. We observe that while global point anomalies are easily identifiable by all methods, the other model variants show relatively weaker performance in detecting other anomaly types that strongly rely on contextual information. In contrast, our proposed method is capable of effectively identifying hard anomalies by leveraging the deviation between the predict and context window through contrastive learning. This approach enables our method to be more sensitive to drastic changes in local context information.

\subsection{Sensitivity of Hyper-parameters}
In this section we conduct the sensitivity analysis on three hyper-parameters, the sizes of the sliding window $w$, the predict window $p$, and the number of transformations $K$, based on SWaT and MSL datasets with each parameter setting result averaged over 5 runs. Figure~\ref{fig: sensitivity_results}a illustrates the F1 score’s correlation with the sliding window size, with the predict window size held constant at 5. We can see a relatively higher performance when the sequence length lies between 20 and 60. This finding is consistent with the performance of other baseline models (e.g., TranAD, MTAD-GAT, and LNT), which also obtain optimal performances by adopting a sequence length within this range. Figure~\ref{fig: sensitivity_results}b explores the F1 score’s variability in response to different predict window sizes, while maintaining the sliding window size at 30. The model exhibits peak performance for prediction window sizes between 3 and 5 and experiences a noticeable decline when the size exceeds 9. This trend is logical, as larger prediction window sizes can smooth out the effect of anomalies (Most anomalies in the benchmark datasets are short-lived), reducing their distinctiveness from normal sample scores. Figure~\ref{fig: sensitivity_results}c portrays the F1 score's responsiveness to varying numbers of transformations. The optimal performance is observed at approximately $K=6$, with some performance fluctuations across other values. In our experiments, the hyperparameters $p$, $w$, and $K$ were set to 5, 30, and 6 respectively for all datasets, informed by the validation set loss. While this strategy may not ensure optimal performance across all datasets, it yields satisfactorily robust results. 
\begin{figure*}[t!]
%\centering
% \begin{subfigure}[b]{1\linewidth}
%     \centering
%      % \includesvg[height=4.2cm]{figures/swat_ts_unidentified_event1.svg}
%     \includegraphics[height=0.5cm]{figures/neural_contrast/legend.eps}
%     %\caption{}
%    % \label{fig: win_size_results}
% \end{subfigure}
%\newline
%\vspace{0.5cm}
%\centering
\begin{subfigure}[b]{.32\linewidth}
    \centering
    \includegraphics[height=2.4cm]{figures/neural_contrast/seq_len_results.eps}
    %\caption{F1 vs. sliding window size}
    \label{fig: seq_len_results}
\end{subfigure}
\begin{subfigure}[b]{.32\linewidth}
    \centering
    \includegraphics[height=2.4cm]{figures/neural_contrast/win_size_results.eps} 
    %\caption{F1 vs. predict window size}
    \label{fig: win_size_results}
\end{subfigure}
\begin{subfigure}[b]{.32\linewidth}
    \centering
    \includegraphics[height=2.4cm]{figures/neural_contrast/n_transformations_results.eps} 
    %\caption{F1 vs. \# transformations}
    \label{fig: n_transformations_results}
\end{subfigure}
\caption{(a) Average F1 versus sliding window size $w$ from 20 to 100; (b) Average F1 versus predict window size $p$ from 1 to 11; (c) Average F1 versus number of transformations $K$ from 2 to 12.}
\label{fig: sensitivity_results}
\end{figure*}

\subsection{Computational Analysis}
Figure~\ref{fig: computation_time} illustrates the training time per epoch and inference time of the training and test datasets based on SWaT for each model, measured in seconds. CNT demonstrates a relatively lower training and inference time compared to other models. In contrast to LNT, which necessitates the computation of distance between the $k$-step ahead time series value and their contextual window, our approach significantly enhances computational efficiency by employing sequence-to-sequence contrastive learning. Furthermore, the base architecture of our method is TCN, inherently a more lightweight design compared to those based on RNN or Transformer architectures.

% \begin{figure}[t!]
% \centering
% %\vspace{-0.2cm}
% \includesvg[height=3.5cm]{figures/neural_contrast/computation_time.svg}

% \caption{The training time per epoch and inference time of each model based on the SWaT dataset.}
% \label{fig: computation_time}
% \end{figure}


==> subtexes/experiments_v3.tex <==
%\section{Experiment}
\subsection{Datasets}
\begin{table}[H]
    \vspace{-0.8cm}
%\small
    %\setlength{\abovecaptionskip}{0cm}
    %\setlength{\belowcaptionskip}{-0.1cm}
    \centering
    \caption{Summary statistics for datasets} 
    \begin{tabular}{ccccc}\\ \toprule
               \textbf{Dataset} & \textbf{\# Channels} & \textbf{\# training} & \textbf{\# test} & \textbf{\% anomalies} \\ \midrule
   SWaT  &  51         &  495000   & 449919 & 12.14      \\
   WADI       &  123         &  784571    & 172801 & 5.77     \\  
%         SMAP       &   25        & 135183 & 427617 & 12.79     \\  

      MSL       &   55        & 58317 & 73729 & 10.53     \\
%    SMD       & 38         &  25300   & 25300 & 4.21    \\  

   HAI       & 79         &  921603   & 270003 & 1.93    \\  
%    TODS  & 1   & 40000 & 20000 & 2.50 \\
   \bottomrule
    \end{tabular}
    \label{tab:data_statistics}
    %\vspace{-0.8cm}
\end{table}
Four industrial real-world datasets, as shown in Table~\ref{tab:data_statistics},  are adopted for the evaluation of time series anomaly detection methods, which are SWaT~\cite{mathur2016swat}, WADI~\cite{ahmed2017wadi}, HAI~\cite{hai21.03}, and MSL~\cite{lstm-ndt}. Each dataset has a unlabeled training set, and a separate test set with anomalies. SWaT and WADI are released by iTrust Center~\footnote{\url{https://itrust.sutd.edu.sg/itrust-labs_datasets/dataset_info/}} to support research in cybersecurity. The SWaT dataset is collected from a scaled-down, secure water treatment testbed, featuring a 51-dimensional multivariate time series from 11 days of continuous operation. The first 7 days reflect normal operations (training set) and the last 4 days contain cyber attack data (test set). Similarly, the WADI dataset, collected from a small-scale water distribution network, includes 123 sensor and actuator time series from a 16-day run, with normal operations in the first 14 days (training set) and cyber attacks in the last 2 (test set). HAI dataset derives from an Industrial Control System testbed enriched with a Hardware-In-the-Loop simulator, featuring processes like boiler, turbine, water treatment, and steam-turbine power generation. As a common pre-processing step similar to~\cite{gdn}, the training and test sets of the above three datasets have been down-sampled to 10-second intervals using median values with anomaly labels assigned 0 or 1 by taking the mode. MSL, published by NASA, contains telemetry anomaly data from Mars Science Laboratory rover. The data contains multiple entities, which are concatenated into one time series for both training and testing.
% HAI contains three entities with each as a 79-dimensional multivariate time series. We train them separately and the performances are averaged over the three entities.


% \begin{table*}[t!]
% %\small
%     \setlength{\abovecaptionskip}{0cm}
%     \centering
%         \caption{Performance comparison (VUS\_ROC (\%), VUS\_PR (\%)) on the benchmark datasets.}
%     \begin{tabular}{ccccccccc}\\ \toprule
%                &   \multicolumn{2}{c}{\textbf{SWaT}} & \multicolumn{2}{c}{\textbf{WADI}} & \multicolumn{2}{c}{\textbf{HAI}} & \multicolumn{2}{c}{\textbf{MSL}} \\ \midrule
%                \textbf{\textbf{Methods}}  & \textbf{VUS\_PR} & \textbf{VUS\_ROC}  & \textbf{VUS\_PR} & \textbf{VUS\_ROC} & \textbf{VUS\_PR} & \textbf{VUS\_ROC} & \textbf{VUS\_PR} & \textbf{VUS\_ROC}   \\ \midrule
% % DAGMM              &  43.02 &   63.80 &  20.88 &   57.85 &  18.95 &   66.50 &  15.22 &   58.76 \\
% % DeepSVDD           &  57.83 &   \textbf{84.37} &  26.60 &   54.66 &  25.01 &   74.93 &  19.71 &   66.50 \\
% LSTM-VAE           &  50.91 &   72.73 &  34.23 &   68.84 &  21.27 &   69.08 &  17.15 &   61.12 \\
% USAD               &  42.10 &   60.88 &  16.56 &   52.44 &  21.34 &   64.42 &  18.41 &   55.59 \\
% MAD-GAN            &  49.98 &   74.63 &  18.51 &   60.03 &  12.62 &   63.90 &  14.45 &   55.32 \\
% MTAD-GAT           &  49.06 &   67.24 &  22.12 &   62.97 &  27.31 &   71.09 &  19.83 &   65.60 \\
% TranAD             &  41.43 &   61.17 &  19.42 &   56.03 &  26.79 &   72.57 &  \textbf{31.84} &   67.00 \\
% LNT                &  54.73 &   \textbf{76.12} &  18.18 &   50.58 &  20.40 &   74.72 &  16.75 &   57.11 \\
% AnomalyTransformer &  20.22 &   53.24 &  10.72 &   51.64 &  12.38 &   54.16 &  14.33 &   51.39 \\


% \midrule
% CNT               &  \textbf{59.76} &   74.25 & \textbf{39.79} &   \textbf{78.38} &  \textbf{46.88} &   \textbf{85.64} &  23.87 &   \textbf{69.84} \\ 
%    \bottomrule
%     \end{tabular}
%     %}
%     %\end{adjustbox}
%     \label{tab:comparison_result_vus}
%     %\vspace{-0.8cm}
% \end{table*}


\subsection{Experimental Setup}
Our model is trained with an Adam optimizer~\cite{kingma2014adam} at a learning rate of 0.001 for 30 epochs. The 20$\%$ of the training set is selected as a validation set where the best epoch is stored based on the validation loss. Note that each input sample is a consecutive time window as stated in Section~\ref{sec: problem formulation}. We employ early stopping with a patience of 10 epochs. The hidden dimension $d$ is set to 64, and the maximum number of TCN blocks is set to 8. The temperature $\tau$ and the number of transformations $K$ for DCL loss are set to 0.1 and 6, respectively. The sequence length is set to 30 and the predict window size $w$ is set to 5. In addition, all performance results are averaged over five independent runs.
%The sequence length $l$ is 30 for SWaT and MSL, and 50 for WADI, HAI, SMAP respectively. 



\subsection{Baseline Methods and Evaluation Metrics}
We compare our framework with common anomaly detection approaches as the baseline methods, including Deep SVDD~\cite{deepSVDD} and DAGMM~\cite{zong2018deep}, which are general anomaly detection deep learning-based models, and LSTM-VAE~\cite{lstm-vae}, MAD-GAN~\cite{mad-gan}, USAD~\cite{usad}, MTAD-GAT~\cite{mtad-gat}, LNT~\cite{lnt}, TranAD~\cite{tranAD}, NeuTralAD~\cite{neuralAD} and AnomalyTransformer~\cite{anomalyTransformer}, which are state-of-the-art anomaly detection methods tailored specifically to time series data.

In line with previous studies~\cite{mtad-gat,omnianomaly,anomalyTransformer,tranAD}, we use F1-score as the main performance metric to evaluate the performance of anomaly detection, with the threshold for each model chosen as the one which achieves the best F1 over the test sets. In addition, we follow the point-adjusting strategy suggested in \cite{omnianomaly}, which labels a whole anomaly segment as 1 as long as one of the points within the segment is detected as an anomaly. Since our primary contribution is not the development of a new thresholding method, we adopt this well-established practice to eliminate potential bias arising from selecting a specific thresholding method. This choice of reporting F1 scores ensures a fair and consistent comparison across all methods. 

% Additionally, we provide the performance comparison based on two recent proposed metrics VUS-ROC and VUS-PR in~\cite{paparrizos2022volume}, which avoid the need to compute threshold and incorporate the concept of buffer regions that are designed for range-based contextual anomalies (anomaly event). Specifically, VUS\-ROC is the volume under the surfaces created based on ROC curve which is calculated by taking anomaly event into consideration, while VUS\-PR is the volume under the surfaces created based on PR curve. We think different evaluation metrics provide different views.
% We also present a performance comparison using two recently introduced metrics: VUS-ROC and VUS-PR, as detailed in \cite{paparrizos2022volume}. These metrics are designed to adapt traditional ROC and PR curves for time series anomalies, which tend to occur in consecutive sequences. Specifically, VUS-ROC measures the volume under the surfaces of the ROC curve while accounting for these consecutive anomaly sequences. In contrast, VUS-PR calculates the volume under the surfaces based on the PR curve. 

\subsection{Comparison Study}
The results are presented in Table~\ref{tab:comparison_result_f1}. First, both DAGMM and DeepSVDD display the lowest average performance among all models, likely due to their architectural design which does not account for temporal information. On the other hand, models such as MTAD-GAT and AnomalyTransformer perform comparatively better across all datasets in terms of F1 score, a testament to their effective utilization of GNNs to capture inter-series relationships or the global characteristics of time series through Transformers. Yet, CNT outperforms all others with the highest F1 score across all datasets, thus demonstrating the best balance between Recall and Precision. In comparison to these approaches, which utilize either time series forecasting or reconstruction-based methods, our approach utilizes the distance of latent representation between input instance and their contextual information as a criterion to identify anomalies, which are more robust to noise and less likely to overfit the data.

It is worth noting that while CNT is built on top of NeuTralAD, it surpasses NeuTralAD in performance by a significant margin. Two key distinctions contribute to this enhanced efficacy: Firstly, NeuTralAD and CNT diverge in their approach to transformation diversity and semantic relevance. Specifically, NeuTralAD aims to learn a diverse set of transformations semantically associated with a given input time window. In other words, it focuses more on capturing the characteristics of the whole window. This can sometimes dilute anomaly effects, especially when the dominant data trends within the window are normal. In contrast, CNT enforces semantic similarity among learned transformations relative to a context window. It concentrates more on deviations between a short predict window and its historical observations, Secondly, NeuTralAD learns a set of augmentations directly from raw input data, whereas CNT generates transformations through the latent feature space. Empirically, the latter approach can lead to better performance. This can be verified by comparing NeuTralAD with the DCL setting in Section~\ref{section: ablation}, which is essentially the CNT version without the temporal-wise contrasting component.

\begin{table*}[t!]
%\small
    \setlength{\abovecaptionskip}{0cm}
    %\setlength{\belowcaptionskip}{-0.1cm}
    \centering
        % \caption{Performance comparison (F1-scores (\%)) on real-world datasets. The best performance is highlighted in bold.} 
        \caption{Performance comparison (F1 (\%)) on the benchmark datasets, precision (Pre (\%)) and recall (Rec (\%)) are attached. }
    %\begin{adjustbox}{width=\columnwidth,center}
    %\setlength{\tabcolsep}{1.68mm}{
    \begin{tabular}{cccccccccccccc}\\ \toprule
               &   \multicolumn{3}{c}{\textbf{SWaT}} & \multicolumn{3}{c}{\textbf{MSL}} & \multicolumn{3}{c}{\textbf{WADI}} & \multicolumn{3}{c}{\textbf{HAI}} \\ \midrule
               \textbf{Methods} & \textbf{F1} &  \textbf{Pre} & \textbf{Rec} & \textbf{F1} &  \textbf{Pre} & \textbf{Rec} & \textbf{F1} &  \textbf{Pre} & \textbf{Rec}  & \textbf{F1} &  \textbf{Pre} & \textbf{Rec}    \\ \midrule
DAGMM              &  82.3 &         90.6 &      75.8 &  81.0 &         77.0 &      85.7 &  43.7 &         53.5 &      38.4 &  34.3 &         41.3 &      39.0 \\
DeepSVDD           &  86.4 &         96.7 &      78.2 &  80.3 &         75.6 &      87.0 &  47.8 &         82.0 &      33.7 &  37.0 &         29.9 &      61.8 \\
LSTM-VAE           &  81.9 &  98.0 &  70.4 &  88.4 &  87.6 &  89.7 &  64.7 &  66.5 &  63.0 &  69.4 &  64.9 &  77.5  \\
USAD               &  83.0 &         97.3 &      72.4 &  60.0 &         74.4 &      60.0 &  35.6 &         66.9 &      26.5 &  73.6 &         87.7 &      65.5 \\
MAD-GAN            &  80.5 &         98.3 &      68.2 &  77.1 &         71.7 &      86.6 &  73.7 &         88.2 &      63.6 &  17.5 &         16.5 &      48.0 \\
MTAD-GAT           &  84.5 &  94.0 &  77.0&  90.1 &	89.1	&91.2 &  51.0 &  63.5 &  43.0 &  81.0 &  88.4 &  76.6  \\
TranAD             &  83.2 &         96.5 &      73.2 &  79.2 &         71.5 &      89.9 &  41.4 &         62.0 &      31.6 &  73.0 &         88.4 &      63.1 \\
NeuTralAD          &  90.6 &         91.3 &      90.1 &  60.6 &         46.8 &      86.4 &  54.2 &         61.9 &      50.3 &  48.4 &         41.8 &      64.7 \\
LNT                &  86.4 &  95.0 &  79.3 &  90.5 &  91.3 &  89.8 &  35.6 &  74.2 &  24.8 &  54.4 &  72.2 &  48.5 \\
AnomalyTransformer &  89.7 &         92.1 &      87.5 &  93.9 &         91.8 &      96.1 &  69.5 &         74.9 &      64.9 &  57.4 &         61.0 &      56.6 \\
\midrule
CNT &  \textbf{91.7} & 96.5 & 87.3 & \textbf{95.1} & 96.1&	94.3&  \textbf{81.6}	& 82.4	& 81.2   & \textbf{84.0} & 81.5 & 87.8  \\
   \bottomrule
    \end{tabular}
    %}
    %\end{adjustbox}
    \label{tab:comparison_result_f1}
    %\vspace{-0.8cm}
\end{table*}

Lastly, LNT, which is closest to ours, showed inferior performance compared to CNT. LNT fuses CPC loss with the objective of neural transformation learning, necessitating the selection of negative samples during the training stage. Since the majority of these negative samples are normal - as most samples in the training datasets are normal - this can introduce additional bias during the training process. To circumvent this, our approach applies a negative-free training scheme, with the representation collapse problem mitigated by incorporating the discriminative contrastive loss. 

% Although CNT heavily depends on NeuTralAD, the performance of CNT is substantially higher than NeuTralAD. Specifically, there are two distinct differences lie between the two models. First, NeuTralAD intends to learn a set of augmentations directly from the raw input, while our framework generates a set of transformations through latent feature space. Our empirical results show that the latter approach can generate a better performance (See DCL setting in Section~\ref{section: ablation}). Secondly, NeuTralAD focuses on learning a set of diverse transformations that are semantically related to a given input time window, while our approach forces the learned transformations to be semantically similar to a context window. The former focuses more on capturing the characteristics of a whole window which can smooth out the effect of anomalies particularly when the majority of the time points are normal. In contrast, the latter focuses more on the deviation between a short predict window and its context, emphasizing more on the abnormal deviation changes between two windows. 




% \begin{table*}[t!]
% %\small
%     \setlength{\abovecaptionskip}{0cm}
%     %\setlength{\belowcaptionskip}{-0.1cm}
%     \centering
%         % \caption{Performance comparison (F1-scores (\%)) on real-world datasets. The best performance is highlighted in bold.} 
%         \caption{Performance comparison (F1 (\%)) on the benchmark datasets, precision (Pre (\%)) and recall (Rec (\%)) are attached. }
%     %\begin{adjustbox}{width=\columnwidth,center}
%     %\setlength{\tabcolsep}{1.68mm}{
%     \begin{tabular}{cccccccccccccc}\\ \toprule
%                &   \multicolumn{3}{c}{\textbf{SWaT}} & \multicolumn{3}{c}{\textbf{WADI}} & \multicolumn{3}{c}{\textbf{HAI}} & \multicolumn{3}{c}{\textbf{MSL}} \\ \midrule
%                \textbf{Methods} & \textbf{F1} &  \textbf{Pre} & \textbf{Rec} & \textbf{F1} &  \textbf{Pre} & \textbf{Rec} & \textbf{F1} &  \textbf{Pre} & \textbf{Rec}  & \textbf{F1} &  \textbf{Pre} & \textbf{Rec}    \\ \midrule
% DAGMM              &  70.17 &  69.96 &  77.07 &  43.68 &  53.50 &  38.42 &  34.95 &  43.81 &  39.21 &  80.96 &  76.96 &  85.73 \\
% DeepSVDD           &  86.41 &  96.68 &  78.16 &  45.37 &  77.44 &  34.30 &  35.36 &  31.08 &  50.39 &  81.03 &  76.99 &  86.87 \\
% LSTM-VAE           &  81.90 &  97.95 &  70.42 &  64.70 &  66.53 &  62.99 &  69.41 &  64.90 &  77.46 &  88.40 &  87.55 &  89.70 \\
% USAD               &  84.60 &  \textbf{98.70} &  74.02 &  61.74 &  84.49 &  48.65 &  74.93 &  83.48 &  68.43 &  92.72 &  88.10 &  \textbf{97.86} \\
% MAD-GAN            &  80.44 &  97.31 &  68.77 &  74.09 &  \textbf{90.23} &  62.96 &  20.94 &  29.06 &  37.45 &  76.45 &  80.66 &  76.55 \\
% TranAD             &  83.17 &  97.39 &  72.61 &  41.05 &  69.83 &  29.91 &  73.93 &  \textbf{88.60} &  64.70 &  91.55 &  90.41 &  92.73 \\
% LNT                &  86.36 &  94.95 &  79.34 &  35.55 &  74.20 &  24.77 &  54.43 &  72.23 &  48.51 &  90.50 &  91.28 &  89.84 \\
% AnomalyTrans &  91.34 &  91.87 &  \textbf{90.82} &  69.00 &  75.41 &  63.59 &  58.02 &  63.33 &  55.26 &  93.97 &  92.75 &  95.25 \\
% \midrule
% CNT &  \textbf{91.68} & 96.50 & 87.33 &  \textbf{81.61}	& 82.39	& \textbf{81.19}   & \textbf{83.95} & 81.48 & \textbf{87.75} &  \textbf{95.13}&	\textbf{96.06}&	94.26 \\
%    \bottomrule
%     \end{tabular}
%     %}
%     %\end{adjustbox}
%     \label{tab:comparison_result_f1}
%     %\vspace{-0.8cm}
% \end{table*}













% Both the sequence-level contrasting objective and the neural transformation learning objective can effectively collaborate to enhance anomaly detection performance. 

% Furthermore, we assessed model performance using VUS\_PR and VUS\_ROC metrics on recent state-of-the-art time series models. While the ranking of all models slightly shifts compared to the F1 score, our approach still maintains consistently high performance across the majority of datasets. (need to be modified)
%only falling behind TranAD on MSL datasets and LNT on SWaT. 

% This outcome could be attributed to our use of the TCN encoder, which may be less capable of capturing global characteristics compared to the Transformer used in TranAD. As such, the design of a more effective base feature encoder is a direction for our future research.

% This could be attributed to its strategy of minimizing the distance between the transformations of point-wise future predictions and the context window, a method that may fail to preserve identical semantic meanings. Conversely, our model leverages a sequence-to-sequence comparison where the suspect and context sequences share semantically meaningful features owing to their overlap and shared feature encoder.


% our model achieves the highest F1 for all datasets. In addition, Precision and Recall are also on average within the top 3. We also compare the performance based on recently proposed metrics, VUS\-ROC and VUS\-PR for the recent state-of-the-art methods, and the results show that our model outperforms them in the majority datasets while slightly falling behind LNT in terms of VUS\_ROC for swat.
% % However, our model's performance falls short on MSL and SMAP. This could be due to the majority of features in these datasets being one-hot encoded commands, making temporal encoding of sequences challenging for simple TCN layers that tend to mix all features through simple sum aggregation. On the other hand, graph-based models like GDN, which explicitly learn the relationship between features, have performed well on these datasets.

% Additionally, NCAD currently holds state-of-the-arts performance on MSL and SMAP due to its semi-supervised classification training schemes based on synthetic anomalies. While supervised training is known to be more effective when the underlying distribution of synthetic anomalies is similar to that of the true anomalies in the dataset, we can see that NCAD performed relatively worse in WADI, HAI, and SMD compared to our methods, suggesting potential overfitting due to these datasets having a variety of different anomaly types beyond the injected ones.

% ON the other hand, LNT, a similar model to ours, showed inferior performance compared to our model, possibly because it attempts to minimize the distance between the transformation of point-wise future predictions and the context window, which may not have identical semantic meanings. In contrast, our model employs a sequence-to-sequence comparison, where the suspect and context sequences share semantically meaningful features due to their overlap and shared feature encoder.


\subsection{Extended Investigation}
\subsubsection{Ablation Study}
\label{section: ablation}
In this section, we aim to verify whether each component does contribute to our final performance. Specifically, we test the following two settings: 
1) CCL: Here, $g(\cdot)$ is trained exclusively under the contextual contrastive loss in Eq.~\eqref{eq. raw contextual one-class objective}. 
2) DCL: The feature encoder network $g(\cdot)$ is trained purely under the discriminative contrastive loss in Eq.\eqref{eq. contextual discriminative contrastive loss}. It's akin to NeutralAD, but transformations are applied to the feature encoder output rather than the original sequence. 

Table~\ref{tab:ablation_result} presents the results of our experiments. The CCL setting is designed to assign similar representations to normal sequences in close proximity, but its performance falls short in comparison to our proposed approach. This can potentially be attributed to the representation collapse problem, wherein the loss function leads the encoder to converge to a parameter space that closely approximates the constant encoder solution. Consequently, the model may fail to capture the rich semantic information of normal sequences. On the other hand, 
\begin{wraptable}{r}{6cm}
%\small
    \vspace{-0.4cm}
    \setlength{\abovecaptionskip}{0cm}
    %\setlength{\belowcaptionskip}{-0.1cm}
    \centering
    \caption{Performance comparison (F1 (\%)) by removing components of our framework.} 
    \begin{tabular}{ccccccc}\\ \toprule
     \textbf{Settings} & \textbf{SWaT} & \textbf{MSL}  & \textbf{WADI} & \textbf{HAI} \\ \midrule
  % Default             &  91.99     &  \\ \midrule
CNT    & \textbf{91.7} & \textbf{95.1} & \textbf{81.6} & \textbf{84.0}\\ \midrule
DCL     &  85.1 &  81.2 &  30.4 &  67.5 \\
CCL &  88.0 &  91.5 &  66.2 &  64.2 \\
   \bottomrule
    \end{tabular}
    \label{tab:ablation_result}
    \vspace{-0.3cm}
\end{wraptable}
The DCL configuration primarily encourages similarity between an input time window and its corresponding transformed sequences, prioritizing the modeling of characteristics across the entire time window. Consequently, anomalies within short time spans may be overlooked, resulting in negligible distance scores between the time window and its transformations, particularly for longer time windows. In contrast, our default setting emphasizes the discrepancy between the predict window and the context window, thereby enhancing accurate anomaly detection within the overlapping region.

\begin{figure}[t]
    \centering
   % \includesvg[width=1\linewidth]{figures/Framework.svg}
        \includesvg[height=6.5cm]{figures/neural_contrast/showcases_tods_small.svg}
        % \includegraphics[height=8cm, width=11.5cm]{figures/neural_contrast/showcases_tods.svg}

        \caption{The above figure showcases various types of anomalies present in the TODS dataset alongside the corresponding anomaly scores generated by CNT, DCL, and CCL settings.}
    \label{fig: tods showcase}
%\vspace{0.5cm}
\end{figure}




\subsubsection{Comparison against different model variants}
In Section~\ref{sec: self-supervised-learning}, we list a couple of existing techniques for contrastive learning that can alleviate the representation collapse issue. In this section, we show that our proposed framework is still superior to those variants. First, here are the details of the variants that we aim to compare with:
(1) CCL + Neg: A straightforward adaptation of CCL loss is to introduce the negative samples into the contrastive framework. Following the settings in CPC~\cite{cpc}, for each predict window, we sample a random set of context windows within the batch as negative samples, and the feature encoder is trained under the infoNCE loss with the distance function replaced by the $l_2$ distance in Eq.~\eqref{eq. raw contextual one-class objective}.
(2) CCL + Vicreg: Similar to~\cite{vicreg}, $g(\cdot)$ is trained under the contextual contrastive loss, supplemented with a regularization term to ensure non-zero variance of the latent representations within a batch, thereby ensuring non-constant encoder outputs. The operation is defined as:
\begin{align}
    &L_{\text{ccl+vicreg}} = L_{\text{ccl}} + v(\{S^{t}\}_{t\in B}) + v(\{C^{t}\}_{t\in B}) \\
    & v(\{S^{t}\}_{t \in B}) = \frac{1}{d} \sum_{j=1}^d \max(0, \gamma - \sqrt{\text{Var}(\{g(S^t)_j\}_{t \in B}) + \epsilon}) \label{eq: regularization on ccl}
\end{align}
where $B$ denotes an arbitrary mini-batch of samples containing $X^t$, $\gamma$ is set to 1 as in~\cite{vicreg}, and $\epsilon$ is a small scaler value to prevent numerical instabilities. The variance in Eq.\eqref{eq: regularization on ccl} is computed over the encoder outputs within the batch $B$. During inference, only $L_{\text{ccl}}$ is used as the anomaly score. 
(3) CCL+Simsiam: Following~\cite{simsiam}, we create unique feature encoders for the predict and context sequences, and compute two CCL losses. Each loss applies the stopping criterion on the representation of one sequence, with the other remaining detached. During inference, the sum of the two losses serves as the anomaly scores. The essential idea of this setting is to incorporate continuous target changes in order to prevent constant encoder solutions.


Table~\ref{tab:variants} presents the results of our experiments. First, we can see that incorporating the negative samples did improve the performance of CCL on average. 
\begin{wraptable}{r}{6.8cm}
%\small
    \vspace{-0.4cm}
    \setlength{\abovecaptionskip}{0cm}
    %\setlength{\belowcaptionskip}{-0.1cm}
    \centering
    \caption{Performance comparison (F1 (\%)) against different model variants.} 
    \begin{tabular}{ccccccc}\\ \toprule
     \textbf{Settings} & \textbf{SWaT} & \textbf{WADI}  & \textbf{HAI} & \textbf{MSL} \\ \midrule
  % Default             &  91.99     &  \\ \midrule
% CNT    & \textbf{91.7} & \textbf{81.6} & \textbf{84.0} & \textbf{95.1} \\ \midrule
% CCL+Neg & & & & \\
% CCL+Vicreg  & 89.0 & 54.3 & 50.3 & 87.5\\
% CCL+Simsiam & \textbf{91.8}	&66.3	&78.3 &	92.7 \\ 
CNT    & 91.7 & \textbf{95.1} & \textbf{81.6} & \textbf{84.0}\\ \midrule
CCL+Neg               &  89.5 &  90.5 &  78.5 &  65.9 \\
CCL+Vicreg               &  89.0 &  87.5 &  54.3 &  50.3 \\
CCL+Simsiam &  \textbf{91.8} &  92.7 &  66.3 &  78.3 \\

   \bottomrule
    \end{tabular}
    \label{tab:variants}
    \vspace{-0.3cm}
\end{wraptable}
but still underperform than CNT. One of the reasons is that the negative samples are selected from a dataset that consists mostly the normal samples. This could make the model a bit confused to distinguish normal samples from abnormal samples based on a wrong classification bound. For the rest of the settings, recall that the goal of the CCL+Vicreg and CCL+Siamsam settings, the direct variants of the CCL setting, aim to prevent the representation collapse issue. Yet, our model still surpasses them on average across datasets. Distinguished from these two configurations, the incorporation of DCL loss ensures not only non-constant latent representations but also compels transformations of the predict sequences to stay semantically akin to original sequences. This provides a diverse range of perspectives on sequence normality and enables multi-angular similarity measurement between sequences.

\subsubsection{Analysis Of Learning Situations}
In section~\ref{sec:theoretical analysis}, we show that simply using 
\begin{wrapfigure}{r}{6.5cm}
\vspace{-0.4cm}
\centering
\includegraphics[height=3.5cm]{figures/neural_contrast/loss_decay.eps}  
\caption{Provided the loss value per epoch with the model trained on the WADI dataset. The small window is the zooming region for loss values from 20 to 30 epochs.}
\label{fig: loss_decay}
\vspace{-0.3cm}
\end{wrapfigure}
$L_{\text{ccl}}$ could lead to the representation collapse issue, where the feature representations of the context window and the predict window collapse to the same constant. Then we proved that under the assumption that $L_{\text{dcl}}<K\log{K}$, this situation does not apply to the case when we combine the CCL and DCL losses. 
Figure~\ref{fig: loss_decay} shows
the loss values per epoch for our model training under purely $L_{\text{ccl}}$ loss or training under both $L_{\text{cncl}}$ and $L_{\text{dcl}}$ (the default setting). It is clear that $L_{\text{ccl}}$ decays quickly to 0 without the regularization of $L_{\text{dcl}}$, which agrees with Proposition~\ref{props: constant encoder}. In contrast, with the additional constraints of $L_{\text{dcl}}$, $L_{\text{cncl}}$ decays much slowly compared to the former. This implies that $L_{\text{dcl}}$ does add additional complexity to the CCL task, preventing from learning trivial feature representations. This is also verified in our ablation study that the combination of both losses can obtain a much higher performance than using $L_{\text{ccl}}$ only. Furthermore, as shown in Figure~\ref{fig: loss_decay}, we can see that the loss value of $L_{\text{dcl}}$ quickly falls below $K\log K$, which is around 4.67 when $K=6$ (the default parameter setting used in our experiments). This verifies the assumption in Proposition ~\ref{props: non-constant encoder} is empirically applicable. 



% \subsubsection{Sensitivity of Hyper-parameters}
% In this section we conduct the sensitivity analysis on three hyper-parameters, the sizes of the sliding window $w$, the predict window $p$, and the number of transformations $K$, primarily based on SWaT and MSL datasets with each parameter setting result averaged over 5 runs. Figure~\ref{fig: sensitivity_results}a illustrates the F1 score’s correlation with the sliding window size, with the predict window size held constant at 5. We can see a relatively higher performance when the sequence length lies between 20 and 60. This finding is consistent with the performance of other baseline models (e.g., TranAD, MTAD-GAT, and LNT), which also obtain optimal performances by adopting a sequence length within this range. Figure~\ref{fig: sensitivity_results}b explores the F1 score’s variability in response to different predict window sizes, while maintaining the sliding window size at 30. The model exhibits peak performance for prediction window sizes between 3 and 5 and experiences a noticeable decline when the size exceeds 9. This trend is logical, as larger prediction window sizes can smooth out the effect of anomalies (Most anomalies in the benchmark datasets are short-lived), reducing their distinctiveness from normal sample scores. Figure~\ref{fig: sensitivity_results}c portrays the F1 score's responsiveness to varying numbers of transformations. The optimal performance is observed at approximately $K=6$, with some performance fluctuations across other values. 
% \begin{figure*}[h]
% %\centering
% % \begin{subfigure}[b]{1\linewidth}
% %     \centering
% %      % \includesvg[height=4.2cm]{figures/swat_ts_unidentified_event1.svg}
% %     \includegraphics[height=0.5cm]{figures/neural_contrast/legend.eps}
% %     %\caption{}
% %    % \label{fig: win_size_results}
% % \end{subfigure}
% %\newline
% %\vspace{0.5cm}
% %\centering
% \begin{subfigure}[b]{.32\linewidth}
%     \centering
%     \includegraphics[height=2.4cm]{figures/neural_contrast/seq_len_results.eps}
%     %\caption{F1 vs. sliding window size}
%     \label{fig: seq_len_results}
% \end{subfigure}
% \begin{subfigure}[b]{.32\linewidth}
%     \centering
%     \includegraphics[height=2.4cm]{figures/neural_contrast/win_size_results.eps} 
%     %\caption{F1 vs. predict window size}
%     \label{fig: win_size_results}
% \end{subfigure}
% \begin{subfigure}[b]{.32\linewidth}
%     \centering
%     \includegraphics[height=2.4cm]{figures/neural_contrast/n_transformations_results.eps} 
%     %\caption{F1 vs. \# transformations}
%     \label{fig: n_transformations_results}
% \end{subfigure}
% \caption{(a) Average F1 versus sliding window size $w$ from 20 to 100; (b) Average F1 versus predict window size $p$ from 1 to 11; (c) Average F1 versus number of transformations $K$ from 2 to 12.}
% \label{fig: sensitivity_results}
% \end{figure*}




\subsubsection{Computational Analysis}
Figure~\ref{fig: computation_time} illustrates the training time per epoch and inference time of the training and test datasets based on SWaT for each model, measured in seconds. CNT demonstrates a substantially lower training and inference time compared to other models. 
% In contrast to LNT, which necessitates the computation of distance between the $k$-step ahead time series value and their contextual window, our approach significantly enhances computational efficiency by employing sequence-to-sequence contrastive learning. Furthermore, the base architecture of our method is TCN, inherently a more lightweight design compared to those based on RNN or Transformer architectures.

\begin{figure}[h]
\centering
%\vspace{-0.2cm}
\includesvg[height=3.5cm]{figures/neural_contrast/computation_time.svg}

\caption{The training time per epoch and inference time of each model based on the SWaT dataset.}
\label{fig: computation_time}
\end{figure}


==> subtexes/experiments_v4.tex <==
%\section{Experiment}
\subsection{Datasets and Experimental Setup}
Four industrial real-world datasets are adopted for the evaluation of time series anomaly detection methods, which are SWaT~\cite{mathur2016swat}, WADI~\cite{ahmed2017wadi}, HAI~\cite{hai21.03}, and MSL~\cite{lstm-ndt}. Each dataset has a unlabeled training set, and a separate test set with anomalies. More detailed descriptions of the datasets as well as summary statistics are shown in \textbf{Section 4} of the supplementary materials. Given the limited space, we present the experimental setting and the sensitivity analysis of hyper-parameters in \textbf{Section 4\&1.5} of the supplementary materials.


\subsection{Baseline Methods and Evaluation Metrics}
We compare our framework with common anomaly detection approaches as the baseline methods, including DeepSVDD~\cite{deepSVDD} and DAGMM~\cite{zong2018deep}, which are general anomaly detection deep learning-based models, and LSTM-VAE~\cite{lstm-vae}, MAD-GAN~\cite{mad-gan}, USAD~\cite{usad}, MTAD-GAT~\cite{mtad-gat}, LNT~\cite{lnt}, TranAD~\cite{tranAD}, NeuTralAD~\cite{neuralAD} and AnomalyTransformer~\cite{anomalyTransformer}, which are popular anomaly detection methods tailored specifically to time series data.

In line with previous studies~\cite{mtad-gat,omnianomaly,anomalyTransformer,tranAD}, we use the best F1-score as the main performance metric to evaluate the performance of anomaly detection. We follow the point-adjusting strategy suggested in \cite{omnianomaly}, which labels a whole anomaly segment as 1 as long as one of the points within the segment is detected as an anomaly. Since our primary contribution is not the development of a new thresholding method, we adopt this well-established practice to eliminate potential bias arising from selecting a specific thresholding method. This choice of reporting F1 scores ensures a fair and consistent comparison across all methods. 

\subsection{Comparison Study}
The results are presented in Table~\ref{tab:comparison_result_f1}. First, both DAGMM and DeepSVDD display relatively lower performance due to their base model which does not account for temporal information. On the other hand, models such as MTAD-GAT and AnomalyTransformer perform comparatively better across all datasets in terms of F1 score, a testament to their effective utilization of GNNs to capture inter-series relationships or the global characteristics of time series through Transformers. Yet, CNT outperforms all others with the highest F1 score across all datasets, thus demonstrating the best balance between Recall and Precision. In comparison to these approaches, which utilize either time series forecasting or reconstruction-based methods, our approach utilizes the distance of latent representation between input instance and their contextual information as a criterion to identify anomalies, which are more robust to noise and less likely to overfit the data.
% \begin{table*}[t!]
% %\small
%     \setlength{\abovecaptionskip}{0cm}
%     \centering
%         \caption{Performance comparison (F1 (\%)) on the benchmark datasets, precision (Pre (\%)) and recall (Rec (\%)) are attached. }
%     \begin{tabular}{cccccccccccccc}\\ \toprule
%                &   \multicolumn{3}{c}{\textbf{SWaT}} & \multicolumn{3}{c}{\textbf{MSL}} & \multicolumn{3}{c}{\textbf{WADI}} & \multicolumn{3}{c}{\textbf{HAI}} \\ \midrule
%                \textbf{Methods} & \textbf{F1} &  \textbf{Pre} & \textbf{Rec} & \textbf{F1} &  \textbf{Pre} & \textbf{Rec} & \textbf{F1} &  \textbf{Pre} & \textbf{Rec}  & \textbf{F1} &  \textbf{Pre} & \textbf{Rec}    \\ \midrule
% DAGMM              &  82.3 &         90.6 &      75.8 &  81.0 &         77.0 &      85.7 &  43.7 &         53.5 &      38.4 &  34.3 &         41.3 &      39.0 \\
% DeepSVDD           &  86.4 &         96.7 &      78.2 &  80.3 &         75.6 &      87.0 &  47.8 &         82.0 &      33.7 &  37.0 &         29.9 &      61.8 \\
% LSTM-VAE           &  81.9 &  98.0 &  70.4 &  88.4 &  87.6 &  89.7 &  64.7 &  66.5 &  63.0 &  69.4 &  64.9 &  77.5  \\
% USAD               &  83.0 &         97.3 &      72.4 &  60.0 &         74.4 &      60.0 &  35.6 &         66.9 &      26.5 &  73.6 &         87.7 &      65.5 \\
% MAD-GAN            &  80.5 &         98.3 &      68.2 &  77.1 &         71.7 &      86.6 &  73.7 &         88.2 &      63.6 &  17.5 &         16.5 &      48.0 \\
% MTAD-GAT           &  84.5 &  94.0 &  77.0&  90.1 &	89.1	&91.2 &  51.0 &  63.5 &  43.0 &  81.0 &  88.4 &  76.6  \\
% TranAD             &  83.2 &         96.5 &      73.2 &  79.2 &         71.5 &      89.9 &  41.4 &         62.0 &      31.6 &  73.0 &         88.4 &      63.1 \\
% NeuTralAD          &  90.6 &         91.3 &      90.1 &  60.6 &         46.8 &      86.4 &  54.2 &         61.9 &      50.3 &  48.4 &         41.8 &      64.7 \\
% LNT                &  86.4 &  95.0 &  79.3 &  90.5 &  91.3 &  89.8 &  35.6 &  74.2 &  24.8 &  54.4 &  72.2 &  48.5 \\
% AnomalyTransformer &  89.7 &         92.1 &      87.5 &  93.9 &         91.8 &      96.1 &  69.5 &         74.9 &      64.9 &  57.4 &         61.0 &      56.6 \\
% \midrule
% CNT &  \textbf{91.7} & 96.5 & 87.3 & \textbf{95.1} & 96.1&	94.3&  \textbf{81.6}	& 82.4	& 81.2   & \textbf{84.0} & 81.5 & 87.8  \\
%    \bottomrule
%     \end{tabular}
%     \label{tab:comparison_result_f1}
% \end{table*}


\begin{table*}[t!]
%\small
    \setlength{\abovecaptionskip}{0cm}
    \centering
        \caption{Performance comparison (F1 (\%)) on the benchmark datasets, precision (Pre (\%)) and recall (Rec (\%)) are attached. }
    \begin{tabular}{cccccccccccccc}\\ \toprule
               &   \multicolumn{3}{c}{\textbf{SWaT}} & \multicolumn{3}{c}{\textbf{MSL}} & \multicolumn{3}{c}{\textbf{WADI}} & \multicolumn{3}{c}{\textbf{HAI}} \\ \midrule
               \textbf{Methods} & \textbf{F1} &  \textbf{Pre} & \textbf{Rec} & \textbf{F1} &  \textbf{Pre} & \textbf{Rec} & \textbf{F1} &  \textbf{Pre} & \textbf{Rec}  & \textbf{F1} &  \textbf{Pre} & \textbf{Rec}    \\ \midrule
DAGMM              &  82.3 &         90.6 &      75.8 &  81.0 &         77.0 &      85.7 &  43.7 &         53.5 &      38.4 &  34.3 &         41.3 &      39.0 \\
DeepSVDD           &  86.4 &         96.7 &      78.2 &  80.3 &         75.6 &      87.0 &  47.8 &         82.0 &      33.7 &  37.0 &         29.9 &      61.8 \\
LSTM-VAE           &  81.9 &         97.9 &      70.4 &  87.5 &         87.8 &      87.7 &  64.6 &         66.3 &      63.0 &  70.8 &         67.8 &      76.4 \\
USAD               &  83.0 &         97.3 &      72.4 &  60.0 &         74.4 &      60.0 &  35.6 &         66.9 &      26.5 &  73.6 &         87.7 &      65.5 \\
MAD-GAN            &  80.5 &         98.3 &      68.2 &  77.1 &         71.7 &      86.6 &  73.7 &         88.2 &      63.6 &  17.5 &         16.5 &      48.0 \\
MTAD-GAT           &  83.2 &         94.4 &      74.5 &  88.4 &         87.1 &      89.8 &  46.3 &         50.1 &      44.2 &  78.0 &         90.8 &      71.0 \\
TranAD             &  83.2 &         96.5 &      73.2 &  79.2 &         71.5 &      89.9 &  41.4 &         62.0 &      31.6 &  73.0 &         88.4 &      63.1 \\
NeuTralAD          &  90.6 &         91.3 &      90.1 &  60.6 &         46.8 &      86.4 &  54.2 &         61.9 &      50.3 &  48.4 &         41.8 &      64.7 \\
LNT                &  86.4 &  95.0 &  79.3 &  90.5 &  91.3 &  89.8 &  35.6 &  74.2 &  24.8 &  54.4 &  72.2 &  48.5 \\
AnomalyTransformer &  89.7 &         92.1 &      87.5 &  93.9 &         91.8 &      96.1 &  69.5 &         74.9 &      64.9 &  57.4 &         61.0 &      56.6 \\
\midrule
CNT &  \textbf{91.7} & 96.5 & 87.3 & \textbf{95.1} & 96.1&	94.3&  \textbf{81.6}	& 82.4	& 81.2   & \textbf{84.0} & 81.5 & 87.8  \\
   \bottomrule
    \end{tabular}
    \label{tab:comparison_result_f1}
\end{table*}
It is worth noting that while CNT is built on top of NeuTralAD, it surpasses NeuTralAD in performance by a significant margin. One key contribution to this enhanced efficacy is that NeuTralAD and CNT diverge in their approach to transformation diversity and semantic relevance. Specifically, NeuTralAD aims to learn a diverse set of transformations semantically associated with a given input time window. In other words, it focuses more on capturing the characteristics of the whole window. This can sometimes dilute anomaly effects, especially when the dominant data trends within the window are normal. In contrast, CNT enforces semantic similarity among learned transformations relative to a context window. It concentrates more on deviations between a short predict window and its historical observations. Additionally, CNT introduces a notable computational advantage. Unlike NeuTralAD, which requires multiple passes of the transformations over the raw time series data, CNT applies the feature encoder a single time to the latent space, creating transformations more efficiently (see the computational analysis in \textbf{Section 1.4} of the supplementary materials). 


Lastly, the LNT model, though conceptually similar to CNT, lags in performance. LNT combines CPC loss with neural transformation learning, relying on negative sample selection which can bias the training due to the prevalence of normal samples. Our CNT model avoids this with a negative-free training strategy, leveraging discriminative contrastive loss to prevent representation collapse.


\subsection{Ablation Study}
\label{section: ablation}
In this section, we aim to verify whether each component does contribute to our final performance. Specifically, we test the following two settings: 
1) CCL: Here, $g(\cdot)$ is trained exclusively under the contextual contrastive loss in Eq.~\eqref{eq. raw contextual one-class objective}. 
2) DCL: The feature encoder network $g(\cdot)$ is trained purely under the discriminative contrastive loss in Eq.\eqref{eq. contextual discriminative contrastive loss}. It's akin to NeutralAD, but transformations are applied to the feature encoder output rather than the original sequence. We also present the results of more settings, including CCL with negative samples, and a variety of negative-sample-free regularizations inspired by BYOL, Simsiam, and VICReg in \textbf{Section 1.2} of the supplementary materials.

Table~\ref{tab:ablation_result} presents the results of our experiments. The CCL setting is designed to assign similar representations to normal sequences in close proximity, but
\begin{wraptable}{r}{6cm}
%\small
    \vspace{-0.4cm}
    \setlength{\abovecaptionskip}{0cm}
    %\setlength{\belowcaptionskip}{-0.1cm}
    \centering
    \caption{Performance comparison (F1 (\%)) for ablation study.} 
    \begin{tabular}{ccccccc}\\ \toprule
     \textbf{Settings} & \textbf{SWaT} & \textbf{MSL}  & \textbf{WADI} & \textbf{HAI} \\ \midrule
  % Default             &  91.99     &  \\ \midrule
CNT    & \textbf{91.7} & \textbf{95.1} & \textbf{81.6} & \textbf{84.0}\\ \midrule
DCL     &  85.1 &  81.2 &  30.4 &  67.5 \\
CCL &  88.0 &  91.5 &  66.2 &  64.2 \\
   \bottomrule
    \end{tabular}
    \label{tab:ablation_result}
    \vspace{-0.3cm}
\end{wraptable}
its performance falls short in comparison to our proposed approach. This can potentially be attributed to the representation collapse problem, wherein the loss function leads the encoder to converge to a parameter space that closely approximates the constant encoder solution. Consequently, the model may fail to capture the rich semantic information of normal sequences. On the other hand, 
The DCL configuration primarily encourages similarity between an input time window and its corresponding transformed sequences, prioritizing the modeling of characteristics across the entire time window. Consequently, anomalies within short time spans may be overlooked, resulting in negligible distance scores between the time window and its transformations, particularly for longer time windows. In contrast, our default setting emphasizes the discrepancy between the predict window and the context window, thereby enhancing accurate anomaly detection within the overlapping region. We also present data visualizations in \textbf{Section 1.1} of the supplementary materials, showing that CNT can generate more discriminative anomaly scores compared to the other two settings for different types of contextual anomalies.


% \subsubsection{Analysis Of Learning Situations}
% In section~\ref{sec:theoretical analysis}, we show that simply using 
% $L_{\text{ccl}}$ could lead to the representation collapse issue, where the feature
% \begin{wrapfigure}{r}{6.5cm}
% \vspace{-0.4cm}
% \centering
% \includegraphics[height=3.5cm]{figures/neural_contrast/loss_decay.eps}  
% \caption{Provided the loss value per epoch with the model trained on WADI.}
% \label{fig: loss_decay}
% \vspace{-0.3cm}
% \end{wrapfigure}
% representations of the context window and the predict window collapse to the same constant. Then we show that under the assumption that $L_{\text{dcl}}<K\log{K}$, this situation does not apply to the case when we combine CCL with DCL. 
% Figure~\ref{fig: loss_decay} shows
% the loss values per epoch for our model training under purely $L_{\text{ccl}}$ loss or training under both $L_{\text{cncl}}$ and $L_{\text{dcl}}$ (the default setting). It is clear that $L_{\text{ccl}}$ decays quickly to 0 without the regularization of $L_{\text{dcl}}$, which agrees with Proposition~\ref{props: constant encoder}. In contrast, with the additional constraints of $L_{\text{dcl}}$, $L_{\text{cncl}}$ decays much slowly compared to the former. This implies that $L_{\text{dcl}}$ does add additional complexity to the CCL task, preventing from learning trivial feature representations. This is also verified in our ablation study that the combination of both losses can obtain a much higher performance than using $L_{\text{ccl}}$ only. Furthermore, Figure~\ref{fig: loss_decay} shows that the loss value of $L_{\text{dcl}}$ quickly falls below $K\log K$, which is around 4.67 when $K=6$ (the default parameter setting used in our experiments). This verifies the assumption in Proposition ~\ref{props: non-constant encoder} is empirically applicable. 

% \begin{figure}[t]
%     \centering
%    % \includesvg[width=1\linewidth]{figures/Framework.svg}
%         \includesvg[height=6.5cm]{figures/neural_contrast/showcases_tods_small.svg}
%         % \includegraphics[height=8cm, width=11.5cm]{figures/neural_contrast/showcases_tods.svg}

%         \caption{The above figure showcases various types of anomalies present in the TODS dataset alongside the corresponding anomaly scores generated by CNT, DCL, and CCL settings.}
%     \label{fig: tods showcase}
% %\vspace{0.5cm}
% \end{figure}




% \subsubsection{Comparison against different model variants}
% In Section~\ref{sec: self-supervised-learning}, we list a couple of existing techniques for contrastive learning that can alleviate the representation collapse issue. In this section, we show that our proposed framework is still superior to those variants. First, here are the details of the variants that we aim to compare with:
% (1) CCL + Neg: A straightforward adaptation of CCL loss is to introduce the negative samples into the contrastive framework. Following the settings in CPC~\cite{cpc}, for each predict window, we sample a random set of context windows within the batch as negative samples, and the feature encoder is trained under the infoNCE loss with the distance function replaced by the $l_2$ distance in Eq.~\eqref{eq. raw contextual one-class objective}.
% (2) CCL + Vicreg: Similar to~\cite{vicreg}, $g(\cdot)$ is trained under the contextual contrastive loss, supplemented with a regularization term to ensure non-zero variance of the latent representations within a batch, thereby ensuring non-constant encoder outputs. 
% (3) CCL+Simsiam: Following~\cite{simsiam}, we create unique feature encoders for the predict and context sequences, and compute two CCL losses. Each loss applies the stopping criterion on the representation of one sequence, with the other remaining detached. During inference, the sum of the two losses serves as the anomaly scores. The essential idea of this setting is to incorporate continuous target changes in order to prevent constant encoder solutions.


% Table~\ref{tab:variants} presents the results of our experiments. First, we can see that incorporating the negative samples did improve the performance of CCL on average. 
% \begin{wraptable}{r}{6.8cm}
% %\small
%     \vspace{-0.4cm}
%     \setlength{\abovecaptionskip}{0cm}
%     %\setlength{\belowcaptionskip}{-0.1cm}
%     \centering
%     \caption{Performance comparison (F1 (\%)) against different model variants.} 
%     \begin{tabular}{ccccccc}\\ \toprule
%      \textbf{Settings} & \textbf{SWaT} & \textbf{WADI}  & \textbf{HAI} & \textbf{MSL} \\ \midrule
%   % Default             &  91.99     &  \\ \midrule
% % CNT    & \textbf{91.7} & \textbf{81.6} & \textbf{84.0} & \textbf{95.1} \\ \midrule
% % CCL+Neg & & & & \\
% % CCL+Vicreg  & 89.0 & 54.3 & 50.3 & 87.5\\
% % CCL+Simsiam & \textbf{91.8}	&66.3	&78.3 &	92.7 \\ 
% CNT    & 91.7 & \textbf{95.1} & \textbf{81.6} & \textbf{84.0}\\ \midrule
% CCL+Neg               &  89.5 &  90.5 &  78.5 &  65.9 \\
% CCL+Vicreg               &  89.0 &  87.5 &  54.3 &  50.3 \\
% CCL+Simsiam &  \textbf{91.8} &  92.7 &  66.3 &  78.3 \\

%    \bottomrule
%     \end{tabular}
%     \label{tab:variants}
%     \vspace{-0.3cm}
% \end{wraptable}
% but still underperform than CNT. One of the reasons is that the negative samples are selected from a dataset that consists mostly the normal samples. This could make the model a bit confused to distinguish normal samples from abnormal samples based on a wrong classification bound. For the rest of the settings, recall that the goal of the CCL+Vicreg and CCL+Siamsam settings, the direct variants of the CCL setting, aim to prevent the representation collapse issue. Yet, our model still surpasses them on average across datasets. Distinguished from these two configurations, the incorporation of DCL loss ensures not only non-constant latent representations but also compels transformations of the predict sequences to stay semantically akin to original sequences. This provides a diverse range of perspectives on sequence normality and enables multi-angular similarity measurement between sequences.








% Lastly, LNT, which is closest to ours, showed inferior performance compared to CNT. LNT fuses CPC loss with the objective of neural transformation learning, necessitating the selection of negative samples during the training stage. Since the majority of these negative samples are normal - as most samples in the training datasets are normal - this can introduce additional bias during the training process. To circumvent this, our approach applies a negative-free training scheme, with the representation collapse problem mitigated by incorporating the discriminative contrastive loss. 

% Although CNT heavily depends on NeuTralAD, the performance of CNT is substantially higher than NeuTralAD. Specifically, there are two distinct differences lie between the two models. First, NeuTralAD intends to learn a set of augmentations directly from the raw input, while our framework generates a set of transformations through latent feature space. Our empirical results show that the latter approach can generate a better performance (See DCL setting in Section~\ref{section: ablation}). Secondly, NeuTralAD focuses on learning a set of diverse transformations that are semantically related to a given input time window, while our approach forces the learned transformations to be semantically similar to a context window. The former focuses more on capturing the characteristics of a whole window which can smooth out the effect of anomalies particularly when the majority of the time points are normal. In contrast, the latter focuses more on the deviation between a short predict window and its context, emphasizing more on the abnormal deviation changes between two windows. 




% \begin{table*}[t!]
% %\small
%     \setlength{\abovecaptionskip}{0cm}
%     %\setlength{\belowcaptionskip}{-0.1cm}
%     \centering
%         % \caption{Performance comparison (F1-scores (\%)) on real-world datasets. The best performance is highlighted in bold.} 
%         \caption{Performance comparison (F1 (\%)) on the benchmark datasets, precision (Pre (\%)) and recall (Rec (\%)) are attached. }
%     %\begin{adjustbox}{width=\columnwidth,center}
%     %\setlength{\tabcolsep}{1.68mm}{
%     \begin{tabular}{cccccccccccccc}\\ \toprule
%                &   \multicolumn{3}{c}{\textbf{SWaT}} & \multicolumn{3}{c}{\textbf{WADI}} & \multicolumn{3}{c}{\textbf{HAI}} & \multicolumn{3}{c}{\textbf{MSL}} \\ \midrule
%                \textbf{Methods} & \textbf{F1} &  \textbf{Pre} & \textbf{Rec} & \textbf{F1} &  \textbf{Pre} & \textbf{Rec} & \textbf{F1} &  \textbf{Pre} & \textbf{Rec}  & \textbf{F1} &  \textbf{Pre} & \textbf{Rec}    \\ \midrule
% DAGMM              &  70.17 &  69.96 &  77.07 &  43.68 &  53.50 &  38.42 &  34.95 &  43.81 &  39.21 &  80.96 &  76.96 &  85.73 \\
% DeepSVDD           &  86.41 &  96.68 &  78.16 &  45.37 &  77.44 &  34.30 &  35.36 &  31.08 &  50.39 &  81.03 &  76.99 &  86.87 \\
% LSTM-VAE           &  81.90 &  97.95 &  70.42 &  64.70 &  66.53 &  62.99 &  69.41 &  64.90 &  77.46 &  88.40 &  87.55 &  89.70 \\
% USAD               &  84.60 &  \textbf{98.70} &  74.02 &  61.74 &  84.49 &  48.65 &  74.93 &  83.48 &  68.43 &  92.72 &  88.10 &  \textbf{97.86} \\
% MAD-GAN            &  80.44 &  97.31 &  68.77 &  74.09 &  \textbf{90.23} &  62.96 &  20.94 &  29.06 &  37.45 &  76.45 &  80.66 &  76.55 \\
% TranAD             &  83.17 &  97.39 &  72.61 &  41.05 &  69.83 &  29.91 &  73.93 &  \textbf{88.60} &  64.70 &  91.55 &  90.41 &  92.73 \\
% LNT                &  86.36 &  94.95 &  79.34 &  35.55 &  74.20 &  24.77 &  54.43 &  72.23 &  48.51 &  90.50 &  91.28 &  89.84 \\
% AnomalyTrans &  91.34 &  91.87 &  \textbf{90.82} &  69.00 &  75.41 &  63.59 &  58.02 &  63.33 &  55.26 &  93.97 &  92.75 &  95.25 \\
% \midrule
% CNT &  \textbf{91.68} & 96.50 & 87.33 &  \textbf{81.61}	& 82.39	& \textbf{81.19}   & \textbf{83.95} & 81.48 & \textbf{87.75} &  \textbf{95.13}&	\textbf{96.06}&	94.26 \\
%    \bottomrule
%     \end{tabular}
%     %}
%     %\end{adjustbox}
%     \label{tab:comparison_result_f1}
%     %\vspace{-0.8cm}
% \end{table*}













% Both the sequence-level contrasting objective and the neural transformation learning objective can effectively collaborate to enhance anomaly detection performance. 

% Furthermore, we assessed model performance using VUS\_PR and VUS\_ROC metrics on recent state-of-the-art time series models. While the ranking of all models slightly shifts compared to the F1 score, our approach still maintains consistently high performance across the majority of datasets. (need to be modified)
%only falling behind TranAD on MSL datasets and LNT on SWaT. 

% This outcome could be attributed to our use of the TCN encoder, which may be less capable of capturing global characteristics compared to the Transformer used in TranAD. As such, the design of a more effective base feature encoder is a direction for our future research.

% This could be attributed to its strategy of minimizing the distance between the transformations of point-wise future predictions and the context window, a method that may fail to preserve identical semantic meanings. Conversely, our model leverages a sequence-to-sequence comparison where the suspect and context sequences share semantically meaningful features owing to their overlap and shared feature encoder.


% our model achieves the highest F1 for all datasets. In addition, Precision and Recall are also on average within the top 3. We also compare the performance based on recently proposed metrics, VUS\-ROC and VUS\-PR for the recent state-of-the-art methods, and the results show that our model outperforms them in the majority datasets while slightly falling behind LNT in terms of VUS\_ROC for swat.
% % However, our model's performance falls short on MSL and SMAP. This could be due to the majority of features in these datasets being one-hot encoded commands, making temporal encoding of sequences challenging for simple TCN layers that tend to mix all features through simple sum aggregation. On the other hand, graph-based models like GDN, which explicitly learn the relationship between features, have performed well on these datasets.

% Additionally, NCAD currently holds state-of-the-arts performance on MSL and SMAP due to its semi-supervised classification training schemes based on synthetic anomalies. While supervised training is known to be more effective when the underlying distribution of synthetic anomalies is similar to that of the true anomalies in the dataset, we can see that NCAD performed relatively worse in WADI, HAI, and SMD compared to our methods, suggesting potential overfitting due to these datasets having a variety of different anomaly types beyond the injected ones.

% ON the other hand, LNT, a similar model to ours, showed inferior performance compared to our model, possibly because it attempts to minimize the distance between the transformation of point-wise future predictions and the context window, which may not have identical semantic meanings. In contrast, our model employs a sequence-to-sequence comparison, where the suspect and context sequences share semantically meaningful features due to their overlap and shared feature encoder.


%\subsection{Extended Investigation}
% \subsubsection{Sensitivity of Hyper-parameters}
% In this section we conduct the sensitivity analysis on three hyper-parameters, the sizes of the sliding window $w$, the predict window $p$, and the number of transformations $K$, primarily based on SWaT and MSL datasets with each parameter setting result averaged over 5 runs. Figure~\ref{fig: sensitivity_results}a illustrates the F1 score’s correlation with the sliding window size, with the predict window size held constant at 5. We can see a relatively higher performance when the sequence length lies between 20 and 60. This finding is consistent with the performance of other baseline models (e.g., TranAD, MTAD-GAT, and LNT), which also obtain optimal performances by adopting a sequence length within this range. Figure~\ref{fig: sensitivity_results}b explores the F1 score’s variability in response to different predict window sizes, while maintaining the sliding window size at 30. The model exhibits peak performance for prediction window sizes between 3 and 5 and experiences a noticeable decline when the size exceeds 9. This trend is logical, as larger prediction window sizes can smooth out the effect of anomalies (Most anomalies in the benchmark datasets are short-lived), reducing their distinctiveness from normal sample scores. Figure~\ref{fig: sensitivity_results}c portrays the F1 score's responsiveness to varying numbers of transformations. The optimal performance is observed at approximately $K=6$, with some performance fluctuations across other values. 
% \begin{figure*}[h]
% %\centering
% % \begin{subfigure}[b]{1\linewidth}
% %     \centering
% %      % \includesvg[height=4.2cm]{figures/swat_ts_unidentified_event1.svg}
% %     \includegraphics[height=0.5cm]{figures/neural_contrast/legend.eps}
% %     %\caption{}
% %    % \label{fig: win_size_results}
% % \end{subfigure}
% %\newline
% %\vspace{0.5cm}
% %\centering
% \begin{subfigure}[b]{.32\linewidth}
%     \centering
%     \includegraphics[height=2.4cm]{figures/neural_contrast/seq_len_results.eps}
%     %\caption{F1 vs. sliding window size}
%     \label{fig: seq_len_results}
% \end{subfigure}
% \begin{subfigure}[b]{.32\linewidth}
%     \centering
%     \includegraphics[height=2.4cm]{figures/neural_contrast/win_size_results.eps} 
%     %\caption{F1 vs. predict window size}
%     \label{fig: win_size_results}
% \end{subfigure}
% \begin{subfigure}[b]{.32\linewidth}
%     \centering
%     \includegraphics[height=2.4cm]{figures/neural_contrast/n_transformations_results.eps} 
%     %\caption{F1 vs. \# transformations}
%     \label{fig: n_transformations_results}
% \end{subfigure}
% \caption{(a) Average F1 versus sliding window size $w$ from 20 to 100; (b) Average F1 versus predict window size $p$ from 1 to 11; (c) Average F1 versus number of transformations $K$ from 2 to 12.}
% \label{fig: sensitivity_results}
% \end{figure*}


==> subtexes/experiments_v5.tex <==
%\section{Experiment}
\subsection{Datasets and Experimental Setup}
\begin{table}[H]
    \vspace{-0.8cm}
%\small
    %\setlength{\abovecaptionskip}{0cm}
    %\setlength{\belowcaptionskip}{-0.1cm}
    \centering
    \caption{Summary statistics for datasets} 
    \begin{tabular}{ccccc}\\ \toprule
               \textbf{Dataset} & \textbf{\# Channels} & \textbf{\# training} & \textbf{\# test} & \textbf{\% anomalies} \\ \midrule
   SWaT  &  51         &  495000   & 449919 & 12.14      \\
   WADI       &  123         &  784571    & 172801 & 5.77     \\  
%         SMAP       &   25        & 135183 & 427617 & 12.79     \\  

      MSL       &   55        & 58317 & 73729 & 10.53     \\
%    SMD       & 38         &  25300   & 25300 & 4.21    \\  

   HAI       & 79         &  921603   & 270003 & 1.93    \\  
%    TODS  & 1   & 40000 & 20000 & 2.50 \\
   \bottomrule
    \end{tabular}
    \label{tab:data_statistics}
    %\vspace{-0.8cm}
\end{table}
Four industrial real-world datasets, as shown in Table~\ref{tab:data_statistics}, are adopted for the evaluation of time series anomaly detection methods, which are SWaT~\cite{mathur2016swat}, WADI~\cite{ahmed2017wadi}, HAI~\cite{hai21.03}, and MSL~\cite{lstm-ndt}. Each dataset has a unlabeled training set, and a separate test set with anomalies. SWaT and WADI are released by iTrust Center~\footnote{\url{https://itrust.sutd.edu.sg/itrust-labs_datasets/dataset_info/}} to support research in cybersecurity. The SWaT dataset is collected from a scaled-down, secure water treatment testbed. The WADI dataset is collected from a small-scale water distribution network. The HAI dataset derives from an Industrial Control System testbed enriched with a Hardware-In-the-Loop simulator. As a common pre-processing step similar to~\cite{gdn}, the training and test sets of the above three datasets have been down-sampled to 10-second intervals using median values with anomaly labels assigned 0 or 1 by taking the mode. MSL, published by NASA, contains telemetry anomaly data from Mars Science Laboratory rover. The data contains multiple entities, which are concatenated into one time series for both training and testing.

% Four industrial real-world datasets, as shown in Table~\ref{tab:data_statistics},  are adopted for the evaluation of time series anomaly detection methods, which are SWaT~\cite{mathur2016swat}, WADI~\cite{ahmed2017wadi}, HAI~\cite{hai21.03}, and MSL~\cite{lstm-ndt}. Each dataset has a unlabeled training set, and a separate test set with anomalies. SWaT and WADI are released by iTrust Center~\footnote{\url{https://itrust.sutd.edu.sg/itrust-labs_datasets/dataset_info/}} to support research in cybersecurity. The SWaT dataset is collected from a scaled-down, secure water treatment testbed, featuring a 51-dimensional multivariate time series from 11 days of continuous operation. The first 7 days reflect normal operations (training set) and the last 4 days contain cyber attack data (test set). Similarly, the WADI dataset, collected from a small-scale water distribution network, includes 123 sensor and actuator time series from a 16-day run, with normal operations in the first 14 days (training set) and cyber attacks in the last 2 (test set). HAI dataset derives from an Industrial Control System testbed enriched with a Hardware-In-the-Loop simulator, featuring processes like boiler, turbine, water treatment, and steam-turbine power generation. As a common pre-processing step similar to~\cite{gdn}, the training and test sets of the above three datasets have been down-sampled to 10-second intervals using median values with anomaly labels assigned 0 or 1 by taking the mode. MSL, published by NASA, contains telemetry anomaly data from Mars Science Laboratory rover. The data contains multiple entities, which are concatenated into one time series for both training and testing.
% Four industrial real-world datasets are adopted for the evaluation of time series anomaly detection methods, which are SWaT~\cite{mathur2016swat}, WADI~\cite{ahmed2017wadi}, HAI~\cite{hai21.03}, and MSL~\cite{lstm-ndt}. Each dataset has a unlabeled training set, and a separate test set with anomalies. More detailed descriptions of the datasets as well as summary statistics are shown in \textbf{Section 4} of the supplementary materials.

% Given the limited space, we present the experimental setting and the sensitivity analysis of hyper-parameters in \textbf{Section 4\&1.5} of the supplementary materials.


\subsection{Baseline Methods and Evaluation Metrics}
We compare our framework with common anomaly detection approaches as the baseline methods, including DeepSVDD~\cite{deepSVDD} and DAGMM~\cite{zong2018deep}, which are general anomaly detection deep learning-based models, and LSTM-VAE~\cite{lstm-vae}, MAD-GAN~\cite{mad-gan}, USAD~\cite{usad}, MTAD-GAT~\cite{mtad-gat}, LNT~\cite{lnt}, TranAD~\cite{tranAD}, NeuTralAD~\cite{neuralAD} and AnomalyTransformer~\cite{anomalyTransformer}, which are popular anomaly detection methods tailored specifically to time series data.

In line with previous studies~\cite{mtad-gat,omnianomaly,anomalyTransformer,tranAD}, we use the best F1-score as the main performance metric to evaluate the performance of anomaly detection. We follow the point-adjusting strategy suggested in \cite{omnianomaly}, which labels a whole anomaly segment as 1 as long as one of the points within the segment is detected as an anomaly. Since our primary contribution is not the development of a new thresholding method, we adopt this well-established practice to eliminate potential bias arising from selecting a specific thresholding method. This choice of reporting F1 scores ensures a fair and consistent comparison across all methods. 

\subsection{Comparison Study}
The results are presented in Table~\ref{tab:comparison_result_f1}. First, both DAGMM and DeepSVDD display relatively lower performance due to their base model which does not account for temporal information. On the other hand, models such as MTAD-GAT and AnomalyTransformer perform comparatively better across all datasets in terms of F1 score, a testament to their effective utilization of GNNs to capture inter-series relationships or the global characteristics of time series through Transformers. Yet, CNT outperforms all others with the highest F1 score across all datasets, thus demonstrating the best balance between Recall and Precision. In comparison to these approaches, which utilize either time series forecasting or reconstruction-based methods, our approach utilizes the distance of latent representation between input instance and their contextual information as a criterion to identify anomalies, which are more robust to noise and less likely to overfit the data.


\begin{table*}[t!]
%\small
    \setlength{\abovecaptionskip}{0cm}
    \centering
        \caption{Performance comparison (F1 (\%)) on the benchmark datasets, precision (Pre (\%)) and recall (Rec (\%)) are attached. }
    \begin{tabular}{cccccccccccccc}\\ \toprule
               &   \multicolumn{3}{c}{\textbf{SWaT}} & \multicolumn{3}{c}{\textbf{MSL}} & \multicolumn{3}{c}{\textbf{WADI}} & \multicolumn{3}{c}{\textbf{HAI}} \\ \midrule
               \textbf{Methods} & \textbf{F1} &  \textbf{Pre} & \textbf{Rec} & \textbf{F1} &  \textbf{Pre} & \textbf{Rec} & \textbf{F1} &  \textbf{Pre} & \textbf{Rec}  & \textbf{F1} &  \textbf{Pre} & \textbf{Rec}    \\ \midrule
DAGMM              &  82.3 &         90.6 &      75.8 &  81.0 &         77.0 &      85.7 &  43.7 &         53.5 &      38.4 &  34.3 &         41.3 &      39.0 \\
DeepSVDD           &  86.4 &         96.7 &      78.2 &  80.3 &         75.6 &      87.0 &  47.8 &         82.0 &      33.7 &  37.0 &         29.9 &      61.8 \\
LSTM-VAE           &  81.9 &         97.9 &      70.4 &  87.5 &         87.8 &      87.7 &  64.6 &         66.3 &      63.0 &  70.8 &         67.8 &      76.4 \\
USAD               &  83.0 &         97.3 &      72.4 &  60.0 &         74.4 &      60.0 &  35.6 &         66.9 &      26.5 &  73.6 &         87.7 &      65.5 \\
MAD-GAN            &  80.5 &         98.3 &      68.2 &  77.1 &         71.7 &      86.6 &  73.7 &         88.2 &      63.6 &  17.5 &         16.5 &      48.0 \\
MTAD-GAT           &  83.2 &         94.4 &      74.5 &  88.4 &         87.1 &      89.8 &  46.3 &         50.1 &      44.2 &  78.0 &         90.8 &      71.0 \\
TranAD             &  83.2 &         96.5 &      73.2 &  79.2 &         71.5 &      89.9 &  41.4 &         62.0 &      31.6 &  73.0 &         88.4 &      63.1 \\
NeuTralAD          &  90.6 &         91.3 &      90.1 &  60.6 &         46.8 &      86.4 &  54.2 &         61.9 &      50.3 &  48.4 &         41.8 &      64.7 \\
LNT                &  86.4 &  95.0 &  79.3 &  90.5 &  91.3 &  89.8 &  35.6 &  74.2 &  24.8 &  54.4 &  72.2 &  48.5 \\
AnomalyTransformer &  89.7 &         92.1 &      87.5 &  93.9 &         91.8 &      96.1 &  69.5 &         74.9 &      64.9 &  57.4 &         61.0 &      56.6 \\
\midrule
CNT &  \textbf{91.7} & 96.5 & 87.3 & \textbf{95.1} & 96.1&	94.3&  \textbf{81.6}	& 82.4	& 81.2   & \textbf{84.0} & 81.5 & 87.8  \\
   \bottomrule
    \end{tabular}
    \label{tab:comparison_result_f1}
\end{table*}
It is worth noting that while CNT is built on top of NeuTralAD, it surpasses NeuTralAD in performance by a significant margin. One key contribution to this enhanced efficacy is that NeuTralAD and CNT diverge in their approach to transformation diversity and semantic relevance. Specifically, NeuTralAD aims to learn a diverse set of transformations semantically associated with a given input time window. In other words, it focuses more on capturing the characteristics of the whole window. This can sometimes dilute anomaly effects, especially when the dominant data trends within the window are normal. In contrast, CNT enforces semantic similarity among learned transformations relative to a context window. It concentrates more on deviations between a short predict window and its historical observations. Additionally, CNT introduces a notable computational advantage. Unlike NeuTralAD, which requires multiple passes of the transformations over the raw time series data, CNT applies the feature encoder a single time to the latent space, creating transformations more efficiently (see the computational analysis in Section~\ref{sec: computation analysis}). 


Lastly, the LNT model, though conceptually similar to CNT, lags in performance. LNT combines CPC loss with neural transformation learning, relying on negative sample selection which can bias the training due to the prevalence of normal samples. Our CNT model avoids this with a negative-free training strategy, leveraging discriminative contrastive loss to prevent representation collapse.


\subsection{Ablation Study}
\label{section: ablation}
In this section, we aim to verify whether each component does contribute to our final performance. Specifically, we test the following two settings: 
1) CCL: Here, $g(\cdot)$ is trained exclusively under the contextual contrastive loss in Eq.~\eqref{eq. raw contextual one-class objective}. 
2) DCL: The feature encoder network $g(\cdot)$ is trained purely under the discriminative contrastive loss in Eq.\eqref{eq. contextual discriminative contrastive loss}. It's akin to NeutralAD, but transformations are applied to the feature encoder output rather than the original sequence. We also present the results of more settings, including CCL with negative samples, and a variety of negative-sample-free regularizations inspired by BYOL, Simsiam, and VICReg in Section 2.1 of the supplementary materials.

Table~\ref{tab:ablation_result} presents the results of our experiments. The CCL setting is designed to assign similar representations to normal sequences in close proximity, but its performance falls short in comparison to our proposed approach. This can potentially be attributed to the representation collapse problem, wherein the loss function leads the encoder to converge to a parameter space that closely approximates the constant encoder solution. Consequently, the model may fail to capture the rich semantic information of normal sequences. On the other hand, The DCL configuration primarily encourages similarity between an in
\begin{table}{r}{6cm}
%\small
   %\vspace{-0.4cm}
    \setlength{\abovecaptionskip}{0cm}
    %\setlength{\belowcaptionskip}{-0.1cm}
    \centering
    \caption{Performance comparison (F1 (\%)) for ablation study.} 
    \begin{tabular}{ccccccc}\\ \toprule
     \textbf{Settings} & \textbf{SWaT} & \textbf{MSL}  & \textbf{WADI} & \textbf{HAI} \\ \midrule
  % Default             &  91.99     &  \\ \midrule
CNT    & \textbf{91.7} & \textbf{95.1} & \textbf{81.6} & \textbf{84.0}\\ \midrule
DCL     &  85.1 &  81.2 &  30.4 &  67.5 \\
CCL &  88.0 &  91.5 &  66.2 &  64.2 \\
   \bottomrule
    \end{tabular}
    \label{tab:ablation_result}
    %\vspace{-0.3cm}
\end{table}
put time window and its corresponding transformed sequences, prioritizing the modeling of characteristics across the entire time window. Consequently, anomalies within short time spans may be overlooked, resulting in negligible distance scores between the time window and its transformations, particularly for longer time windows. In contrast, our default setting emphasizes the discrepancy between the predict window and the context window, thereby enhancing accurate anomaly detection within the overlapping region.


%\section{Extended Investigations}
\subsection{Data Visualization}
\begin{figure}[h]
    \centering
   % \includesvg[width=1\linewidth]{figures/Framework.svg}
        \includesvg[height=9.5cm]{figures/neural_contrast/tods_case_study_more.svg}
        % \includegraphics[height=8cm, width=11.5cm]{figures/neural_contrast/showcases_tods.svg}

        \caption{A visual comparison among CNT, DCL, and CCL Models based on the TODS dataset. The top row shows the original time series with anomalies. Subsequent rows illustrate the corresponding anomaly scores from the CNT, DCL, and CCL models.}
    \label{fig: tods showcase}
%\vspace{0.5cm}
\end{figure}
We further conducted experiments on a univariate dataset (TODS) generated from the rules outlined in~\cite{tods}. The TODS dataset adopts a sinusoidal wave as the base shapelet to generate a univariate time series, and synthetic anomalies of various types are injected using predefined rules. Examples of different types of anomalies are shown in Figure~\ref{fig: tods showcase}. TODS is specifically chosen for data visualization as it offers clearly classified anomalies of different types, enabling a better understanding of the performance of our method. Furthermore, the univariate nature of the dataset makes it easy to visualize the results directly from the plot.
% , and summary statistics of the data are shown in Table~\ref{tab:data_statistics}

Figure~\ref{fig: tods showcase} provides a visual comparative analysis of anomaly detection performances among the CNT, DCL, and CCL models. The first row reveals the original time series data, featuring various types of anomalies such as shapelet, seasonal, and trend-based disturbances, excluding point anomalies for their consistent detection across models. CNT distinguishes itself by generating distinctly elevated anomaly scores in areas of anomalies, demonstrating exceptional sensitivity to aberrant patterns. DCL, however, shows a reduction in performance, particularly with trend anomalies where its scores fail to capture the irregularities effectively, hinting at a potential under-detection of nuanced anomalies in predominantly normal data streams. CCL, while producing sharper scores than DCL, does not achieve the same level of discrimination as CNT, occasionally misidentifying normal regions as anomalous. This underperformance is likely a consequence of the representation collapse issue, wherein the feature encoder defaults to oversimplified representations that overlook temporal dynamics within the data. Overall, CNT demonstrates a superior capacity to detect a wide range of anomalies with its discriminative scoring, while the DCL and CCL models appear constrained by their focus on broader patterns and a vulnerability to representation collapse, respectively.


\subsection{Analysis Of Learning Situations}
In Section~\ref{sec:theoretical analysis}, we show that simply using 
$L_{\text{ccl}}$ could lead to the representation collapse issue, where the feature representations of the context window and the predict window collapse to the same constant. Then we proved that under the assumption that $L_{\text{dcl}}<K\log{K}$, this situation does not apply to the case when we combine the CCL and DCL losses. 
Figure~\ref{fig: loss_decay} shows the loss values per epoch for our model training under purely $L_{\text{ccl}}$ loss or training under both $L_{\text{cncl}}$ and $L_{\text{dcl}}$ (the default setting). It is clear that $L_{\text{ccl}}$ decays quickly to 0 without the regularization of $L_{\text{dcl}}$, which agrees with Proposition~\ref{props: constant encoder}. In contrast, with the additional constraints of $L_{\text{dcl}}$, $L_{\text{cncl}}$ decays much slowly compared to the former. 
\begin{wrapfigure}{r}{6.5cm}
\vspace{-0.4cm}
\centering
\includegraphics[height=3.5cm]{figures/neural_contrast/loss_decay.eps}  
\caption{Provided the loss value per epoch with the model trained on the WADI dataset. The small window is the zooming region for loss values from 20 to 30 epochs.}
\label{fig: loss_decay}
\vspace{-0.3cm}
\end{wrapfigure}
This implies that $L_{\text{dcl}}$ does add additional complexity to the CCL task, preventing from learning trivial feature representations. This is also verified in our ablation study that the combination of both losses can obtain a much higher performance than using $L_{\text{ccl}}$ only. Furthermore, as shown in Figure~\ref{fig: loss_decay}, we can see that the loss value of $L_{\text{dcl}}$ quickly falls below $K\log K$, which is around 4.67 when $K=6$ (the default parameter setting used in our experiments). This verifies the assumption in Proposition~\ref{props: non-constant encoder} is empirically applicable. 


\subsection{Computational Analysis}
\label{sec: computation analysis}
\begin{figure}[h]
\centering
\vspace{-0.2cm}
\includesvg[height=4cm]{figures/neural_contrast/computation_time.svg}
\caption{The training time per epoch and inference time of each model based on the SWaT dataset.}
\label{fig: computation_time}
\end{figure}
Figure~\ref{fig: computation_time} provides a comparison of the computational demands for various models, including both training time per epoch and inference time, benchmarked on the SWaT dataset. To ensure consistency across models, we maintained the same batch size during the training and testing phases. CNT demonstrates a considerable reduction in both training and inference times relative to other models, particularly NeutralAD. The efficiency of CNT can be attributed to its approach of applying transformations to the hidden representations - outputs of a feature encoder - rather than operating directly on the input data. This design choice means that CNT requires only a single pass of the data through the feature encoder, irrespective of the number of transformations applied, in stark contrast to NeutralAD, which must repeatedly process the input data for each transformation, incurring high computational overhead. Additionally, the observed computational efficiency in models like USAD, DeepSVDD, and DAGMM can be rationalized by their reliance on simpler MLP-based feature encoders, which are inherently less computationally intensive than more complex architectures.




==> subtexes/introduction.tex <==
\section{Introduction}
Time series anomaly detection is a critical tool in industrial applications, helping to detect abnormal behavior in complex systems and prevent costly failures. With the rise of data-driven industries, identifying anomalous patterns in real-time monitoring and analysis of sensor data is becoming increasingly important. By detecting anomalies, industries can improve production efficiency, reduce downtime, and enhance the safety and reliability of their systems.

Detecting anomalies in temporal data presents unique challenges compared to traditional anomaly detection tasks, as anomalies in temporal data are often context-dependent, meaning that they are contingent upon the temporal dynamics of the system. As shown in Figure~\ref{fig: msl_contextual_anomalies}, anomalies in temporal data may occur within normal value ranges, but they represent events that deviate from their expected behavior given the dynamic temporal context in which they occur. Thus, an effective time series anomaly detection method needs to capture the context-aware nature of anomalies and the temporal dependencies within the data.

One-class classification methods are widely used in anomaly detection tasks, with the objective of learning a model of normal data and identifying anomalies as data points outside this model. Examples of these methods include Support Vector Data Description (SVDD)~\cite{svdd} and one-class SVM~\cite{ocsvm}, which respectively construct a hypersphere or a hyperplane around the normal data. However, such methods are computationally expensive in dealing with complex data structures and high-dimensional data, and often require substantial feature engineering. To address these challenges, deep learning-based one-class classification methods have been developed to learn more complex representations of normal data. One popular method in this category is DeepSVDD~\cite{deepSVDD}, which employs a deep neural network to map the input data into a high-dimensional feature space and learns a hypersphere that encapsulates the normal data. 

\begin{figure*}[t!]
    \centering
       % \includesvg[height=2.3cm]{figures/neural_contrast/msl_contextual_anomalies.svg}  
                \includegraphics[height=2.3cm]{figures/neural_contrast/msl_contextual_anomalies.eps}  

    \caption{The figure presents several examples of time series segments from a real-world industrial dataset, with anomalies highlighted in yellow. Contextual information plays a crucial role in identifying these anomalies.}
    \label{fig: msl_contextual_anomalies}
\end{figure*}
While one-class classification methods have demonstrated success in detecting anomalies in various scenarios such as computer vision, they exhibit a tendency to map all data points to a single center point or region in the feature space, which limits their efficacy in detecting anomalies in time series data. This is particularly relevant as time series data often display intricate and nonlinear temporal patterns, and the majority of anomalies in time series data are context-specific, i.e., they deviate from recent past observations. Consequently, a single global representation of normal behavior may not be able to fully capture the complex and context-specific nature of anomalies in time series data. 

 Recent research has proposed several approaches to extend DeepSVDD for time series anomaly detection. For instance, COUTA~\cite{couta} and COCA~\cite{coca} use TCNs and LSTMs, respectively, to capture temporal patterns in time series data, while OCPAE~\cite{OCPAE} incorporates time series forecasting and sequence reconstruction objectives along with a one-class classification objective to account for local temporal dependencies. However, these methods still has the limitation of mapping all latent representations of normal instances into a single hypersphere. In contrast, THOC~\cite{thoc} uses a dilated RNN with skip connections to encode time series data, and clusters features from all intermediate layers into multiple clusters, allowing for the representation of normal behaviors by multiple hyperspheres. However, selecting the appropriate number of $k$ centers remains a challenge.


In this work, we propose a novel adaptation based on the original loss function of DeepSVDD. Instead of converging all normal instances towards a single center, we propose a contextual-based loss function that pulls the latent representation of each instance toward its context. The underlying assumption is that nearby sequences should share similar latent representations, while anomalous instances should exhibit significant dissimilarity from their neighbors. This approach enables more precise identification of anomalous instances than traditional one-class methods, which often fail to account for the temporal characteristics and contextual nature of anomalies.

However, our proposed approach, like DeepSVDD, may be susceptible to a representation collapse issue, where the neural network encoding a given instance and its context may be optimized towards a constant encoder solution. To address this issue, we augment our approach with a deterministic contrastive loss from the recent self-supervised learning-based anomaly detection approach, Neural AD~\cite{neuralAD}, which has demonstrated success in various data types. The deterministic contrastive loss applies regularizations to the transformations of an input sequence to guarantee diverse and semantically meaningful latent representations of the sequences. 

In summary, our contributions are threefold:
\begin{enumerate}
\item We propose a novel anomaly detection framework that considers the contextual nature of temporal anomalies through a combination of contextual contrastive loss and deterministic contrastive loss.
\item We provide theoretical analysis demonstrating that a combination of the two losses effectively mitigates the representation collapse problem.
\item We conduct extensive experiments on real-world industrial datasets, including comparison studies, ablation studies, and visual analysis, that demonstrate the superior performance of our proposed approach over various baseline methods and variants of our model.
\end{enumerate}

==> subtexes/introduction_v2.tex <==




Time series anomaly detection is a critical tool in industrial applications. By detecting anomalies, industries can improve production efficiency, prevent costly failures, reduce downtime, and enhance the safety and reliability of their systems. Despite its potential, the effectiveness of time series anomaly detection is often hampered by several inherent challenges. Firstly, the infrequent occurrence of anomalies combined with the costly and time-consuming nature of their labeling can make supervised techniques less feasible~\cite{choi2021deep}. Moreover, the intricate properties of time series data, such as its high dimensionality, temporal dependencies, and non-stationarity, further complicate the detection process~\cite{yang2021pipeline}. Given these challenges, there has been a growing inclination towards unsupervised learning methods. Additionally, deep learning models, with their capability to handle complex data structures and patterns, have emerged as a preferred choice for many researchers and practitioners.


% Despite its potential, the effectiveness of time series anomaly detection is often hampered by several challenges. Firstly, the infrequent occurrence of anomalies combined with the costly and time-consuming nature of their labeling complicates the application of traditional supervised learning schemes~\cite{choi2021deep}. This situation has fostered a general preference for unsupervised learning approaches, relying on the assumption that the majority of training data represents normal behavior. Secondly, the intrinsic properties of time series data - high dimensionality, temporal dependencies, and non-stationarity - add additional layers of complexity to the accurate identification of anomalies~\cite{yang2021pipeline}.  



Current deep learning-based unsupervised time series anomaly detection primarily includes forecasting-based~\cite{lstm-ndt,tcnanomaly,gdn,mtad-gat}, reconstruction-based~\cite{mad-gan,usad,tranAD,lstm-vae,lstmed,anomalyTransformer}, and one-class-based approaches~\cite{OCPAE,coca,deepSVDD,couta}, each operating under a different set of assumptions. Forecasting-based methods assume normal instances are predictable, but their performances can falter when temporal patterns are unpredictable or rapidly changing~\cite{lstmed}. Reconstruction-based approaches, founded on the principle that normal instances can be accurately reconstructed, can run into issues for which anomalies are also well-reconstructed due to the infrequent presence of them in the training data. One-class-based methods posit that normal data points can be enclosed within a certain region, such as a hypersphere, in the feature space~\cite{deepSVDD}. However, such a singular, global representation of normal behavior may fail to capture the intricacies and context-specific characteristics of anomalies in time series data.

Recently, self-supervised contrastive learning has attracted considerable attention due to its ability to mine valuable representations from unlabelled data. Its application has also extended to time series forecasting, where a growing number of proposed methods have consistently outperformed traditional supervised learning approaches~\cite{ts-tcc,cost,ts-tfc,tnc}. At the core of contrastive learning is its goal to learn feature representations by pulling similar instances together while pushing dissimilar instances away~\cite{cpc}. However, applying this paradigm to time series anomaly detection has its own unique challenges. Firstly, classical contrastive learning often selects dissimilar samples from the same training set. This can become problematic in anomaly detection where the training set predominantly comprises normal samples~\cite{coca}. Besides, randomly selecting a large number of negative samples is also computationally expensive. 
Secondly, most contrastive learning techniques adopt the instance discrimination-based approach, which treat an instance with its augmented version as a positive pair. When applying this to time series anomaly detection, an intuitive adaptation is to calculate anomaly scores based on the distance between a sliding window and its augmented version. Since this approach emphasizes capturing temporal characteristics across entire windows, short-lived temporal anomalies might not be effectively captured.

In this study, we introduce a novel contrastive learning approach specifically tailored for time series anomaly detection. This method utilizes a time window-based strategy where each instance is defined by a predict time window and compared with a corresponding context window, which is an overlapping time period including past data. We hypothesize that under normal circumstances, the latent representations of the predict and context windows would exhibit high similarity due to their shared data segment. Anomalies are discerned when there is a significant divergence in the non-overlapping region of these windows, which can be minimized to ensure a short detection delay.

However, merely aligning the latent representation of the predict window with that of the context window can lead to the representation collapse issue: the feature encoders of both windows produce constant representations irrespective of their input, a phenomenon akin to the hypersphere collapse in~\cite{deepSVDD}.
A common solution, as in contrastive learning, is to push away other samples in a batch to ensure a uniform distribution of representations~\cite{wang2020understanding}. This method, however, could introduce a bias when training sets are predominantly comprised of the same class (i.e., normal instances). Other strategies include the imposition of non-zero variance constraints on the feature representations~\cite{vicreg} or applying a stopping gradient criterion on the target representations to be pulled against~\cite{simsiam,byol}. Unlike those approaches that focus on enforcing non-constant representations on input instances, our approach augments the window-based contrastive loss with the neural transformation loss proposed by~\cite{neuralAD}. Specifically, a set of learnable augmentations is applied to the input time window, resulting in a range of transformations that are diverse yet semantically consistent with the original inputs. By pitting these transformations against the context window, we not only circumvent the issue of constant encoder solution but also bolster the efficacy of our window-based contrastive approach by adding complexity to the training process.

We summarize our contributions as follows:
\begin{enumerate}
\item We propose a novel time series anomaly detection framework, CNT, based on the idea of contrastive learning. The approach is specifically tailored for the detection of temporal anomalies through a combination of window-based contrastive loss and neural transformation loss.
\item We provide theoretical analysis demonstrating that a combination of the window-based contrastive loss and the neural transformation loss effectively mitigates the representation collapse problem.
\item We conduct extensive experiments on real-world industrial datasets to demonstrate the superior performance of our proposed approach over various baseline methods and variants of our model.
\end{enumerate}


% With the rise of data-driven industries, identifying anomalous patterns in real-time monitoring and analysis of sensor data is becoming increasingly important. 
%{\color{red} basically saying the same thing}

% However, simply pulling the latent representation of the predict window towards that of the context window suffers from the representation collapse issue, a situation where the feature encoder of the predict and context windows generate constant representations regardless of the input (similar to the hypersphere collapse in~\cite{deepSVDD}).

% the majority of contrastive learning adopts the instance discrimination-based approach~\cite{wu2018unsupervised}, which focuses on capture the temporal characteristics of a long time window. However, this may overlook anomalies that appear shortly overtime.
% Secondly, minimizing detection delay is critical in time series anomaly detection. However, the traditional instance discrimination-based contrastive learning~\cite{wu2018unsupervised} can introduce delays, as it requires waiting for a long time window to capture data's temporal patterns, hindering timely anomaly detection.
% Secondly, minimizing detection delay in time series anomaly detection is crucial. Hence, the instance discrimination-based contrastive learning~\cite{wu2018unsupervised} may be less applicable due to their reliance on long time windows for capturing the temporal patterns within the data.

==> subtexes/introduction_v3.tex <==
Time series anomaly detection (TSAD) plays a pivotal role in a wide range of applications, spanning from finance and healthcare to industrial process monitoring and cybersecurity~\cite{anandakrishnan2018anomaly,liu2022arrhythmia,ren2019time,cook2019anomaly}. For instance, TSAD is instrumental in financial risk management, helping institutions identify unusual patterns and potential threats in financial data. Whereas in industrial process monitoring, it ensures optimal operational efficiency by swiftly detecting system irregularities.

Despite its potential, the effectiveness of TSAD is often hampered by several inherent challenges. Firstly, the infrequent occurrence of anomalies combined with the costly and time-consuming nature of their labeling can make supervised techniques less feasible~\cite{choi2021deep}. Moreover, the intricate properties of time series data, such as its high dimensionality, temporal dependencies, and non-stationarity, further complicate the detection process~\cite{yang2021pipeline}. This backdrop has intensified interest in unsupervised methods, with deep learning models emerging as a popular choice due to their ability to handle intricate data structures.

Deep learning-based unsupervised approaches for TSAD primarily focus on understanding the distribution of normal data through auxiliary tasks. Current TSAD methods primarily include forecasting-based and reconstruction-based approaches. The former assume normal instances are predictable, but their performances can falter when temporal patterns are unpredictable or rapidly changing~\cite{lstmed}. The latter, despite not depending on sample extrapolation, can run into overfitting issues due to an undue emphasize on pixel-wise reconstructions. Recently, contrastive learning has emerged as a significant area of interest in various domains~\cite{he2020momentum,chen2020simple,saeed2021contrastive,shi2019deepchannel}, lauded for its capability to distill valuable feature representations from data. Unlike traditional approaches, contrastive learning operates on the latent feature space, advocating for the alignment of similar instances and the segregation of dissimilar ones. Given its powerful representation learning ability, some researches have applied it to solve the anomaly detection problem and have shown promising results, particularly in Computer Vision (CV) domain~\cite{geoTransformation,robustAndUncertainty,inlier}. 

Yet applying contrastive learning to TSAD presents unique challenges. First, in contrastive learning, the task of constructing similar positive samples is usually accomplished by augmenting a sample using data-specific transformations, such as geometric alterations for images (e.g., cropping and rotating)~\cite{geoTransformation}. However, designing transformations for time series data to constitute ``similar'' instances isn't straightforward, given its complex temporal interdependencies. 
Moreover, the conventional paradigm of deriving negative samples from training data in contrastive learning is ill-suited for anomaly detection, where the majority of the training dataset consists of normal instances~\cite{coca}. Adding another layer of complexity,  time series anomalies heavily lean on contextual rather than individual data. The core objective remains to detect anomalous patterns that deviate a lot from historical observations. Thus, it is crucial to understand each instance in relation to its contextual backdrop.

To address the aforementioned challenges, we propose a simple but effective time series anomaly detection method, CNT, which synergizes the idea of temporal-wise contrasting learning with the neural transformation learning framework~\cite{neuralAD}. First, motivated by several recent works (e.g., ~\cite{cpc,ts-tcc}) that adopt a temporal-wise contrasting framework - the latent representation of future time points can be predicted from that of the historical observations, we utilize a time window-based strategy where each instance is defined by a predict time window and is pulled closer to a corresponding context window, a window that containing past information, through a contextual contrastive loss. We hypothesize that under normal circumstances, the latent representations of the predict and context windows would exhibit high similarity due to their shared data segment. Anomalies are discerned when there is a significant divergence in the non-overlapping region of these windows, which can be minimized to ensure a short detection delay. 

However, this alignment alone can usher in the ``representation collapse'' issue: the feature encoders of both windows produce constant representations irrespective of their input, a phenomenon akin to the hypersphere collapse in~\cite{deepSVDD}. In traditional contrastive learning, this issue is often circumvented by using negative samples, ensuring diversity in the learned representations. To avoid wrongly selecting negative samples within the same normal class (given that the majority of samples are normal within training data), we directly augment the temporal contrastive loss with a discriminative contrastive loss proposed in NeuTralAD~\cite{neuralAD}. Specifically, a set of learnable augmentations is applied to the latent space of the predict window, resulting in a range of transformations that are diverse yet semantically consistent with the original inputs. It is imperative to understand that while CNT incorporates elements from existing methods, its distinction lies not in mere combination but in strategic integration tailored for TSAD. Theoretically, we demonstrate that pitting the learnable transformation of the predict window against the context window circumvents representation collapse issues. Whereas empirically, we demonstrate that this strategy significantly outperforms the individual performance of its constituent methodologies.


==> subtexes/introduction_v4.tex <==
Time series anomaly detection (TSAD) is vital in diverse sectors, such as industrial monitoring and cybersecurity, where it aids in identifying irregular patterns that may indicate critical events or system failures~\cite{ren2019time,cook2019anomaly}. However, its efficacy is often constrained by two primary challenges: the rarity of anomalies and the resource-intensive nature of obtaining accurate labels. These issues limit the practicality of supervised methods and drive the need for unsupervised TSAD approaches. Deep learning models excel in this regard, as they can learn complex feature representations without reliance on manual labeling.

Among unsupervised deep-learning methods, contrastive learning has captured significant interest across various fields such as Computer Vision (CV), audio processing, and Natural Language Processing (NLP), thanks to its ability to distill robust feature representations by contrasting similar and dissimilar instances~\cite{chen2020simple,saeed2021contrastive,shi2019deepchannel}. Particularly in CV, it has been leveraged to address anomaly detection challenges with promising outcomes~\cite{geoTransformation,robustAndUncertainty,inlier}. Yet applying contrastive learning to TSAD presents unique challenges. First, anomalies in time series data are context-dependent, necessitating an analysis that understands each instance in relation to its contextual backdrop. Secondly, standard contrastive learning requires the selection of negative samples in order to avoid a representation collapse - a scenario where a model converges to trivial solutions that map different inputs to indistinguishable representations. However, deriving negative samples from a pool of predominantly normal instances is ill-suited for anomaly detection. Additionally, the generation of ``similar'' positive samples through data augmentation, such as geometric transformations for images (e.g., cropping and rotating)~\cite{geoTransformation}, is not directly applicable to time series data due to their intricate temporal dependencies.

In this study, we propose a simple but effective time series anomaly detection method, CNT, to address the aforementioned challenges. Motivated by Contrastive Predictive Coding (CPC)~\cite{cpc} - where the latent representation of future time points can be predicted from that of the historical observations - we implement a temporal-wise contrasting where each instance is defined by a predict time window and is pulled closer to a corresponding context window through a contextual contrastive loss. This strategy naturally discerns anomalies by highlighting significant divergences from historical patterns. To counter the absence of manual transformations and mitigate the risk of representation collapse, we adapt the temporal-wise contrasting to NeuTralAD~\cite{neuralAD} - a framework that alleviates the need for manual augmentation by generating a set of learnable, diverse and semantically rich transformations from data. Our theoretical analysis indicates that this duel-loss circumvents the issue of representation collapse without introducing negative samples. Unlike NeuTralAD which focuses on learning augmentations from raw time series at the instance level, CNT applies the transformation at the latent space, and contrastive learning occurs between each instance and its temporal context. Empirical results confirm CNT's superior performance, yielding higher F1 scores and better computational efficiency compared to NeuTralAD, as well as enhanced detection capabilities over other benchmarks across various real-world industrial datasets.

We summarize our contributions as follows:
\begin{enumerate}
\item We propose a novel time series anomaly detection framework, CNT, based on the idea of contrastive learning. The approach is specifically tailored for the detection of temporal anomalies through a combination of window-based contrastive loss and neural transformation loss.
\item We provide theoretical analysis demonstrating that a combination of the window-based contrastive loss and the neural transformation loss effectively mitigates the representation collapse problem.
\item We conduct extensive experiments on real-world industrial datasets to demonstrate the superior performance of our proposed approach over various baseline methods and variants of our model.
\end{enumerate}


% To surmount these challenges, our approach adapts contrastive learning to the temporal nature of TSAD. We shift from instance-level to temporal-wise contrasting, which inherently considers the contextual relationship of data points. Leveraging a contextual contrastive loss, our method predicts the latent representation of future time points based on past observations, aligning instances within their temporal windows. This strategy naturally discerns anomalies by highlighting significant divergences from historical patterns. To counter the absence of manual transformations and mitigate the risk of representation collapse, we incorporate a discriminative contrastive loss from NeuTralAD~\cite{neuralAD}. Specifically, instead of learning transformations from raw time series data and focusing on contrasting augmentations with respect to a single instance, CNT applies the transformations on the latent space of data, and a temporal-wise contrasting is adapted to NeutralAD to enable the model to align diverse transformations of future instances with respect to their temporal context. Theoretical analysis and empirical results demonstrate CNT's superior performance, showcasing a notable margin in F1 scores across various datasets when compared to NeuTralAD and other benchmarks. 


% It introduces learnable augmentations in the latent space, enriching the feature space without requiring explicit negative samples. Our theoretical analysis further supports that this dual-loss framework precludes the need for traditional negative sampling.



% To address the aforementioned challenges, we propose a simple but effective time series anomaly detection method, CNT, which synergizes the idea of temporal-wise contrasting learning with the neural transformation learning framework~\cite{neuralAD}. First, motivated by the Contrastive Predictive Coding (CPC)~\cite{cpc} that adopt a temporal-wise contrasting framework - the latent representation of future time points can be predicted from that of the historical observations, we utilize a time window-based strategy where each instance is defined by a predict time window and is pulled closer to a corresponding context window (an example is shown in Figure~\ref{fig: notation_example}), through a contextual contrastive loss. We hypothesize that under normal circumstances, the latent representations of the predict and context windows would exhibit high similarity due to their shared data segment. Anomalies are discerned when there is a significant divergence in the non-overlapping region of these windows.

% However, this alignment alone can usher in the ``representation collapse'' issue: the feature encoders of both windows produce constant representations irrespective of their input, a phenomenon akin to the hypersphere collapse in~\cite{deepSVDD}. In a classic contrastive learning setting, this issue is often circumvented by using negative samples, ensuring diversity in the learned representations. To avoid wrongly selecting negative samples within the same normal class (given that the majority of samples are normal within training data), we directly augment the contextual contrastive loss with a discriminative contrastive loss proposed in NeuTralAD~\cite{neuralAD}. Specifically, a set of learnable augmentations is applied to the latent space of the predict window, resulting in a range of transformations that are diverse yet semantically consistent with the original inputs. Theoretically, we demonstrate that pitting the learnable transformation of the predict window against the context window circumvents representation collapse issues. Note that different from NeuTralAD, CNT focuses on the deviations between short predict windows and their historial context, sharpening the detection of contextual anomalies. Additionally, CNT generates transformations within the latent space, harnessing deeper data abstraction for more effective anomaly identification. Our experiments show that this simple adaptation significantly outperforms the performance of NeutralAD and also surpasses a variety of existing anomaly detection methods.





% Time series anomaly detection (TSAD) plays a pivotal role in a wide range of applications, spanning from finance and healthcare to industrial process monitoring and cybersecurity~\cite{anandakrishnan2018anomaly,liu2022arrhythmia,ren2019time,cook2019anomaly}. Despite its potential, the effectiveness of TSAD is often hampered by several inherent challenges. Firstly, the infrequent occurrence of anomalies combined with the costly and time-consuming nature of their labeling can make supervised techniques less feasible~\cite{choi2021deep}. Moreover, the intricate properties of time series data, such as its high dimensionality, temporal dependencies, and non-stationarity, further complicate the detection process~\cite{yang2021pipeline}. This backdrop has intensified interest in unsupervised methods, with deep learning models emerging as a popular choice due to their ability to handle intricate data structures.

% Deep learning-based unsupervised approaches for TSAD primarily include forecasting-based and reconstruction-based approaches. The former assumes normal instances are predictable, but their performances can falter when temporal patterns are unpredictable or rapidly changing~\cite{lstmed}. The latter, despite not depending on sample extrapolation, can run into overfitting issues due to an undue emphasis on pixel-wise reconstructions. In recent years, contrastive learning has emerged as a significant area of interest in various domains~\cite{he2020momentum,chen2020simple,saeed2021contrastive,shi2019deepchannel}, lauded for its capability to distill valuable feature representations from data. Unlike traditional approaches, contrastive learning operates on the latent feature space, advocating for the alignment of similar instances and the segregation of dissimilar ones. Given its powerful representation learning ability, some researches have applied it to solve the anomaly detection problem and have shown promising results, particularly in Computer Vision (CV) domain~\cite{geoTransformation,robustAndUncertainty,inlier}. 

% Yet applying contrastive learning to TSAD presents unique challenges. First, in contrastive learning, the task of constructing similar positive samples is usually accomplished by augmenting a sample using data-specific transformations, such as geometric alterations for images (e.g., cropping and rotating)~\cite{geoTransformation}. However, designing transformations for time series data to constitute ``similar'' instances isn't straightforward, given its complex temporal interdependencies. 
% Moreover, the conventional paradigm of deriving negative samples from training data in contrastive learning is ill-suited for anomaly detection, where the majority of the training dataset consists of normal instances~\cite{coca}. Adding another layer of complexity,  time series anomalies heavily lean on contextual rather than individual data. The core objective remains to detect anomalous patterns that deviate a lot from historical observations. Thus, it is crucial to understand each instance in relation to its contextual backdrop.

% To address the aforementioned challenges, we propose a simple but effective time series anomaly detection method, CNT, which synergizes the idea of temporal-wise contrasting learning with the neural transformation learning framework~\cite{neuralAD}. First, motivated by the Contrastive Predictive Coding (CPC)~\cite{cpc} that adopt a temporal-wise contrasting framework - the latent representation of future time points can be predicted from that of the historical observations, we utilize a time window-based strategy where each instance is defined by a predict time window and is pulled closer to a corresponding context window (an example is shown in Figure~\ref{fig: notation_example}), through a contextual contrastive loss. We hypothesize that under normal circumstances, the latent representations of the predict and context windows would exhibit high similarity due to their shared data segment. Anomalies are discerned when there is a significant divergence in the non-overlapping region of these windows.

% However, this alignment alone can usher in the ``representation collapse'' issue: the feature encoders of both windows produce constant representations irrespective of their input, a phenomenon akin to the hypersphere collapse in~\cite{deepSVDD}. In a classic contrastive learning setting, this issue is often circumvented by using negative samples, ensuring diversity in the learned representations. To avoid wrongly selecting negative samples within the same normal class (given that the majority of samples are normal within training data), we directly augment the contextual contrastive loss with a discriminative contrastive loss proposed in NeuTralAD~\cite{neuralAD}. Specifically, a set of learnable augmentations is applied to the latent space of the predict window, resulting in a range of transformations that are diverse yet semantically consistent with the original inputs. Theoretically, we demonstrate that pitting the learnable transformation of the predict window against the context window circumvents representation collapse issues. Note that different from NeuTralAD, CNT focuses on the deviations between short predict windows and their historial context, sharpening the detection of contextual anomalies. Additionally, CNT generates transformations within the latent space, harnessing deeper data abstraction for more effective anomaly identification. Our experiments show that this simple adaptation significantly outperforms the performance of NeutralAD and also surpasses a variety of existing anomaly detection methods.



% In this study, we propose a simple but effective time series anomaly detection method, CNT, to address the aforementioned challenges. Motivated by Contrastive Predictive Coding (CPC)--the latent representation of future time points can be predicted from that of the historical observations, we implement a temporal-wise contrasting where each instance is defined by a predict time window and is pulled closer to a corresponding context window, through a contextual contrastive loss. This strategy naturally discerns anomalies by highlighting significant divergences from historical patterns. To counter the absence of manual transformations and mitigate the risk of representation collapse, we adapt the temporal-wise contrasting to NeutralAD--a framework that alleviates the needs of manual augmentation by generating a set of learnable diverse and semantic transformations from data. 
% While NeuTralAD focuses on learning augmentations from raw time series at the instance level, CNT applies the transformation at the latent space and the contrastive learning occurs between each instance and its temporal context. This adaptation refines the sensitivity of the model to temporal anomalies. Theoretically, our analysis indicates that CNT circumvents the issue of representation collapse without resorting to negative samples. Empirical results substantiate the efficacy of CNT, revealing an improved F1 score compared to NeuTralAD and other benchmarks.


% Note that different from NeuTralAD, we adapt the learnable transformation on the latent space of input data, and contrastive learning is performed between the latent representation of the predict window with respect to its contextual backdrop. Theoretically, our analysis shows that this simple synergy can alleviate the representation collapse issue without the need to introduce negative samples, Additionally, empirical results reinforce the effectiveness of CNT, with F1 scores exhibiting a notable improvement over NeuTralAD and other benchmarks.





% % Those methods generally leverage various neural network architectures like MLPs~\cite{mad-gan,usad}, LSTMs~\cite{lstm-vae,lstm-ndt}, TCNs~\cite{tcnanomaly}, GNNs~\cite{mtad-gat}~\cite{gdn}, Transformers~\cite{gta,anomalyTransformer,anomalybert} to capture the temporal patterns within data, and the anomalies are identified based on the forecasting errors or reconstruction errors. Forecasting-based approaches

==> subtexes/introduction_v5.tex <==
% Time series anomaly detection (TSAD) is a crucial research area with applications across various industries~\cite{anandakrishnan2018anomaly,ren2019time,cook2019anomaly}. For instance, in device monitoring, TSAD is instrumental in identifying unusual machine behavior that may precede equipment malfunctions. and in cybersecurity, it helps in detecting atypical network activities that could be signs of security breaches. Despite the importance of TSAD, its efficacy is often constrained by the rarity of anomalies and the resource-intensive nature of obtaining accurate labels. These issues limit the practicality of supervised methods and drive the need for unsupervised TSAD approaches. Deep learning models excel in this regard, as they can learn complex feature representations without reliance on manual labeling. 

Modern industrial systems rely on Internet of Things (IoT) technology to facilitate communication and information exchange among different sub-systems and sub-processes. Due to the vast scale of these distributed systems, unanticipated events such as cyber-attacks can cause system downtime and may even lead to catastrophic failures~\cite{mohammadi2018deep}~\cite{gdn}~\cite{mad-gan}. For instance, in smart power grids, malicious activities can disrupt electricity distribution, leading to widespread blackouts and significant economic losses. Similarly, in water treatment and distribution networks, unauthorized access can manipulate data to indicate false contamination events or mask actual contamination, jeopardizing public health and safety. Therefore, an efficient and accurate time series anomaly detection (TSAD) system is essential for the continuous monitoring of critical infrastructure, providing timely notifications of any probable anomalous occurrences. This proactive monitoring helps in preventing failures, ensuring system reliability, and safeguarding sensitive data. Despite the importance of TSAD, its efficacy is often constrained by the rarity of anomalies and the resource-intensive nature of obtaining accurate labels. These issues limit the practicality of supervised methods and drive the need for unsupervised TSAD approaches. Deep learning models excel in this regard, as they can learn complex feature representations without reliance on manual labeling.


Deep learning-based unsupervised anomaly detection primarily focus on identifying patterns of normality within unlabeled data, with the expectation that anomalies will manifest as deviations from these identified patterns. Current TSAD methods primarily include forecasting-based and reconstruction-based approaches. The former assume normal instances are predictable, but their performances can falter when temporal patterns are unpredictable or rapidly changing~\cite{lstmed}. The latter, despite not depending on sample extrapolation, can run into overfitting issues due to an undue emphasis on pixel-wise reconstructions. In recent years, contrastive learning has emerged as a significant area of interest in various domains~\cite{he2020momentum}~\cite{chen2020simple}~\cite{saeed2021contrastive}~\cite{shi2019deepchannel}, lauded for its capability to distill valuable feature representations from data. Unlike traditional approaches, contrastive learning operates on the latent feature space, advocating for the alignment of similar instances and the segregation of dissimilar ones. Given its powerful representation learning ability, some researches have applied it to solve the anomaly detection problem and have shown promising results, particularly in Computer Vision (CV) domain~\cite{geoTransformation}~\cite{robustAndUncertainty}~\cite{inlier}. 


% Among unsupervised deep-learning methods, contrastive learning has captured significant interest across various fields such as Computer Vision (CV), audio processing, and Natural Language Processing (NLP), thanks to its ability to distill robust feature representations by contrasting similar and dissimilar instances~\cite{chen2020simple,saeed2021contrastive,shi2019deepchannel}. Particularly in CV, it has been leveraged to address anomaly detection challenges with promising outcomes~\cite{geoTransformation,robustAndUncertainty,inlier}. 

Yet applying contrastive learning to TSAD presents unique challenges. First, anomalies in time series data are context-dependent, necessitating an analysis that understands each instance in relation to its contextual backdrop. Secondly, standard contrastive learning requires the selection of negative samples in order to avoid a representation collapse - a scenario where a model converges to trivial solutions that map different inputs to indistinguishable representations. However, deriving negative samples from a pool of predominantly normal instances is ill-suited for anomaly detection. Additionally, the generation of ``similar'' positive samples through data augmentation, such as geometric transformations for images (e.g., cropping and rotating)~\cite{geoTransformation}, is not directly applicable to time series data due to their intricate temporal dependencies.


In this work, we propose a new TSAD method, CNT, to address the aforementioned challenges. Motivated by Contrastive Predictive Coding (CPC)~\cite{cpc}, we implement a relatively simple but effective temporal-wise contrasting where each instance is defined by a prediction time window and is pulled closer to a corresponding context window through a contextual contrastive loss. This strategy naturally discerns anomalies by highlighting significant divergences from historical patterns. However, this alignment alone can result in the representation collapse issue: the feature encoders of both windows produce constant representations irrespective of their input. In traditional contrastive learning, this issue is often circumvented by using negative samples, ensuring diversity in the learned representations. To avoid wrongly selecting negative samples within the same normal class,  we directly augment the temporal-wise contrasting with a discriminative contrastive loss proposed in NeuTralAD~\cite{neuralAD}. Specifically, a set of learnable augmentations is applied to the latent space of the prediction window, resulting in a range of transformations that are diverse yet semantically consistent with the original inputs. Subsequently, temporal-wise contrasting is executed between these transformed future windows and their past observations, with anomalies anticipated to disrupt this contextual consistency more than normal instances. Lastly, our theoretical analysis indicates that this duel-loss circumvents the issue of representation collapse without the need for negative samples. 

To summarize, our key contribution includes:
\begin{enumerate}
\item We propose a simple and computationally efficient TSAD framework, CNT, which harnesses the idea of temporal-wise contrastive learning with neural transformation learning. 
The approach is specifically tailored for the detection of temporal anomalies through a combination of contextual contrastive loss and discriminative contrastive loss.
\item We provide theoretical analysis demonstrating that a combination of the aforementioned two losses effectively mitigates the representation collapse problem of contrastive learning without introducing negative samples.
\item Extensive experiments are conducted on five real-world industrial datasets to demonstrate the superior performance of our proposed approach over existing baseline methods and a variety of model variants.
\end{enumerate}

% Unlike NeuTralAD which focuses on learning augmentations from raw time series at the instance level, CNT applies the transformation at the latent space, and contrastive learning occurs between each instance and its temporal context. 

% Empirical results confirm CNT's superior performance, yielding higher F1 scores and better computational efficiency compared to NeuTralAD, as well as enhanced detection capabilities over other benchmarks across various real-world industrial datasets.


==> subtexes/literature_review.tex <==
\section{Related Works}
This section primarily focuses on reviewing deep learning-related methods in anomaly detection due to the rapid advances in deep learning approaches.

The two mainstream deep time series anomaly detection approaches are forecasting-based and reconstruction-based methods. Forecasting-based methods predict future values and identify anomalies as data points deviating from predictions. Reconstruction-based methods reconstruct input data and identify anomalies as data points that cannot be accurately reconstructed. Recent works~\cite{lstm-ndt}~\cite{deng2021graph}~\cite{zhao2020multivariate}~\cite{han2022learning} for forecasting-based methods leverage various neural network architectures like LSTMs, GRUs, TCNs, GNNs, and hybrid combinations. Reconstruction-based methods include deep autoencoders (AEs)~\cite{su2019robust}~\cite{malhotra2016lstm}~\cite{park2018multimodal}~\cite{zhanggrelen} and Generative Adversarial Networks (GANs)~\cite{audibert2020usad}~\cite{li2019mad} with varying underlying sequence encoder architectures. 
% These methods may have limitations in certain scenarios. For example, forecasting-based methods may struggle when the underlying temporal patterns are unpredictable or rapidly changing~\cite{lstmed}, while reconstruction-based methods may suffer from the identity mapping problem. Researchers have proposed various techniques, such as regularization and additional constraints, to address these limitations~\cite{gong2019memorizing}.

% In time series anomaly detection, two primary methods are commonly utilized: forecasting-based and reconstruction-based. Forecasting-based methods aim to predict future values of the time series and identify anomalies as data points that significantly deviate from the predicted values. Reconstruction-based methods, on the other hand, utilize a trained model to reconstruct the input time series data and identify anomalies as data points that cannot be accurately reconstructed. The rationale behind those methods is that anomalies exhibit patterns that are challenging to predict or reconstruct. Some recent works for forecasting-based methods are~\cite{lstm-ndt}~\cite{deng2021graph}~\cite{zhao2020multivariate}~\cite{han2022learning}, where the differences lie in their underlying neural network architecture to encode temporal sequences, including Long Short Term Memory (LSTMs)~\cite{lstm}, Gated Recurrent Units (GRUs)~\cite{gru}, Temporal Convolutional Networks (TCNs)~\cite{tcn}, Graph Neural Networks (GNNs)~\cite{kipf2016semi}, and hybrid combinations thereof. For reconstruction-based methods, representative works include deep autoencoders (AEs)~\cite{su2019robust}~\cite{malhotra2016lstm}~\cite{park2018multimodal}~\cite{zhanggrelen} and Generative Adversarial Networks (GANs)~\cite{audibert2020usad}~\cite{li2019mad}. These methods can also vary in terms of their underlying sequence encoder architectures. While these methods have demonstrated effectiveness, they may be limited in certain scenarios. For example, forecasting-based methods may struggle when the underlying temporal patterns are unpredictable or rapidly changing~\cite{lstmed}, while reconstruction-based methods may suffer from the identity mapping problem. Researchers have proposed various techniques, such as regularization and additional constraints, to address these limitations~\cite{gong2019memorizing}.

% Other promising branches of methods are the aforementioned one-class classification methods, and self-supervised learning approaches. Self-supervised learning methods have recently been explored for use in anomaly detection. The techniques that fall in this line can be generally categorized into two main branches: contrastive learning-based approaches and augmentation prediction approaches. The idea of contrastive learning is to pull the representations of each data instance and its augmented version together while pushing away from a set of negative samples~\cite{cpc}. When adapting to anomaly detection, the underlying assumption is that normal samples are close to its augmented version which is not true for anomaly samples. Some recent works~\cite{coca}~\cite{tsCPCAD} adapt this idea to time series anomaly detection by leveraging a feature encoder that is tailored to temporal sequences. The process of augmentation prediction involves generating a set of samples by applying various data augmentation operations to each data instance, followed by training a model to classify the specific augmentation that a given augmented sample corresponds to\cite{geoTransformation},\cite{robustAndUncertainty}, and~\cite{inlier}. The underlying assumption when adapting to anomaly detection is that it is easier to classify the augmentation of normal instances compared to anomaly samples. \cite{neuralAD} relieves the difficulties of selecting the right augmentations by learning the transformation by itself through a discriminative contrastive loss. 

% In addition to forecasting-based and reconstruction-based methods, other promising approaches for time series anomaly detection include the aforementioned one-class classification methods and self-supervised learning methods. Self-supervised learning has recently gained attention for anomaly detection, with techniques falling into two categories: contrastive learning-based and augmentation prediction-based approaches (See details in Section~\ref{sec: neutral AD}). Contrastive learning aims to bring together the representations of each data instance and its augmented version while pushing away from negative samples~\cite{cpc}. Recent works have adapted this approach to time series anomaly detection using a feature encoder tailored to temporal sequences~\cite{coca}~\cite{tsCPCAD}. 
% Augmentation prediction involves generating a set of samples by applying various data augmentation operations to each data instance and training a model to classify the specific augmentation that a given augmented sample corresponds to~\cite{geoTransformation}~\cite{robustAndUncertainty}~\cite{inlier}. As selecting the appropriate augmentation for a particular data type can be a challenging task,~\cite{neuralAD} have tackled this issue by training the model to learn the transformation itself using a discriminative contrastive loss.

Other promising approaches for time series anomaly detection include the aforementioned one-class classification methods and self-supervised learning methods. Self-supervised learning techniques can be divided into two categories: augmentation prediction-based (See details in Section~\ref{sec: neutral AD}) and contrastive learning-based approaches. Contrastive learning brings together representations of data instances and their augmented versions while pushing away negative samples~\cite{cpc}. Recent works have adapted this approach to time series anomaly detection using a feature encoder tailored to temporal sequences~\cite{coca}~\cite{tsCPCAD}.


Two similar approaches to our proposed method are LNT~\cite{lnt} and NCAD~\cite{ncad}. LNT uses NeuTral AD and CPC loss to bring together latent representations of $k$-step ahead time series values and their context windows, while maintaining distinguishable representations via neural transformation learning. In contrast, our approach performs computationally efficient sequence-level contrasting and contrasts transformations of input sequences against both their context window and itself to prevent representation collapse.
On the other hand, NCAD trains a semi-supervised binary classifier with negative samples generated from synthetic anomalies using a similar window-based approach. However, tuning the ratio of different types of anomalies can be challenging, as different applications may have different types of anomalies. Our approach circumvents this challenge by using the discriminative contrastive loss from Neutral AD to learn salient features from temporal sequences and prevent representation collapse. We also enforce the same sequence encoder for an input instance and its context window, ensuring that the feature representations are in the same space.

==> subtexes/methodology.tex <==
\subsection{Problem Formulation}
\label{sec: problem formulation}
% Following commonly used notations, the $i^{th}$ row and $j^{th}$ column of an arbitrary 2D matrix $A$ are denoted by $A_{i\cdot}$ and $A_{\cdot j}$ respectively. The $(i,j)^{th}$ entry of A is denoted by $A_{ij}$. The $l_2$-norm of a vector is represented by ${\| \cdot \|}_2$, while the Frobenius norm for a matrix is referred as $\|\cdot\|_F$.
We use common notations such as $A_{i,\cdot}$ and $A_{\cdot, j}$ to denote the $i^{th}$ row and $j^{th}$ column of an arbitrary 2D matrix $A$, and $A_{i,j}$ to denote the $(i,j)^{th}$ entry of $A$. The $l_2$-norm of a vector is represented by ${\| \cdot \|}_2$, while the Frobenius norm for a matrix is referred as $\|\cdot\|_F$. We use $\oslash$ to denote the element-wise division, $\odot$ for element-wise multiplication, and $\mathbin\Vert$ for vector concatenation.

In this study, we are given a multivariate time series $X \in \R^{N\times T}$, collected over $T$ time ticks with $N$ features, as a training set. The goal is to detect anomalies in a test set, which is a time series with $N$ features collected over a different span of time ticks from the training set. The training sample set $\D$ contains sub-sequences extracted from $X$, i.e., $X$ is split into a series of sub-sequences with stride 1. Here, a sample $X^t$ represents a collection of time ticks within a sliding context window of length $w$: $X^t=\{X_{\cdot i}\}_{i=t-w+1}^t$, where $X_{\cdot t} \in \R^{N}$ is the multivariate time series value at timestamp $t$. We aim at assigning an anomaly score to each time tick in the test set given a test sample, which is later threshold-ed to a binary label with $0$ being normal and $1$ being abnormal. 
% We consider a semi-supervised setting, where the training set consists of only normal data and the test set contains a mixture of normal and anomalous data. 

Furthermore, in our framework, each sample $X^t$ is segmented into two sub-sequences of length $c$, which we referred to as a context sequence $C^t$ and suspect sequence $S^t$. $S^t$ is shifted forward from $C^t$ by a time window of length $p$, i.e., $C^t=\{X_{\cdot,i}\}_{i=t-w+1}^{t-p}$ and $S^t = \{X_{\cdot,i}\}_{i=t-c}^{t}$. The time window from $t-p+1$ to $t$ is referred to as the suspect window, and the one from $t-w+1$ to $t-p$ is denoted as the context window. $c$ and $p$ are two hyper-parameters tuned for each dataset. A visualization of notations is shown in Figure~\ref{fig: framework}.

% Furthermore, in our framework, each sample $X^t$ is segmented into two sub-sequences of length $c$, with one shifted from the other of a time window of length $p$, where $c=w-p$, i.e., $C^t=\{X^t_{\cdot,i}\}_{i=t-w+1}^{t-p}$ and $S^t = \{X^t_{\cdot,i}\}_{i=t-c}^{t}$. We denote $C^t$ and $S^t$ as the context and suspect sequence, respectively. The time window from $t-p+1$ to $t$ is referred to as the suspect window, and the one from $t-w+1$ to $t-p$ is denoted as the context window. c and p are two hyper-parameters tuned for each dataset. A visualization of notations is shown in Figure~\ref{fig: framework}.

% Each training sample $X^t$ is segmented into two sub-sequences of length $c$, which are referred to as context sequence and suspect sequence, with one overlapping the other of a time window of length $p$, where $c=w-p$. The context sequence $C^t$ consists of the time ticks in the context window, while the suspect sequence $S^t$ consists of the time ticks in the suspect window.




% For time series anomaly detection, we have a multivariate time series $X \in R^{N \times T_{\text{train}}}$ with N features collected over $T_{\text{train}}$ time ticks as the training set and another multivariate time series with the same number of features spanning $T_{\text{test}}$ time steps as the test set. Following the semi-supervised setting, the training set only contains normal samples, and the test set consists of both normal and anomalous samples.

% The input to our model, $X^t=\{X_{\cdot t-w+1}, ..., X_{\cdot i},...,X^t_{t}\}$, is a multivariate sequence with a window size of $w$, where $X_{\cdot i}\in R^{N}$ denotes the multivariate time series value at time step $i$. 
% The goal is to detect anomalies in the test set by assigning a score $y^t$ on each time step t over $T_{\text{test}}$, which is later thresholded into a binary label with 0 as normal and 1 as anomalous. 




\subsection{Overview}
% \begin{figure*}[t!]
    
%     \centering
%    % \includesvg[width=1\linewidth]{figures/Framework.svg}
%         \includesvg[width=1\linewidth]{figures/neural_contrast/Framework_contrast.svg}  
%     \caption{To be continued}
%     \label{fig:framework}
% \end{figure*}


This section presents an overview of the proposed framework (See Figure~\ref{fig: framework}), which includes a feature encoder module and a neural transformation module, jointly optimized using two contrastive losses. Specifically, the framework transforms the suspect sequence into multiple latent representations and utilizes two loss functions: a contextual neural contrastive loss and a discriminative contrastive loss. The former aims to minimize distance between the transformed suspect and context sequences, while the latter ensures diversity of transformed sequences while preserving original semantics to avoid representation collapse.

% This section presents an overview of the proposed framework. Figure~\ref{fig: framework} illustrates the overall architecture, which comprises a feature encoder module and a neural transformation module, jointly optimized using contextual contrastive loss and discriminative contrastive loss. 
% The pipeline of the framework begins with the feature encoder, which converts suspect and context sequences of a given sample into hidden representations. Next, the neural transformation network transforms the hidden representation of the suspect sequence into multiple different latent representations. Finally, the model leverages two loss functions to optimize the framework: a contextual contrastive loss and a discriminative contrastive loss. 
% The contextual contrastive loss aims to minimize the distance between the transformed suspect sequences and the context sequence. On the other hand, the discriminative contrastive loss ensures that the transformed sequences remain diverse while maintaining the original semantics of the suspect sequence, in order to prevent the representation collapse problem arising from optimizing the contextual contrastive loss alone.




% \begin{figure}[t]
% \centering
% \begin{subfigure}[t]{0.7\linewidth}
%     \centering
%     % \includesvg[height=2.9cm]{figures/swat_graph_deviation.svg}
%     %\includesvg[height=5cm]{figures/neural_contrast/Framework_contrast.svg} 
%         \includegraphics[height=5cm]{figures/neural_contrast/Framework_contrast.eps}  

%     %\vspace{-0.55cm}
%     \caption{}
%     \label{fig: framework}
% \end{subfigure}
% %\hspace{\fill} % maximize horizontal separation
% %\newline
% %\vspace{-0.1cm}
% \centering
% \begin{subfigure}[t]{0.28\linewidth}
%     \centering
%     % \includesvg[height=2.9cm]{figures/wadi_graph_deviation.svg}
% %\includesvg[height=4.5cm]{figures/neural_contrast/tcn_feature_encoder.svg}  
%  \includegraphics[height=4.5cm]{figures/neural_contrast/tcn_feature_encoder.eps}  

%        % \vspace{-0.55cm}
%     \caption{}
%     \label{fig: tcn feature encoder}
% \end{subfigure}
% \caption{(a) The overall architecture of our proposed framework. (b) The inner structure of feature encoder.}
% \end{figure}


% The former aims to pull the hidden representation of the suspect sequence close to the context sequence. The latter prevents the hyper-sphere collapse problem of the former, by transforming the suspect feature representation into different views which are diverse among themselves as well as preserving the semantics of the suspect sequence.
% \begin{itemize}
%     \item Feature encoder: Given an input sample, The suspect sequence and the context sequence are converted into hidden representations by the feature encoder, which aims to capture both the temporal pattern as well as the inter-series relationship of the sequences. 
%     \item The optimization module takes the encoded feature representation of the two sequences as the input and calculates two losses: a contextual one-class loss and a neural transformation loss. The former aims to pull the hidden representation of the suspect sequence close to the context sequence. The latter prevents the hyper-sphere collapse problem of the former, by transforming the suspect feature representation into different views which are diverse among themselves as well as preserving the semantics of the suspect sequence.
%     \item Scoring module: After the training is done, the module is used to compute an anomalous sore for each test sample based on the aforementioned losses. 
% \end{itemize}
% The overall architecture of XXX is shown in Figure. The framework is composed of three modules:
% \begin{itemize}
%     \item Feature encoder: Given an input sequence, the feature encoder converts it into two sequence 
%     The encoder converts a given input sequence into a list of inter-series graphs that aim to capture the time-varying relationship among timeseries. 
%     \item Neural transformation: The encoded feature representation of the graphs from the feature encoder is segmented into a suspect window and a context window. The suspect window is transformed into different latent views through distinct neural networks.
%     \item Optimization: the framework is optimized under a contextual one-class loss and a neural transformation loss. The former aims to pull the views of the suspect window close to the context window. The latter prevents the hyper-sphere collapse problem of the former by making the views diverse while still preserving the semantics of the suspect vector.
%     % The former is the feature representation of the graph learned based on the sequence within the suspect window, while the latter contains the features of the historical graphs within the context window.
% \end{itemize}



\subsection{Feature Encoder}
\label{sec: feature encoder}
% The feature encoder aims to capture temporal dependencies within a suspect or context sequence, enabling our framework to detect anomalies in the suspect window by identifying abnormal temporal patterns with respect to the context window. To apply the same feature encoder to both sequences, we define two overlapping sequences, denoted by $C^t$ and $S^t$, with equal lengths, as discussed in Section~\ref{sec: problem formulation}. Following the work of~\cite{tcn, wu2020connecting}, we adopt a temporal convolution network as the base feature encoder, with the temporal convolution layer replaced by a dilated inception layer to allow for different kernel sizes. The general pipeline is shown in Figure~\ref{fig: tcn feature encoder}. Here, we illustrate the pipeline using $S^t$ as input, but the same process is applied to $C^t$.

% Specifically, we pass $S^t$ through a $\text{1D}$ convolution with a kernel size of $1$ and a channel size of $d$ to obtain its initial representation $Z^t \in \R^{d \times c}$. Next, we pass it through a series of $L$ blocks, each defined as:
% \begin{align}
% Z^{t,l} = \text{BN}(\sigma(f_{\text{DIL}}(Z^{t, l-1}))) + Z^{t, l-1},
% \end{align}
% where $\text{BN}$ denotes a batch normalization layer~\cite{ioffe2015batch}, $\sigma$ is a ReLU function, and $Z^{t, l}$ is the output from the $l^{th}$ block. $\text{DIL}$ represents the dilated inception layer, which is defined as:
% \begin{align}
% & f_{\text{DIL}}(X) = X \star f_{2} \mathbin\Vert X \star f_{3} \mathbin\Vert X \star f_{5} \mathbin\Vert X \star f_{7},
% \end{align}
% where $X \star f_k$ is a $\text{1D}$ convolution layer applied on $X$ with a kernel size $k$ and an output channel size of $\frac{d}{4}$, and the concatenation operation $\mathbin\Vert$ is performed on the channel-wise dimension. We don't pad the sequences so that each concatenation is performed on the truncated outputs from the four different convolutions, with the truncated size matching the length of the shortest output.


The feature encoder serves the purpose of capturing temporal dependencies within a suspect or context sequence, thereby facilitating the detection of anomalies in the suspect window by identifying anomalous temporal patterns with respect to the context window. 
we have defined two overlapping sequences - $C^t$ and $S^t$, with equal lengths, as discussed in Section~\ref{sec: problem formulation}. 
The reason for making these sequences overlap is to ensure that their latent representations remain close to each other thus not violating our assumptions. 
% To ensure the use of the same feature encoder for both sequences, we have defined two overlapping sequences - $C^t$ and $S^t$, with equal lengths, as discussed in Section~\ref{sec: problem formulation}. 
Following the methodology employed by~\cite{tcn}~\cite{wu2020connecting}, we have utilized a temporal convolution network as the base feature encoder, wherein the temporal convolution layer has been replaced by a dilated inception layer (DIL)~\cite{wu2020connecting} that enables the use of different kernel sizes. The general pipeline of the encoder is depicted in Figure~\ref{fig: tcn feature encoder}. Note that we have demonstrated the pipeline using $S^t$ as input; however, the same procedure is implemented for $C^t$.

More specifically, we start by passing $S^t$ through a $\text{1D}$ convolution with a channel size of $d$ and a kernel size of $1$ to obtain its initial representation, $Z^t \in \R^{d \times c}$. Subsequently, we pass it through $L$ TCN blocks, with each containing a DIL layer followed by a batch normalization layer~\cite{ioffe2015batch}. The residual connection is added in between each TCN blocks. After applying a sequence of TCN blocks, we obtain a final output with a dimension of $(d, 1)$, which is subsequently fed through another $\text{1D}$ convolution layer with a kernel size of $(1, 1)$ to derive the ultimate latent representation of $S^t$. We denote the latent representations of $S^t$ and $C^t$ as $O^t$ and $G^t$, respectively.

% More specifically, we start by passing $S^t$ through a $\text{1D}$ convolution with a channel size of $d$ and a kernel size of $1$ to obtain its initial representation, $Z^t \in \R^{d \times c}$. Subsequently, we pass it through $L$ TCN blocks, each of which is defined as:
% \begin{align}
% Z^{t,l} = \text{BN}(\sigma(f_{\text{DIL}}(Z^{t, l-1}))) + Z^{t, l-1},
% \end{align}
% where $\text{BN}$ refers to a batch normalization layer~\cite{ioffe2015batch}, $\sigma$ represents a ReLU function, and $Z^{t, l}$ is the output from the $l^{th}$ block. The dilated inception layer is represented by $\text{DIL}$, which is defined as:
% \begin{align}
% & f_{\text{DIL}}(X) = X \star f_{2} \mathbin\Vert X \star f_{3} \mathbin\Vert X \star f_{5} \mathbin\Vert X \star f_{7},
% \end{align}
% where $X \star f_k$ denotes a $\text{1D}$ temporal convolution layer applied to $X$ with a kernel size of $k$, a dilation factor of $2^{(l-1)}$, and an output channel size of $\frac{d}{4}$, and the concatenation operation $\mathbin\Vert$ is performed on the channel dimension. We do not pad the sequences, and thus, each concatenation is performed on the truncated outputs from the four different convolutions, with the truncated size matching the length of the shortest output. After applying a sequence of TCN blocks, we obtain a final output with a dimension of $(d, 1)$, which is subsequently fed through another $\text{1D}$ convolution layer with a kernel size of $(1, 1)$ to derive the ultimate latent representation of $S^t$. We denote the latent representations of $S^t$ and $C^t$ as $O^t$ and $G^t$, respectively.

% \begin{wrapfigure}{r}{0.3\textwidth}
%   \begin{center}
%     %\includegraphics[width=0.48\textwidth]{birds}
%     \includesvg[height=4cm]{figures/neural_contrast/tcn_feature_encoder.svg} 
%   \end{center}
%   \caption{Birds}
% \end{wrapfigure}


% \begin{wrapfigure}{r}
%     %\centering
%    % \includesvg[width=1\linewidth]{figures/Framework.svg}
%         \includesvg[width=0.5\linewidth]{figures/neural_contrast/tcn_feature_encoder.svg}  
%     \caption{To be continued}
%     \label{fig:tcn feature encoder}
% \end{wrapfigure}





% In a nutshell, 
% the feature encoder first converts the input sequence into an inter-series graph. Next, a graph convolution module is applied on top of the adjacency matrix and the input sequence to obtain the final hidden representations of the graph. The general pipeline is defined as follows
% \begin{align}
%      & A^t = f_{\text{g}}(C^t) \\
%      & H^t = f_{\text{c}}(A^t, C^t) 
% \end{align}
% where $f_{\text{g}}(\cdot): R^{N \times c}\rightarrow R^{d}$ is the graph generator, and $f_{\text{c}}(\cdot): R^{N \times N} \times R^{N \times c} \rightarrow R^{N \times d}$ is the graph convolution module.

% \subsubsection{Graph generator} 
% The graph generator takes the sequence $C^t$ as the input and generates an adjacency matrix $A^t \in R^{N \times N}$. We adopt the simplest setting, where $A^t$ is generated based on the cosine distance between pairwise nodes. Other advanced graph generation approaches can be adapted to this framework as well, such as adding an additional graph sparsification layer as in~\cite{deng2021graph}. The graph generator is defined as
% \begin{align}
%     & A^t = D^{-1/2} \textnormal{ReLU}(S^t) D^{-1/2} \\
%     & S^t_{ij} = \frac{Z'_i^t Z'_j^t}{|Z'_i^t| |Z'_j^t|} \\
% % \end{align}
% % \begin{align}
%     & Z'^t = \text{ReLU}(f_{p2}(Z^t)W_1+b_1)W_2+b_2 \\
%     & Z^t = f_{p1}(C^t)
% \end{align}
% where $D$ is the degree matrix of the un-normalized adjacency matrix $S^t$, $f_{p1}(\cdot)$ is an 1D convolution layer with a channel size of $d$ and kernel size of $(1, 1)$, $f_{p2}(\cdot)$ is an 1D convolution layer with a channel size of $d$ and kernel size of $(1, c)$ followed by a transpose operation on time-axis and feature-axis, ($W_1\in R^{c \times d}$, $b_1 \in R^{d}$) and ($W_2 \in R^{d}$, $b_2 \in R$) are learnable weights and biases. 

% \subsubsection{Graph convolution}
% Given $Z^t$ and $A^t$ from the graph generator, we perform the following two operations iteratively for L times to obtain the node feature representations
% \begin{align}
%     & H^{t, l+1} = f_{tconv}(Z^{t, l}) \\
%     & Z^{t, l+1} = f_{gconv}(H^{t, l+1}, A^t)+H^{t,l+1}  
% \end{align}
% where $f_{\text{tconv}}$ is the dilated inception layer~\cite{wu2020connecting} and $f_{\text{gconv}}$ is a graph convolution layer~\cite{kipf2016semi}. dilated inception layer applies multiple 1D convolutions with different kernel sizes separately on top of the input sequence, and the obtained representation is a concatenation of the outputs from those convolutions. This step can be treated as local feature engineering, incorporating information from different granularity into each time tick. In addition, the receptive field of the dilation layer grows exponentially at a rate of 2, which is capable of capturing the long-term temporal dynamics of a time series and is computationally efficient compared to recurrent neural networks. 

% Finally, the output from the feature encoder $O^t \in R^{d}$ is obtained as
% \begin{align}
%     O^t = \text{Pooling}(\text{Concat}(H^{t, L}, Z^{t,L}, ..., H^{t,1}, Z^{t, 1}))
% \end{align}
% where the concatenation is performed on the time axis, and the mean pooling operation is taken on both the time dimension and the feature dimension. In particular, the output $O^t \in R^{d}$ can be treated as the representation of the generated graph, where the node features are temporal sequences encoded through a series of temporal convolution layers.

\begin{figure}[t!]
\centering
\includesvg[height=3.5cm]{figures/neural_contrast/notation_graph.svg}  

\caption{(a) The overall architecture of our proposed framework. (b) The inner structure of feature encoder.}
\label{fig: framework}

\end{figure}
\subsection{Optimization Framework}
\label{sec: optimizatino}
% Given the encoded feature representation $O^t$ for the suspect sequence and $G^t$ for the context sequence, the optimization module aims to minimize two losses: a contextual contrastive loss and a discriminative contrastive loss.

\subsubsection{Contextual Contrastive Loss Without Regularization}
% Our proposed framework is based on the assumption that normal sequences within the prediction window change mildly in comparison to abnormal sequences from recent history. To implement this idea, we contrast the prediction window with the context window by minimizing the distance between the hidden representations of the two windows for normal samples. This idea is inspired by DeepSVDD, which trains neural networks by minimizing the volume of a hypersphere that encloses normal data. However, instead of adopting a fixed hypersphere center, we allow the center to vary based on the context. By incorporating more information about the surrounding context, anomalies can be identified based on their abnormal pattern with respect to the past. This approach is better adapted to time series anomaly detection, where the majority of anomalies are contextually irregular.

Our framework assumes that normal sequences change mildly compared to abnormal sequences from recent history. To implement this, we contrast the prediction window with the context window by minimizing the distance between their hidden representations for normal samples. This approach is inspired by DeepSVDD, but allows the center of the hypersphere to vary based on the context, better adapting it to time series anomaly detection where most anomalies are contextually irregular.

% Let $O^t$ and $Q^t$ be the encoded representation of the suspect sequence $P^t$ and context sequence $C^t$ from the feature encoder respectively. 
Formally, let $g(\cdot, W): \R^{N \times c} \rightarrow \R^d$ be the feature encoder in section~\ref{sec: feature encoder} with learnable weights $W$. We define a contextual contrastive loss as
\begin{align}
   %&  \min_W L_{\text{ccl}} \\
   & \LL_{\text{ccl}}:= \EX_{X^t \sim \D}{ \|g(S^t;W) - g(C^t;W)\|}^2_2
    \label{eq. raw contextual one-class objective}
\end{align}
which is the mean euclidean distance between the hidden representations of the suspect sequence and context sequence. However, minimizing Eq.~\eqref{eq. raw contextual one-class objective} can lead to constant encoder solutions, which we refer to as the representation collapse issue. Specifically, the optimal solution of the objective can be trivially achieved when the output of the encoder is a constant for arbitrary input values (More details in section~\ref{sec:theoretical analysis}).

One way to avoid the constant encoder solution is to add an objective that enforces the encoder to produce different outputs under different contexts. In this work, we explore the combination of this contextual contrastive objective with neural transformation learning~\cite{qiu2021neural} for time series anomaly detection. 
% For example, we could let the encoder be optimized under the regression task or reconstruction task settings. 

\subsubsection{Equipping With Neural Transformations}
Neural transformation learning learns diverse transformations that maintain the original sample's semantic information. We could leverage this approach to prevent the representation collapse, by contrasting the diverse but semantic-related hidden representations of the suspect feature representation $O^t$ against the context feature representation $G^t$.

% In this case, the feature representation of the predict sequence are guaranteed to be contextually dependent on the given input, which avoids the constant encoder solution.
Formally, given the suspect feature representation $O^t$, we project it into K latent representations $\{O^{t,i}\}_{i=1}^K$ using distinct transformation networks $T=\{T_1, ..., T_K|T_k:\R^d \rightarrow \R^d\}$. In our implementation, we choose three-layer MLPs with hidden dimension $d$ for $T_k$. In contrast to the original neural transformation learning, where transformations are applied to the raw inputs and fed through the feature encoder multiple times, we apply transformations directly to the hidden space to avoid computational burden. This allows us to apply the feature encoder only once, followed by K lightweight transformation encoders, reducing the overall computation required.


% Formally, given the suspect feature representation $O^t$ from the feature encoder, we project it into K latent representations $\{O^{t,i}\}_{i=1}^K$ through distinct transformation networks $T=\{T_1, ..., T_K|T_k:\R^d \rightarrow \R^d\}$. In our implementation, we choose $T_k$ as a three-layer MLP with the same hidden dimension $d$ in each layer. Note that in the original neural transformation learning, transformations are applied to the raw inputs directly and each transformation has to be fed through the feature encoder once, which can be computationally expensive when the encoder has complex neural network architectures. In this work, we circumvent the computation burden by applying the transformation directly on the hidden space so that the feature encoder is applied only once followed by K lightweight transformation encoders.

Concretely, to ensure the K transformations are diverse and semantically similar to the original input, ~\cite{qiu2021neural} proposes a discriminative contrastive loss as stated in~\ref{sec: neutral AD}. We rephrase it with the notation in our section 
% which is defined as
\begin{align}
    \LL_{\text{dcl}}:= -\EX_{X^t \sim \D} \sum_{k=1}^K \log{\frac{h(O^t,O^{t, k})}{h(O^t,O^{t, k})+\sum_{l \neq k} h(O^{t, k}, O^{t, l})}} 
\end{align}
% where the scoring function $h(x_i, x_j)$ is denoted as
% \begin{align}
%     & h(x_i, x_j) = \exp(\text{sim}(x_i, x_j)) \\
%     & \text{sim}(x_i, x_j) = \frac{x_i^Tx_j}{\|x_i\|\|x_j\|}
% \end{align}

To adapt the neural transformation loss to our framework, we re-define a contextual neural contrastive loss $L_{\text{cncl}}$ as
\begin{align}
        & \LL_{\text{cncl}} := \EX_{X^t \sim \D} \sum_{k=1}^K { \|O^{t, k} - G^t\|}^2_2 
        \label{eq. contextual neural contrastive loss}
\end{align}
where the contrastion is performed between the transformations of suspect feature representation against the context feature representation. During the training, the model architecture, including the feature encoder and the neural transformations, is optimized under a contextual discriminative contrastive loss $\LL_\text{cdcl}$ during the training, which is defined as
% $L_{\text{lnctl}}$ as
\begin{align}
    & \LL_{\text{cdcl}} := \LL_{\text{cncl}} + \LL_{\text{dcl}} 
    \label{eq. contextual discriminative contrastive loss}
\end{align}
We prove in section~\ref{sec:theoretical analysis} that the edge case, where both the outputs of the transformations and the feature encoder generates the same constant, does not minimize the joint loss in Eq.~\eqref{eq. contextual discriminative contrastive loss}. Additionally, during inference, Eq.~\eqref{eq. contextual discriminative contrastive loss} can be directly utlized as an anomaly score of an input sample.
% where
% \begin{align}
%         & L_{\text{lcl}} := \sum_{t=1}^{T_{\text{train}}} \sum_{k=1}^K { \|O^{t, k} - G^t\|}^2 
% \end{align}
% our proposed model architecture, including the feature encoder and the neural transformations, is optimized under $L_\text{lcntl}$ during the training.









% Let $O^t$ and $Q^t$ be the encoded representation of the suspect sequence $P^t$ and context sequence $C^t$ from the feature encoder respectively. The local contrasting loss can be defined as
% \begin{align}
%     L_{\text{cocc}} ={ \|O^t - Q^t\|}^2 
%     \label{eq. contextual one-class loss}
% \end{align}
% which is the euclidean distance between the hidden representations of the suspect sequence and context sequence.

% Similar to the one-class classification loss, minimizing Eq.~\eqref{eq. contextual one-class loss} can lead to trivial solutions which is proved in the following proposition.

% \begin{proposition} \label{prop.constant_weights}
% have bias, leads to the constant solution.
% \end{proposition}

% first fed into a dilated inception layer (i.e., with kernel sets of $(2, 3, 5, 7)$ and channel size of $d$) to obtain a dense hidden representation $C^t \in R^{d \times N \times c}$. The dilated inception layer, proposed in~\cite{wu2020connecting}, applies multiple 1D convolutions with different kernel sizes separately on top of the input sequence, and the obtained representation is a concatenation of the outputs from those convolutions. This step can be treated as local feature engineering, which encapsulates information from different granularity to the hidden representation at a different time step.
% \begin{align}
%     & C^t = f_{\text{p}}(C^t) \\
%     & A'_{ij} = \frac{C'_i C'_j}{|C'_i| |C'_j|}\\
%     & A = D^{-1/2} \textnormal{ReLU}(A') D^{-1/2}
% \end{align}
% where $f_p$



% Given an input sequence $X_t \in R^{N \times c}$, the encoder breaks it into $m$ patches $\{S_{i,t}\}_{i=1}^m$ with $S_{i,t} \in R^{N \times w}$. Specifically, the operation is performed in parallel through a 2D convolution layer with a kernel size of $(1, w)$ and stride size of $w$, which guarantees that the patches are disjoint from each other. Additionally, a dilated inception layer with a kernel set of $(2, 3, 5, 7)$ is applied before the segmentation to preserve the local similarity within the sequence. 

% Next, the patches are converted into a series of graphs through graph structure learning. The operation for generating the graph for a given patch S is defined as
% \begin{align}
%     & S' = \textnormal{MLP}(S) \\
%     & A'_{ij} = \frac{S'_i S'_j}{|S'_i| |S'_j|}\\
%     & A = D^{-1/2} \textnormal{ReLU}(A') D^{-1/2} 
% \end{align}
% where MLP is a two-layer neural network, and $D$ is the degree matrix of the unnormalized adjacency matrix $A'$. Our intuition for constructing a series of graphs instead of a static graph is of two-folds. On the one hand, a static graph has limited power to model the timeseries with a time-varying relationship. On the other hand, our framework can identify anomalies based on the abnormal relationship changing from the context window to the suspect window, i.e., an anomaly that happened within the suspect window may have an inter-series relationship that deviates a lot from its historical graphs.

% Upon obtaining the list of graphs, we convert them into dense hidden representations by performing the graph convolution on top of each graph and their corresponding patch. We adopt the MixHop graph convolution, which is commonly used in time series-related tasks. The operation, proposed by~\cite{wu2020connecting}, is defined as 
% \begin{align}
%     & Z_i = \text{concat}(Z_i \star f_{1\times 2}, Z_i \star f_{1 \times 3}, Z_i \star f_{1 \times 5}, Z_i \star f_{1 \times 7}) \label{eq: dilated convolution} \\
%     & z \star f_{1 \times k}(t) = \sum^{k=1}_{s=0} f_{1 \times k}(s)z(t-ns) 
% \end{align}


% The framework XXXX is composed of a feature encoder and an optimization framework. The feature encoder aims to capture the dynamically evolving feature-wise relationship within a given input sequence, while the optimization framework 

% This section gives an overview of the proposed framework, XXXX. First, given an input sequence $X_t$, a feature encoder breaks it into patches and converts them into a series of dynamically evolving graphs. The graph convolution is then applied to each graph and the corresponding segment sequentially to obtain the hidden representation $Z_t$. Next, $Z_t$ is segmented into a context vector $Z_t^c$ and a suspect vector $Z_t^s$, and $Z_t^s$ is transformed through distinct neural networks to obtain $k$ different views $\{Z_{t, i}^s\}_{i=1}^k$. Finally, the framework is optimized under a contextual one-class loss and a neural transformation loss. The former loss aims to pull the transformed views of the suspect vector close to the context vector, while the latter prevents the hyper-sphere collapse problem of the former by making the views diverse while still preserving the semantics of the suspect vector. The intuition of the framework is that the intra-series temporal dynamic and the inter-series relationship within a normal sequence do not vary drastically in a relatively short period, i.e., the sequences within the context window and the suspect window are similar. 

==> subtexes/methodology_v2.tex <==


Let $A$ be an arbitrary 2D matrix, we denote its $i^{th}$ row, its $j^{th}$ column, and its $(i, j)^{th}$ entry by $A_{i\cdot}$, $A_{\cdot j}$ and $A_{ij}$ respectively.
The $l_2$-norm of a vector is represented by ${\| \cdot \|}_2$. In addition, we use $\mathbin\Vert$ to represent the vector concatenation. 
% while the Frobenius norm for a matrix is referred as $\|\cdot\|_F$. We use $\oslash$ to denote the element-wise division, $\odot$ for element-wise multiplication, and $\mathbin\Vert$ for vector concatenation.

In this study, we are given a multivariate time series $X \in \R^{N\times T}$, collected over $T$ time ticks with $N$ features, as a training set. The goal is to detect 
\begin{wrapfigure}{r}{0.5\textwidth}
\vspace{-0.4cm}
    \includesvg[height=3.2cm]{figures/neural_contrast/notation_graph_small.svg}  
    \caption{An illustrative example for the notations based on an input sample $X^t$.}
    \label{fig: notation_example}
\vspace{-0.3cm}
\end{wrapfigure}
anomalies in a test set, which is a time series with $N$ features collected over a different span of time ticks from the training set. The training sample set $\D$ contains sub-sequences extracted from $X$, i.e., $X$ is converted into sliding windows with stride 1. Here, a sample $X^t$ represents a collection of time ticks within a sliding window of length $w$: $X^t=\{X_{\cdot i}\}_{i=t-w+1}^t$, where $X_{\cdot i} \in \R^{N}$ is the multivariate time series value at timestamp $i$. We aim at assigning an anomaly score to each time tick in the test set given a test sample, which is later threshold-ed to a binary label with 0 or 1 for normal or abnormal, respectively.
Furthermore, in our framework, each sample $X^t$ is segmented into two overlapping sub-sequences of length $c$, which we refer to as a context sequence $C^t$ and a predict sequence $S^t$. $S^t$ is shifted forward from $C^t$ by a small time window of length $p=w-c$, i.e., $C^t=\{X_{\cdot i}\}_{i=t-w+1}^{t-p}$ and $S^t = \{X_{\cdot i}\}_{i=t-c}^{t}$. The time window from $t-p+1$ to $t$ is referred to as the predict window, and the one from $t-w+1$ to $t-p$ is denoted as the context window. $c$ and $p$ are two hyper-parameters to be tuned for each dataset. A visualization of notations is shown in 
Figure~\ref{fig: notation_example}.

% Furthermore, in our framework, each sample $X^t$ is segmented into two sub-sequences of length $c$, with one shifted from the other of a time window of length $p$, where $c=w-p$, i.e., $C^t=\{X^t_{\cdot,i}\}_{i=t-w+1}^{t-p}$ and $S^t = \{X^t_{\cdot,i}\}_{i=t-c}^{t}$. We denote $C^t$ and $S^t$ as the context and suspect sequence, respectively. The time window from $t-p+1$ to $t$ is referred to as the suspect window, and the one from $t-w+1$ to $t-p$ is denoted as the context window. c and p are two hyper-parameters tuned for each dataset. A visualization of notations is shown in Figure~\ref{fig: framework}.

% Each training sample $X^t$ is segmented into two sub-sequences of length $c$, which are referred to as context sequence and suspect sequence, with one overlapping the other of a time window of length $p$, where $c=w-p$. The context sequence $C^t$ consists of the time ticks in the context window, while the suspect sequence $S^t$ consists of the time ticks in the suspect window.




% For time series anomaly detection, we have a multivariate time series $X \in R^{N \times T_{\text{train}}}$ with N features collected over $T_{\text{train}}$ time ticks as the training set and another multivariate time series with the same number of features spanning $T_{\text{test}}$ time steps as the test set. Following the semi-supervised setting, the training set only contains normal samples, and the test set consists of both normal and anomalous samples.

% The input to our model, $X^t=\{X_{\cdot t-w+1}, ..., X_{\cdot i},...,X^t_{t}\}$, is a multivariate sequence with a window size of $w$, where $X_{\cdot i}\in R^{N}$ denotes the multivariate time series value at time step $i$. 
% The goal is to detect anomalies in the test set by assigning a score $y^t$ on each time step t over $T_{\text{test}}$, which is later thresholded into a binary label with 0 as normal and 1 as anomalous. 




\subsection{Overview}
% \begin{figure*}[t!]
    
%     \centering
%    % \includesvg[width=1\linewidth]{figures/Framework.svg}
%         \includesvg[width=1\linewidth]{figures/neural_contrast/Framework_contrast.svg}  
%     \caption{To be continued}
%     \label{fig:framework}
% \end{figure*}


This section presents an overview of the proposed framework, CNT (See Figure~\ref{fig: framework}), which includes a feature encoder module and a neural transformation module with both jointly optimized using two contrastive losses. Specifically, the framework begins with the feature encoder, which converts the predict and context sequence of a given sample into hidden representations. Next, the neural transformation network transforms the latent representation of the predict sequence into multiple latent representations. Finally, model parameters are optimized under two loss functions: a contextual neural contrastive loss and a discriminative contrastive loss. 
% The former aims to minimize distance between the transformations of predict sequence and context sequence, while the latter ensures diversity of those transformations while preserving original semantics to avoid representation collapse.
The contextual contrastive loss aims at minimizing the distance between the transformations of predict sequence and context sequence. On the other hand, the discriminative contrastive loss ensures that the transformed sequences remain diverse while maintaining the original semantics of the predict sequence. In addition, it serves the purpose of preventing the representation collapse problem arising from solely optimizing the contextual contrastive loss.


\begin{figure*}[t!]
    \begin{minipage}[b]{1\textwidth}
        \begin{subfigure}[b]{\textwidth}
        \centering
\includesvg[height=5.2cm]{figures/neural_contrast/Framework.svg} 
            \caption{Framework}
           \label{fig: framework}
        \end{subfigure}
    \end{minipage}
        \newline % To push the next figure to the right
        %\vspace{0.3cm}
    \begin{minipage}[b]{1\textwidth}
    \vspace{0.3cm}
%         \begin{subfigure}[b]{\textwidth}
%         \centering
% \includesvg[height=3.2cm]{figures/neural_contrast/notation_graph.svg}  
%             \caption{Notation Example}
%             \label{fig: notation_example}
%         \end{subfigure}
        %\par\bigskip % You can adjust the distance between the two left figures here
        \begin{subfigure}[b]{\textwidth}
        \centering
\includesvg[height=1.7cm]{figures/neural_contrast/feature_encoder.svg}  
            \caption{Feature Encoder}
\label{fig: feature_encoder}
        \end{subfigure}
    \end{minipage}
    \caption{(a) The training pipeline: The blue dashed box indicates that the transformations of the predict sequence are pushing away among themselves while pulling towards the latent feature of the predict sequence. The orange dashed box indicates that the latent representation of the context sequence is pulling closer to the transformations of the predict sequence; (b) The feature encoder architecture;}
    \label{fig:main}
\end{figure*}


\subsection{Feature Encoder}
\label{sec: feature encoder}
% The feature encoder aims to capture temporal dependencies within a suspect or context sequence, enabling our framework to detect anomalies in the suspect window by identifying abnormal temporal patterns with respect to the context window. To apply the same feature encoder to both sequences, we define two overlapping sequences, denoted by $C^t$ and $S^t$, with equal lengths, as discussed in Section~\ref{sec: problem formulation}. Following the work of~\cite{tcn, wu2020connecting}, we adopt a temporal convolution network as the base feature encoder, with the temporal convolution layer replaced by a dilated inception layer to allow for different kernel sizes. The general pipeline is shown in Figure~\ref{fig: tcn feature encoder}. Here, we illustrate the pipeline using $S^t$ as input, but the same process is applied to $C^t$.

% Specifically, we pass $S^t$ through a $\text{1D}$ convolution with a kernel size of $1$ and a channel size of $d$ to obtain its initial representation $Z^t \in \R^{d \times c}$. Next, we pass it through a series of $L$ blocks, each defined as:
% \begin{align}
% Z^{t,l} = \text{BN}(\sigma(f_{\text{DIL}}(Z^{t, l-1}))) + Z^{t, l-1},
% \end{align}
% where $\text{BN}$ denotes a batch normalization layer~\cite{ioffe2015batch}, $\sigma$ is a ReLU function, and $Z^{t, l}$ is the output from the $l^{th}$ block. $\text{DIL}$ represents the dilated inception layer, which is defined as:
% \begin{align}
% & f_{\text{DIL}}(X) = X \star f_{2} \mathbin\Vert X \star f_{3} \mathbin\Vert X \star f_{5} \mathbin\Vert X \star f_{7},
% \end{align}
% where $X \star f_k$ is a $\text{1D}$ convolution layer applied on $X$ with a kernel size $k$ and an output channel size of $\frac{d}{4}$, and the concatenation operation $\mathbin\Vert$ is performed on the channel-wise dimension. We don't pad the sequences so that each concatenation is performed on the truncated outputs from the four different convolutions, with the truncated size matching the length of the shortest output.


The feature encoder aims at capturing temporal dependencies within a predict or context sequence, thereby facilitating the detection of anomalies in the predict window by identifying anomalous temporal patterns with respect to the context window. 
We have defined two overlapping sequences - $C^t$ and $S^t$, with equal lengths, as discussed in Section~\ref{sec: problem formulation} and as shown in Figure~\ref{fig: notation_example}. 
%The reason for making these sequences overlap is to ensure that their latent representations remain close to each other so as not to violate our assumptions. 
% To ensure the use of the same feature encoder for both sequences, we have defined two overlapping sequences - $C^t$ and $S^t$, with equal lengths, as discussed in Section~\ref{sec: problem formulation}. 
Following the methodology employed by~\cite{tcn}~\cite{wu2020connecting}, we have utilized a TCN as the base feature encoder, wherein the temporal convolution layer has been replaced by a dilated inception layer (DIL)~\cite{wu2020connecting} that enables the use of different kernel sizes. In the following paragraph, we demonstrate the pipeline using $S^t$ as input. The same procedure is also implemented for $C^t$.
% \begin{wrapfigure}{R}{3.5cm}
%     %\centering
% \includesvg[height=5cm, width=7cm]{figures/neural_contrast/feature_encoder.svg}  
%     \label{fig: feature_encoder}
%     \caption{}
% \end{wrapfigure}

More specifically, we start by passing $S^t$ through a $\text{1D}$ convolution with a channel size of $d$ and a kernel size of $1$ to obtain its initial representation, $Z^t \in \R^{d \times c}$. Subsequently, we pass it through $L$ TCN blocks, with each containing a DIL layer followed by a batch normalization layer~\cite{ioffe2015batch}. The DIL operation is defined as
\begin{align}
& f_{\text{DIL}}(X) = (X \star f_{2}) \mathbin\Vert (X \star f_{3}) \mathbin\Vert (X \star f_{5}) \mathbin\Vert (X \star f_{7}) \nonumber
\end{align}
where $X \star f_k$ denotes a $\text{1D}$ temporal convolution layer applied to $X$ with a kernel size of $k$.
A batch normalization~\cite{ioffe2015batch} followed by a residual connection are added between each TCN block. After applying a sequence of TCN blocks, we obtain a final output with a dimension of $(d, 1)$, which is subsequently fed through another $\text{1D}$ convolution layer with a kernel size of $(1, 1)$ to derive the ultimate latent representation of $S^t$. We denote the latent representations of $S^t$ and $C^t$ as $O^t$ and $G^t$, respectively. The pipeline is shown in Figure~\ref{fig: feature_encoder} taking $S^t$ as the input.


% More specifically, we start by passing $S^t$ through a $\text{1D}$ convolution with a channel size of $d$ and a kernel size of $1$ to obtain its initial representation, $Z^t \in \R^{d \times c}$. Subsequently, we pass it through $L$ TCN blocks, each of which is defined as:
% \begin{align}
% Z^{t,l} = \text{BN}(\sigma(f_{\text{DIL}}(Z^{t, l-1}))) + Z^{t, l-1},
% \end{align}
% where $\text{BN}$ refers to a batch normalization layer~\cite{ioffe2015batch}, $\sigma$ represents a ReLU function, and $Z^{t, l}$ is the output from the $l^{th}$ block. The dilated inception layer is represented by $\text{DIL}$, which is defined as:
% \begin{align}
% & f_{\text{DIL}}(X) = X \star f_{2} \mathbin\Vert X \star f_{3} \mathbin\Vert X \star f_{5} \mathbin\Vert X \star f_{7},
% \end{align}
% where $X \star f_k$ denotes a $\text{1D}$ temporal convolution layer applied to $X$ with a kernel size of $k$, a dilation factor of $2^{(l-1)}$, and an output channel size of $\frac{d}{4}$, and the concatenation operation $\mathbin\Vert$ is performed on the channel dimension. We do not pad the sequences, and thus, each concatenation is performed on the truncated outputs from the four different convolutions, with the truncated size matching the length of the shortest output. After applying a sequence of TCN blocks, we obtain a final output with a dimension of $(d, 1)$, which is subsequently fed through another $\text{1D}$ convolution layer with a kernel size of $(1, 1)$ to derive the ultimate latent representation of $S^t$. We denote the latent representations of $S^t$ and $C^t$ as $O^t$ and $G^t$, respectively.

% \begin{wrapfigure}{r}{0.3\textwidth}
%   \begin{center}
%     %\includegraphics[width=0.48\textwidth]{birds}
%     \includesvg[height=4cm]{figures/neural_contrast/tcn_feature_encoder.svg} 
%   \end{center}
%   \caption{Birds}
% \end{wrapfigure}


% \begin{wrapfigure}{r}
%     %\centering
%    % \includesvg[width=1\linewidth]{figures/Framework.svg}
%         \includesvg[width=0.5\linewidth]{figures/neural_contrast/tcn_feature_encoder.svg}  
%     \caption{To be continued}
%     \label{fig:tcn feature encoder}
% \end{wrapfigure}





% In a nutshell, 
% the feature encoder first converts the input sequence into an inter-series graph. Next, a graph convolution module is applied on top of the adjacency matrix and the input sequence to obtain the final hidden representations of the graph. The general pipeline is defined as follows
% \begin{align}
%      & A^t = f_{\text{g}}(C^t) \\
%      & H^t = f_{\text{c}}(A^t, C^t) 
% \end{align}
% where $f_{\text{g}}(\cdot): R^{N \times c}\rightarrow R^{d}$ is the graph generator, and $f_{\text{c}}(\cdot): R^{N \times N} \times R^{N \times c} \rightarrow R^{N \times d}$ is the graph convolution module.

% \subsubsection{Graph generator} 
% The graph generator takes the sequence $C^t$ as the input and generates an adjacency matrix $A^t \in R^{N \times N}$. We adopt the simplest setting, where $A^t$ is generated based on the cosine distance between pairwise nodes. Other advanced graph generation approaches can be adapted to this framework as well, such as adding an additional graph sparsification layer as in~\cite{deng2021graph}. The graph generator is defined as
% \begin{align}
%     & A^t = D^{-1/2} \textnormal{ReLU}(S^t) D^{-1/2} \\
%     & S^t_{ij} = \frac{Z'_i^t Z'_j^t}{|Z'_i^t| |Z'_j^t|} \\
% % \end{align}
% % \begin{align}
%     & Z'^t = \text{ReLU}(f_{p2}(Z^t)W_1+b_1)W_2+b_2 \\
%     & Z^t = f_{p1}(C^t)
% \end{align}
% where $D$ is the degree matrix of the un-normalized adjacency matrix $S^t$, $f_{p1}(\cdot)$ is an 1D convolution layer with a channel size of $d$ and kernel size of $(1, 1)$, $f_{p2}(\cdot)$ is an 1D convolution layer with a channel size of $d$ and kernel size of $(1, c)$ followed by a transpose operation on time-axis and feature-axis, ($W_1\in R^{c \times d}$, $b_1 \in R^{d}$) and ($W_2 \in R^{d}$, $b_2 \in R$) are learnable weights and biases. 

% \subsubsection{Graph convolution}
% Given $Z^t$ and $A^t$ from the graph generator, we perform the following two operations iteratively for L times to obtain the node feature representations
% \begin{align}
%     & H^{t, l+1} = f_{tconv}(Z^{t, l}) \\
%     & Z^{t, l+1} = f_{gconv}(H^{t, l+1}, A^t)+H^{t,l+1}  
% \end{align}
% where $f_{\text{tconv}}$ is the dilated inception layer~\cite{wu2020connecting} and $f_{\text{gconv}}$ is a graph convolution layer~\cite{kipf2016semi}. dilated inception layer applies multiple 1D convolutions with different kernel sizes separately on top of the input sequence, and the obtained representation is a concatenation of the outputs from those convolutions. This step can be treated as local feature engineering, incorporating information from different granularity into each time tick. In addition, the receptive field of the dilation layer grows exponentially at a rate of 2, which is capable of capturing the long-term temporal dynamics of a time series and is computationally efficient compared to recurrent neural networks. 

% Finally, the output from the feature encoder $O^t \in R^{d}$ is obtained as
% \begin{align}
%     O^t = \text{Pooling}(\text{Concat}(H^{t, L}, Z^{t,L}, ..., H^{t,1}, Z^{t, 1}))
% \end{align}
% where the concatenation is performed on the time axis, and the mean pooling operation is taken on both the time dimension and the feature dimension. In particular, the output $O^t \in R^{d}$ can be treated as the representation of the generated graph, where the node features are temporal sequences encoded through a series of temporal convolution layers.



% \begin{figure}[t!]
% \centering
% \includesvg[height=3.5cm]{figures/neural_contrast/notation_graph.svg}  
% \caption{An illustrative example for the notations based on an input sample $X^t$.}
% \label{fig: notation_example}
% \end{figure}

% \begin{wrapfigure}{R}{}%[t!]
% \includesvg[height=3.5cm]{figures/neural_contrast/feature_encoder.svg}  
% \caption{An illustrative example for the notations.}
% \label{fig: notation_example}
% \end{wrapfigure}


% \begin{figure}[t!]
% \begin{subfigure}[t]{1\linewidth}
% \centering
% \includesvg[height=3.5cm]{figures/neural_contrast/Framework.svg}  
% \caption{Training Pipeline}
% \label{fig: framework}
% \end{subfigure}
% \hfill
% \centering
% \newline
% \vspace{0.05cm}
% \begin{subfigure}[t]{1\linewidth}
% \centering
% \includesvg[height=1.5cm]{figures/neural_contrast/feature_encoder.svg}  
% \caption{Feature Encoder}
% \label{fig: feature_encoder}
% \end{subfigure}
% \caption{The proposed framework: (a) The training pipeline: The blue dashed box indicates that the transformations of the predict sequence are pushing away among themselves while pulling towards the latent feature of the predict sequence. The orange dashed box indicates that the latent representation of the context sequence is pulling close to the transformations of the predict sequence; (b) The feature encoder architecture.}
% \end{figure}



\subsection{Optimization Framework}
\label{sec: optimizatino}
% Given the encoded feature representation $O^t$ for the suspect sequence and $G^t$ for the context sequence, the optimization module aims to minimize two losses: a contextual contrastive loss and a discriminative contrastive loss.

\subsubsection{Contextual Contrastive Loss Without Regularization}
% Our proposed framework is based on the assumption that normal sequences within the prediction window change mildly in comparison to abnormal sequences from recent history. To implement this idea, we contrast the prediction window with the context window by minimizing the distance between the hidden representations of the two windows for normal samples. This idea is inspired by DeepSVDD, which trains neural networks by minimizing the volume of a hypersphere that encloses normal data. However, instead of adopting a fixed hypersphere center, we allow the center to vary based on the context. By incorporating more information about the surrounding context, anomalies can be identified based on their abnormal pattern with respect to the past. This approach is better adapted to time series anomaly detection, where the majority of anomalies are contextually irregular.

Our framework assumes that normal sequences change mildly compared to abnormal sequences. To implement this idea, we pull closer the predict sequence with the context sequence by minimizing the distance between their hidden representations for normal samples. 
% This approach is inspired by DeepSVDD, but allows the center of the hypersphere to vary based on the context, better adapting it to time series anomaly detection where most anomalies are contextually irregular.

% Let $O^t$ and $Q^t$ be the encoded representation of the suspect sequence $P^t$ and context sequence $C^t$ from the feature encoder respectively. 
Formally, let $g(\cdot; W): \R^{N \times c} \rightarrow \R^d$ be the feature encoder in section~\ref{sec: feature encoder} with learnable weights $W$ (including biases). We define a contextual contrastive loss as
\begin{align}
   %&  \min_W L_{\text{ccl}} \\
   & L_{\text{ccl}}:= \EX_{X^t \sim \D}{ \|g(S^t;W) - g(C^t;W)\|}^2_2
    \label{eq. raw contextual one-class objective}
\end{align}
which is the mean Euclidean distance between the hidden representations of the predict sequence and context sequence. However, minimizing Eq.~\eqref{eq. raw contextual one-class objective} can lead to constant encoder solutions, which we refer to earlier as the representation collapse issue. Specifically, when the encoder always outputs a constant, the contrastive loss is zero, which is clearly the minimum value for a vector norm (see Section 4 for more details). 

% Specifically, the optimal solution of the objective can be trivially achieved when the output of the encoder is a constant for arbitrary input values (More details in section~\ref{sec:theoretical analysis}).

One way to avoid the constant encoder solution is to append an objective that enforces the encoder to produce different outputs under different contexts. In this work, we explore the combination of this contextual contrastive objective with neural transformation learning~\cite{qiu2021neural} for time series anomaly detection. 
% For example, we could let the encoder be optimized under the regression task or reconstruction task settings. 



\subsubsection{Combining With Neural Transformations}
Neural transformation learning learns diverse transformations that maintain the original sample's semantic information. We could leverage this approach to prevent the representation collapse, by contrasting the diverse but semantic-related hidden representations of the predict sequence, $O^t$, against the feature representation of the context sequence, $G^t$.

% In this case, the feature representation of the predict sequence are guaranteed to be contextually dependent on the given input, which avoids the constant encoder solution.
Formally, given the feature representation $O^t$, we project it into $K$ latent representations, denoted as $\{O^{t,i}\}_{i=1}^K$, using distinct transformation networks $T=\{T_1, ..., T_K|T_k:\R^d \rightarrow \R^d\}$. In our implementation, we choose three-layer MLPs with hidden dimension $d$ for $T_k$. In contrast to the original neural transformation learning, where transformations are applied to the raw inputs and fed through the feature encoder multiple times, we apply transformations directly to the hidden space to ease the computational burden. This allows us to apply the feature encoder only once, followed by $K$ lightweight transformation encoders, reducing the overall computation required.


% Formally, given the suspect feature representation $O^t$ from the feature encoder, we project it into K latent representations $\{O^{t,i}\}_{i=1}^K$ through distinct transformation networks $T=\{T_1, ..., T_K|T_k:\R^d \rightarrow \R^d\}$. In our implementation, we choose $T_k$ as a three-layer MLP with the same hidden dimension $d$ in each layer. Note that in the original neural transformation learning, transformations are applied to the raw inputs directly and each transformation has to be fed through the feature encoder once, which can be computationally expensive when the encoder has complex neural network architectures. In this work, we circumvent the computation burden by applying the transformation directly on the hidden space so that the feature encoder is applied only once followed by K lightweight transformation encoders.

Concretely, to ensure the K transformations are diverse and semantically similar to the original input, ~\cite{neuralAD} proposes a discriminative contrastive loss, which is defined as
\begin{align}
    L_{\text{dcl}}:= -\EX_{X^t \sim \D} \left[ \sum_{k=1}^K \log{\frac{h(O^t,O^{t, k})}{h(O^t,O^{t, k})+\sum_{l \neq k} h(O^{t, k}, O^{t, l})}} \right] 
\end{align}
%The scoring function $h(x, y)$ is denoted as
\begin{align}
    & h(x, y) = \exp(\text{sim}(x, y)/\tau) \\
    & \text{sim}(x, y) = \frac{x^Ty}{{\|x\|}_2{\|y\|}_2}
\end{align}
where $\tau$ is a hyperparameter called the temperature, and $K$ is the number of learnable transformations. %{\color{red}symbol}

To adapt the neural transformation loss to our framework, we re-define a contextual neural contrastive loss $L_{\text{cncl}}$ as
\begin{align}
        & L_{\text{cncl}} := \EX_{X^t \sim \D} \left[ \sum_{k=1}^K { \|O^{t, k} - G^t\|}^2_2 \right]
        \label{eq. contextual neural contrastive loss}
\end{align}
where the transformations of predict feature representation are pulled closer to the context feature representation. 

Finally, the model architecture, including the feature encoder and the neural transformations, is optimized under a contextual discriminative contrastive loss $L_\text{cdcl}$ during the training, which is defined as
% $L_{\text{lnctl}}$ as
\begin{align}
    & L_{\text{cdcl}} := L_{\text{cncl}} + L_{\text{dcl}} 
    \label{eq. contextual discriminative contrastive loss}
\end{align}
We prove in section~\ref{sec:theoretical analysis} that the edge case, where both the outputs of the transformations and the feature encoder generates the same constant, does not minimize the joint loss in Eq.~\eqref{eq. contextual discriminative contrastive loss}. 

During inference, the loss in Eq.~\eqref{eq. contextual discriminative contrastive loss} for an input at time $t+p-1$, i.e., $X^{t+p-1}$, is used as the anomaly score for time $t$. Thus, a shorter predict window size $p$ can introduce a smaller detection delay.
% where
% \begin{align}
%         & L_{\text{lcl}} := \sum_{t=1}^{T_{\text{train}}} \sum_{k=1}^K { \|O^{t, k} - G^t\|}^2 
% \end{align}
% our proposed model architecture, including the feature encoder and the neural transformations, is optimized under $L_\text{lcntl}$ during the training.









% Let $O^t$ and $Q^t$ be the encoded representation of the suspect sequence $P^t$ and context sequence $C^t$ from the feature encoder respectively. The local contrasting loss can be defined as
% \begin{align}
%     L_{\text{cocc}} ={ \|O^t - Q^t\|}^2 
%     \label{eq. contextual one-class loss}
% \end{align}
% which is the euclidean distance between the hidden representations of the suspect sequence and context sequence.

% Similar to the one-class classification loss, minimizing Eq.~\eqref{eq. contextual one-class loss} can lead to trivial solutions which is proved in the following proposition.

% \begin{proposition} \label{prop.constant_weights}
% have bias, leads to the constant solution.
% \end{proposition}

% first fed into a dilated inception layer (i.e., with kernel sets of $(2, 3, 5, 7)$ and channel size of $d$) to obtain a dense hidden representation $C^t \in R^{d \times N \times c}$. The dilated inception layer, proposed in~\cite{wu2020connecting}, applies multiple 1D convolutions with different kernel sizes separately on top of the input sequence, and the obtained representation is a concatenation of the outputs from those convolutions. This step can be treated as local feature engineering, which encapsulates information from different granularity to the hidden representation at a different time step.
% \begin{align}
%     & C^t = f_{\text{p}}(C^t) \\
%     & A'_{ij} = \frac{C'_i C'_j}{|C'_i| |C'_j|}\\
%     & A = D^{-1/2} \textnormal{ReLU}(A') D^{-1/2}
% \end{align}
% where $f_p$



% Given an input sequence $X_t \in R^{N \times c}$, the encoder breaks it into $m$ patches $\{S_{i,t}\}_{i=1}^m$ with $S_{i,t} \in R^{N \times w}$. Specifically, the operation is performed in parallel through a 2D convolution layer with a kernel size of $(1, w)$ and stride size of $w$, which guarantees that the patches are disjoint from each other. Additionally, a dilated inception layer with a kernel set of $(2, 3, 5, 7)$ is applied before the segmentation to preserve the local similarity within the sequence. 

% Next, the patches are converted into a series of graphs through graph structure learning. The operation for generating the graph for a given patch S is defined as
% \begin{align}
%     & S' = \textnormal{MLP}(S) \\
%     & A'_{ij} = \frac{S'_i S'_j}{|S'_i| |S'_j|}\\
%     & A = D^{-1/2} \textnormal{ReLU}(A') D^{-1/2} 
% \end{align}
% where MLP is a two-layer neural network, and $D$ is the degree matrix of the unnormalized adjacency matrix $A'$. Our intuition for constructing a series of graphs instead of a static graph is of two-folds. On the one hand, a static graph has limited power to model the timeseries with a time-varying relationship. On the other hand, our framework can identify anomalies based on the abnormal relationship changing from the context window to the suspect window, i.e., an anomaly that happened within the suspect window may have an inter-series relationship that deviates a lot from its historical graphs.

% Upon obtaining the list of graphs, we convert them into dense hidden representations by performing the graph convolution on top of each graph and their corresponding patch. We adopt the MixHop graph convolution, which is commonly used in time series-related tasks. The operation, proposed by~\cite{wu2020connecting}, is defined as 
% \begin{align}
%     & Z_i = \text{concat}(Z_i \star f_{1\times 2}, Z_i \star f_{1 \times 3}, Z_i \star f_{1 \times 5}, Z_i \star f_{1 \times 7}) \label{eq: dilated convolution} \\
%     & z \star f_{1 \times k}(t) = \sum^{k=1}_{s=0} f_{1 \times k}(s)z(t-ns) 
% \end{align}


% The framework XXXX is composed of a feature encoder and an optimization framework. The feature encoder aims to capture the dynamically evolving feature-wise relationship within a given input sequence, while the optimization framework 

% This section gives an overview of the proposed framework, XXXX. First, given an input sequence $X_t$, a feature encoder breaks it into patches and converts them into a series of dynamically evolving graphs. The graph convolution is then applied to each graph and the corresponding segment sequentially to obtain the hidden representation $Z_t$. Next, $Z_t$ is segmented into a context vector $Z_t^c$ and a suspect vector $Z_t^s$, and $Z_t^s$ is transformed through distinct neural networks to obtain $k$ different views $\{Z_{t, i}^s\}_{i=1}^k$. Finally, the framework is optimized under a contextual one-class loss and a neural transformation loss. The former loss aims to pull the transformed views of the suspect vector close to the context vector, while the latter prevents the hyper-sphere collapse problem of the former by making the views diverse while still preserving the semantics of the suspect vector. The intuition of the framework is that the intra-series temporal dynamic and the inter-series relationship within a normal sequence do not vary drastically in a relatively short period, i.e., the sequences within the context window and the suspect window are similar. 

==> subtexes/methodology_v3.tex <==
\subsection{Problem Formulation}
\label{sec: problem_formulation}
In this study, we are given a multivariate time series $X \in \R^{N\times T}$, collected over
\begin{wrapfigure}{r}{0.5\textwidth}
\vspace{-0.4cm}
    \includesvg[height=3.2cm]{figures/neural_contrast/notation_graph_small.svg}  
    \caption{An illustrative example for the notations based on an input sample $X^t$.}
    \label{fig: notation_example}
\vspace{-0.3cm}
\end{wrapfigure}
$T$ time ticks with $N$ features, as a training set. The goal is to detect anomalies in a test set, which is a time series with $N$ features collected over a different span of time ticks from the training set. The training sample set $\D$ contains sub-sequences extracted from $X$, i.e., $X$ is converted into sliding windows with stride 1. Here, a sample $X^t$ represents a collection of time ticks within a sliding
window of length $w$: $X^t=\{X_{\cdot i}\}_{i=t-w+1}^t$, where $X_{\cdot i} \in \R^{N}$ is the multivariate time series value at timestamp $i$. We aim at assigning an anomaly score to each time tick in the test set given a test sample, which is later threshold-ed to a binary label with 0 or 1 for normal or abnormal, respectively.
Furthermore, in our framework, each sample $X^t$ is segmented into two overlapping sub-sequences of length $c$, which we refer to as a context sequence $C^t$ and a predict sequence $S^t$. $S^t$ is shifted forward from $C^t$ by a small time window of length $p=w-c$, i.e., $C^t=\{X_{\cdot i}\}_{i=t-w+1}^{t-p}$ and $S^t = \{X_{\cdot i}\}_{i=t-c}^{t}$. The time window from $t-p+1$ to $t$ is referred to as the predict window, and the one from $t-w+1$ to $t-p$ is denoted as the context window. A visualization of notations is shown in 
Figure~\ref{fig: notation_example}.

\subsection{Overview}
This section presents an overview of the proposed framework, CNT, which includes a feature encoder module and a neural transformation module
with both jointly optimized using two contrastive losses (See Figure~\ref{fig: framework} for an illustration). Specifically, the framework begins with the feature encoder, which converts the predict and context
sequence of a given sample into hidden representations. Next, the neural transformation network transforms the latent representation of the predict sequence into multiple latent representations. Finally, model parameters are optimized under two loss functions: a contextual neural contrastive loss and a discriminative contrastive loss. 
The former aims at minimizing the distance between the transformations of predict sequence and context sequence. The latter ensures that the transformed sequences remain diverse while maintaining the original semantics of the predict sequence.

\begin{figure}[t!]
%\vspace{-0.4cm}
    \centering
\includesvg[height=3.5cm]{figures/neural_contrast/Framework_cnt_small.svg} 
\caption{Overview of CNT: the blue dashed box indicates the transformations of the predict sequence are pushing away among themselves while pulling towards the latent feature of the predict sequence. The orange dashed box indicates the latent representation of the context sequence is pulling closer to the transformations of the predict sequence.}
\label{fig: framework}
%\vspace{-0.3cm}
\end{figure}


\subsection{Feature Encoder}
\label{sec: feature encoder}
The feature encoder aims at capturing temporal dependencies within a predict or context sequence, thereby facilitating the detection of anomalies in the predict window by identifying anomalous temporal patterns with respect to the context window. 
We have defined two overlapping sequences - $C^t$ and $S^t$, with equal lengths, as discussed in Section~\ref{sec: problem_formulation}. 
Following the methodology employed by~\cite{wu2020connecting}, we have utilized a temporal convolutional network (TCN) as the base feature encoder, wherein the temporal convolution layer has been replaced by a dilated inception layer (DIL)~\cite{wu2020connecting} that enables the use of different kernel sizes. In the following paragraph, we demonstrate the pipeline using $S^t$ as input. 

More specifically, we start by passing $S^t$ through a $\text{1D}$ convolution with a channel size of $d$ and a kernel size of $1$ to obtain its initial representation, $Z^t \in \R^{d \times c}$. Subsequently, we pass it through $L$ TCN blocks, with each containing a DIL layer followed by a batch normalization layer~\cite{ioffe2015batch}. 
A batch normalization~\cite{ioffe2015batch} followed by a residual connection are added between each TCN block. After applying a sequence of TCN blocks, we obtain a final output with a dimension of $(d, 1)$, which is subsequently fed through another $\text{1D}$ convolution layer with a kernel size of $(1, 1)$ to derive the ultimate latent representation of $S^t$. We denote the latent representations of $S^t$ and $C^t$ as $O^t$ and $G^t$, respectively. See a visualization of the encoder in the supplementary materials.


\subsection{Optimization Framework}
\label{sec: optimizatino}
\subsubsection{Contextual Contrastive Loss Without Regularization}
Our framework assumes that normal sequences change mildly compared to abnormal sequences. To implement this idea, we pull closer the predict sequence with the context sequence by minimizing the distance between their hidden representations for normal samples. 

Formally, let $g(\cdot; W): \R^{N \times c} \rightarrow \R^d$ be the feature encoder in Section~\ref{sec: feature encoder} with learnable weights $W$ (including biases). We define a contextual contrastive loss as
\begin{align}
   %&  \min_W L_{\text{ccl}} \\
   & L_{\text{ccl}}:= \EX_{X^t \sim \D}{ \|g(S^t;W) - g(C^t;W)\|}^2_2
    \label{eq. raw contextual one-class objective}
\end{align}
which is the mean Euclidean distance between the hidden representations of the predict sequence and context sequence. However, minimizing Eq.~\eqref{eq. raw contextual one-class objective} can lead to constant encoder solutions, which we refer to earlier as the representation collapse issue. Specifically, when the encoder always outputs a constant, the contrastive loss is zero, which is clearly the minimum value for a vector norm (see Section~\ref{sec:theoretical analysis} for more details). 

One way to avoid the constant encoder solution is to append an objective that enforces the encoder to produce different outputs under different contexts. In this work, we explore the combination of this contextual contrastive objective with neural transformation learning proposed in NeuTralAD for time series anomaly detection. 

\subsubsection{Combining With Neural Transformations}
Neural transformation learning learns diverse transformations that maintain the original sample's semantic information. We could leverage this approach to prevent the representation collapse, by contrasting the diverse but semantic-related hidden representations of the predict sequence, $O^t$, against the feature representation of the context sequence, $G^t$.

Formally, given the feature representation $O^t$, we project it into $K$ latent representations, denoted as $\{O^{t,i}\}_{i=1}^K$, using distinct transformation networks $T=\{T_1, ..., T_K|T_k:\R^d \rightarrow \R^d\}$. In our implementation, we choose three-layer MLPs with hidden dimension $d$ for $T_k$. In contrast to the original neural transformation learning, where transformations are applied to the raw inputs and fed through the feature encoder multiple times, we apply transformations directly to the hidden space to ease the computational burden. This allows us to apply the feature encoder only once, followed by $K$ lightweight transformation encoders, reducing the overall computation required.

Concretely, to ensure the K transformations are diverse and semantically similar to the original input,~\cite{neuralAD} proposes a discriminative contrastive loss, which is defined as
\begin{align}
    L_{\text{dcl}}:= -\EX_{X^t \sim \D} \left[ \sum_{k=1}^K \log{\frac{h(O^t,O^{t, k})}{h(O^t,O^{t, k})+\sum_{l \neq k} h(O^{t, k}, O^{t, l})}} \right] 
\end{align}
\begin{align}
    & h(x, y) = \exp(\frac{x^Ty}{{\tau\|x\|}_2{\|y\|}_2}) 
\end{align}
where $\tau$ is a hyperparameter called the temperature, and $K$ is the number of learnable transformations. 

To adapt the neural transformation loss to our framework, we re-define a contextual neural contrastive loss $L_{\text{cncl}}$ as
\begin{align}
        & L_{\text{cncl}} := \EX_{X^t \sim \D} \left[ \sum_{k=1}^K { \|O^{t, k} - G^t\|}^2_2 \right]
        \label{eq. contextual neural contrastive loss}
\end{align}
where the transformations of predict feature representation are pulled closer to the context feature representation. 

Finally, the model architecture, including the feature encoder and the neural transformations, is optimized under a contextual discriminative contrastive loss $L_\text{cdcl}$ during training, which is defined as
\begin{align}
    & L_{\text{cdcl}} := L_{\text{cncl}} + L_{\text{dcl}} 
    \label{eq. contextual discriminative contrastive loss}
\end{align}
We prove in Section~\ref{sec:theoretical analysis} that the edge case, where both the outputs of the transformations and the feature encoder generates the same constant, does not minimize the joint loss in Eq.~\eqref{eq. contextual discriminative contrastive loss}. Furthermore, during inference, the loss in Eq.~\eqref{eq. contextual discriminative contrastive loss} for an input at time $t+p-1$, i.e., $X^{t+p-1}$, is used as the anomaly score for time $t$. Thus, a shorter predict window size $p$ can introduce a smaller detection delay.









% Let $O^t$ and $Q^t$ be the encoded representation of the suspect sequence $P^t$ and context sequence $C^t$ from the feature encoder respectively. The local contrasting loss can be defined as
% \begin{align}
%     L_{\text{cocc}} ={ \|O^t - Q^t\|}^2 
%     \label{eq. contextual one-class loss}
% \end{align}
% which is the euclidean distance between the hidden representations of the suspect sequence and context sequence.

% Similar to the one-class classification loss, minimizing Eq.~\eqref{eq. contextual one-class loss} can lead to trivial solutions which is proved in the following proposition.

% \begin{proposition} \label{prop.constant_weights}
% have bias, leads to the constant solution.
% \end{proposition}

% first fed into a dilated inception layer (i.e., with kernel sets of $(2, 3, 5, 7)$ and channel size of $d$) to obtain a dense hidden representation $C^t \in R^{d \times N \times c}$. The dilated inception layer, proposed in~\cite{wu2020connecting}, applies multiple 1D convolutions with different kernel sizes separately on top of the input sequence, and the obtained representation is a concatenation of the outputs from those convolutions. This step can be treated as local feature engineering, which encapsulates information from different granularity to the hidden representation at a different time step.
% \begin{align}
%     & C^t = f_{\text{p}}(C^t) \\
%     & A'_{ij} = \frac{C'_i C'_j}{|C'_i| |C'_j|}\\
%     & A = D^{-1/2} \textnormal{ReLU}(A') D^{-1/2}
% \end{align}
% where $f_p$



% Given an input sequence $X_t \in R^{N \times c}$, the encoder breaks it into $m$ patches $\{S_{i,t}\}_{i=1}^m$ with $S_{i,t} \in R^{N \times w}$. Specifically, the operation is performed in parallel through a 2D convolution layer with a kernel size of $(1, w)$ and stride size of $w$, which guarantees that the patches are disjoint from each other. Additionally, a dilated inception layer with a kernel set of $(2, 3, 5, 7)$ is applied before the segmentation to preserve the local similarity within the sequence. 

% Next, the patches are converted into a series of graphs through graph structure learning. The operation for generating the graph for a given patch S is defined as
% \begin{align}
%     & S' = \textnormal{MLP}(S) \\
%     & A'_{ij} = \frac{S'_i S'_j}{|S'_i| |S'_j|}\\
%     & A = D^{-1/2} \textnormal{ReLU}(A') D^{-1/2} 
% \end{align}
% where MLP is a two-layer neural network, and $D$ is the degree matrix of the unnormalized adjacency matrix $A'$. Our intuition for constructing a series of graphs instead of a static graph is of two-folds. On the one hand, a static graph has limited power to model the timeseries with a time-varying relationship. On the other hand, our framework can identify anomalies based on the abnormal relationship changing from the context window to the suspect window, i.e., an anomaly that happened within the suspect window may have an inter-series relationship that deviates a lot from its historical graphs.

% Upon obtaining the list of graphs, we convert them into dense hidden representations by performing the graph convolution on top of each graph and their corresponding patch. We adopt the MixHop graph convolution, which is commonly used in time series-related tasks. The operation, proposed by~\cite{wu2020connecting}, is defined as 
% \begin{align}
%     & Z_i = \text{concat}(Z_i \star f_{1\times 2}, Z_i \star f_{1 \times 3}, Z_i \star f_{1 \times 5}, Z_i \star f_{1 \times 7}) \label{eq: dilated convolution} \\
%     & z \star f_{1 \times k}(t) = \sum^{k=1}_{s=0} f_{1 \times k}(s)z(t-ns) 
% \end{align}


% The framework XXXX is composed of a feature encoder and an optimization framework. The feature encoder aims to capture the dynamically evolving feature-wise relationship within a given input sequence, while the optimization framework 

% This section gives an overview of the proposed framework, XXXX. First, given an input sequence $X_t$, a feature encoder breaks it into patches and converts them into a series of dynamically evolving graphs. The graph convolution is then applied to each graph and the corresponding segment sequentially to obtain the hidden representation $Z_t$. Next, $Z_t$ is segmented into a context vector $Z_t^c$ and a suspect vector $Z_t^s$, and $Z_t^s$ is transformed through distinct neural networks to obtain $k$ different views $\{Z_{t, i}^s\}_{i=1}^k$. Finally, the framework is optimized under a contextual one-class loss and a neural transformation loss. The former loss aims to pull the transformed views of the suspect vector close to the context vector, while the latter prevents the hyper-sphere collapse problem of the former by making the views diverse while still preserving the semantics of the suspect vector. The intuition of the framework is that the intra-series temporal dynamic and the inter-series relationship within a normal sequence do not vary drastically in a relatively short period, i.e., the sequences within the context window and the suspect window are similar. 

==> subtexes/preliminary.tex <==
\section{Preliminary}
In this section, we provide a brief review of two methods closely related to our work, DeepSVDD and Neutral AD. 
% Additionally, we provide a review for anomaly detection methods that are similar to our approach.

\subsection{DeepSVDD}
\label{sec: DeepSVDD}
DeepSVDD is an unsupervised learning method that aims to learn a compact representation of the normal class using a neural network encoder. Specifically, under the semi-supervised setting where the majority of training data are assumed to be normal instances, DeepSVDD seeks to map all instances into a hypersphere of minimum volume. This is achieved by minimizing the following objective function:
\begin{align}
\min_{\theta,c} \frac{1}{N} \sum^N_{i=1} \|\phi(x_i;\theta)-c\|^2_2 + \lambda \Omega(\theta),
\end{align}
where $x_i$ denotes the $i$-th instance out of $N$ training samples, $\phi(\cdot)$ is a neural network with parameter $\theta$ that encodes a given input into its latent representation, and $c$ represents the center of the hypersphere. The regularization term, $\lambda \Omega(\theta)$, typically takes the form of an $l_2$ regularization, which encourages the model's weights to be small and reduces the model's complexity. The selection of the center $c$ in the objective function is crucial to prevent a hypersphere collapse issue, which occurs when all instances are simply mapped to a constant. 
% A theoretical analysis is provided in the paper~\cite{deepSVDD} that a constant encoder solution may arise when either the parameter $\theta$ is set to zero, or when $\phi(\cdot)$ includes bias terms or bounded activation functions. Therefore, the center is typically assigned as the mean of the encoded inputs after an initial forward pass of the encoder in practice. Moreover, it is recommended to avoid using bias terms and bounded activation functions in the encoder to circumvent the constant encoder solution problem.

\subsection{NeuTral AD}
\label{sec: neutral AD}
% The idea of Neutral AD is inspired by the recent progress of self-supervised learning techniques that are primarily intended for anomaly detection in vision domain. These methods commonly adopt an augmentation prediction approach, which involves generating a set of samples by applying various data augmentation operations (primarily geometric transformations) to each input image, and then training a model to classify the specific augmentation that a given augmented sample corresponds to. Some examples of works are~\cite{geoTransformation},~\cite{robustAndUncertainty}, and~\cite{inlier}. The hypothesis is that a self-supervised approach will give priority to solving its training task for inliers. However, one significant limitation of these techniques is their reliance on hand-crafted transformations that are specialized for image data, and designing such transformations for data beyond images may be a daunting task. To overcome this challenge, the NeuTral AD framework proposed by~\cite{neuralAD} employs learnable transformations. In this framework, the transformed data is embedded into a semantic space that maintains the similarity of the transformed data to their original form while enabling easy differentiation between different transformations via separation in the representation space.

The idea of NeuTral AD is inspired by the recent progress of self-supervised learning techniques that are primarily intended for anomaly detection in vision domain. These techniques adopt an augmentation prediction approach that generates a set of samples by applying various data augmentation operations to input images, training a model to classify the specific augmentation corresponding to an augmented sample~\cite{geoTransformation},~\cite{robustAndUncertainty}, and~\cite{inlier}. However, majority of them rely on hand-crafted transformations specialized for image data, making it challenging to design such transformations for data beyond images. To overcome this challenge, NeuTral AD~\cite{neuralAD} employs learnable transformations to embed transformed data into a semantic space that maintains the similarity of the transformed data to their original form while enabling easy differentiation between different transformations via separation in the representation space.

The NeuTral AD approach utilizes a determinative contrastive loss to enable the use of learnable transformations. Given an input sample $x$, the loss is defined as:
\begin{align}
& \LL = -\sum^K_{k=1}\log\frac{h(x^{k}, x^0)}{h(x^{k}, x^0)+\sum_{l\neq k}h(x^{k}, x^{l})}
\end{align}
Here, $h(x^k, x^l)$ is defined as:
\begin{align}
%& h(x^k, x^l) = \text{exp}(\text{sim}(f_{\phi}(T_k(x)), f_{\phi}(T_l(x)))/\tau)
& h(x^k, x^l) = \text{exp}(\text{sim}(f_{\phi}(x^k), f_{\phi}(x^l))/\tau) \\
& x^k = T_k(x)
\end{align}
where $\tau$ is a hyperparameter called temperature, $\text{sim}(\cdot, \cdot)$ computes the cosine similarity between two inputs, $T_k(\cdot)$ is the $k^{th}$ transformation function that maps the original data into a different subspace of the same dimension as the input (e.g., via an MLP), $T_0(\cdot)$ is an identity function, $K$ is the number of learnable transformations, and $f_{\phi}(\cdot)$ is an encoder network that extracts latent information from different transformed inputs.

==> subtexes/related_works.tex <==
\subsection{Deep Time Series Anomaly Detection}
The mainstream deep time series anomaly detection approaches are forecasting-based and reconstruction-based methods. Forecasting-based methods predict future values and identify anomalies as data points deviating from predictions. Reconstruction-based methods reconstruct input data and identify anomalies as data points that cannot be accurately reconstructed. Existing works for forecasting-based methods generally leverage various neural network architectures like LSTMs, GRUs, TCNs, GNNs, Transformers, or hybrid combinations to capture the temporal patterns and inter-series relationships~\cite{lstm-ndt,gdn,mtad-gat,grelen,gta,tcnanomaly}. Reconstruction-based methods include deep autoencoders (AEs)~\cite{omnianomaly,grelen,anomalyTransformer,anomalybert} and Generative Adversarial Networks (GANs)~\cite{mad-gan,tanogan} with varying underlying sequence encoder architectures aiming to learn the characteristics within time series. 

Apart from the above approaches, one-class classification methods are also widely used in anomaly detection tasks, which have the objective of learning a model of normal data and identifying anomalies as data points outside this model. One popular method in this category is DeepSVDD~\cite{deepSVDD}, which employs a deep neural network to map the input data into a high-dimensional feature space and learns a hypersphere that encapsulates the normal data. Recent works adapt the idea of DeepSVDD to time series data, either by employing advanced sequence encoders such as RNN-based and CNN-based networks~\cite{coca,couta} or incorporating additional training objectives to account for local temporal dependencies~\cite{OCPAE}. 

\subsection{Self-supervised Learning-based Anomaly Detection}
\label{sec: self-supervised-learning}
Self-supervised learning is a process that involves training a model on a certain auxiliary task using unsupervised learning, where the learned representation can be applied to downstream tasks such as regression or classification without the need for explicit labels
or annotations. Self-supervised methods have recently gained attention in the domain of anomaly detection. The techniques under this branch can be generally divided into two categories: augmentation prediction-based and contrastive learning-based approaches. 

Augmentation prediction involves generating a set of samples by applying various data augmentation operations to each input instance and then training a model to classify the specific augmentation that a given augmented sample corresponds to~\cite{geoTransformation,robustAndUncertainty,inlier}. However, the majority of them rely on hand-crafted transformations specialized for image data, making it challenging to design such transformations for data beyond images. To overcome this challenge, NeuTral AD~\cite{neuralAD} employs learnable transformations to embed transformed data into a semantic space that maintains the similarity of the transformed data to their original form while enabling easy differentiation between different transformations via separation in the representation space. 

Contrastive learning brings together representations of data instances and their augmented versions (or similar instances) while pushing away negative samples. A seminal work in this field is Contrastive Predictive Coding (CPC)~\cite{cpc}, which is tailored specifically to sequential data. ~\cite{tsCPCAD} adapt the idea of CPC to time series anomaly detection, where the InfoNCE loss of each sample serves as an anomaly score. However, the negative samples used to compute the loss are all selected from normal instances of training data, which contradicts the assumption that normal samples are typically clustered together in a
feature space~\cite{deepSVDD}. In contrast, other
contrastive learning approaches, such as BYOL~\cite{byol}, Simsiam~\cite{simsiam}, and VICReg~\cite{vicreg}, do not require negative samples. These methods aim to avoid the manifold collapse that arises from only contrasting positive
samples. VICReg has been applied in a recent work~\cite{coca}, which adopts a contrastive learning approach for time series anomaly detection, with a contrastive loss function regularized by a variance term to prevent representation collapse. 

One approach similar to our method is LNT~\cite{lnt}, which employs learnable transformations on $k$ step ahead time series values, treating these transformations and their corresponding context window as positive pairs for contrastive learning. To mitigate the representation collapse issue, they integrate the CPC objective, which contrasts $k$-step future representations against negative samples. Our method, however, offers a simpler, more efficient sequence-level contrasting technique. Moreover, we tackle the representation collapse problem by incorporating an additional contrasting layer between the input time window and its learnable transformations, which inherently bypasses the representation collapse issue without introducing negative samples.


% One approach similar to our method is LNT~\cite{lnt}, which applies learnable transformations on $k$ step ahead time series, with these transformations and their context window serving as contrastive learning's positive pairs. To circumvent the representation collapse issue, they utilize the CPC objective. In contrast, our method offers a simpler and more efficient sequence-level contrasting objective and addresses the representation collapse issue by introducing an additional contrasting layer (following~\cite{neuralAD}) between the input time window and its learnable transformations.

% These training paradigms may have limitations in certain scenarios. Forecasting-based methods may struggle when the time series is difficult to predict, such as rapidly changing or noisy sequences~\cite{lstmed}. Reconstruction-based methods may suffer from the identity mapping problem. Researchers have proposed various techniques, such as regularization and additional constraints, to address these limitations~\cite{gong2019memorizing}. One-class classification may have limitations when the distribution of normal instances is complex to be encoded with one hypersphere, especially for time series 

==> subtexes/related_works_IS.tex <==
\subsection{Deep Time Series Anomaly Detection}
The mainstream deep learning-based TSAD approaches can be generally categorized into forecasting-based and reconstruction-based methods. Forecasting-based methods predict future values and identify anomalies as data points deviating from predictions. Existing works leverage different neural network architectures such as LSTMs, CNNs, GNNs, and Transformers to encode time series before feeding to the forecasting task~\cite{lstm-ndt}~\cite{tcnanomaly}~\cite{gdn}~\cite{fusagnet}~\cite{gta}. For example, LSTM-NDT~\cite{lstm-ndt} employs LSTMs to encode time series data, which is subsequently employed to predict one-step time series values based on historical observations. GDN~\cite{gdn} constructs a learnable graph that describes the dependencies within multivariate time series. It then uses GNNs to encode time series and perform prediction-based detection. Similarly, FuSAGNet~\cite{fusagnet} leverages GNNs as the backbone encoder for the time series forecasting, and employs sparse autoencoder to enhance the learning of time series feature representation.

Reconstruction-based methods are techniques that identify anomalies by learning a model of the normal patterns within the data, either through direct reconstruction or by modeling the data distribution to generate new, similar data points. Anomalies are detected based on the deviation from these normal patterns, which is quantified by reconstruction errors or the inability of the model to accurately generate data resembling the input. Representative TSAD methods in this line of research are techniques based on deep autoencoders (AEs) and Generative Adversarial Networks (GANs)~\cite{mad-gan}~\cite{usad}~\cite{lstm-vae}~\cite{ mscred}~\cite{tranAD}~\cite{fusagnet}~\cite{grelen}~\cite{anomalyTransformer}~\cite{chen2023adversarial}. For example, LSTM-VAE~\cite{lstm-vae} integrates LSTM for temporal dynamics and employs a Variational AutoEncoder (VAE) for sequence reconstruction. MAD-GAN~\cite{mad-gan} combines a GAN model with a reconstruction-based model using LSTM, utilizing both discriminator outputs and reconstruction results to assign anomaly scores. DAEMON~\cite{chen2023adversarial} adopts an autoencoder in conjunction with dual discriminators within an adversarial learning setup to capture the normality in time series data. 


% Reconstruction-based methods reconstruct input data and identify anomalies as data points that cannot be accurately reconstructed. 
% Reconstruction-based methods are techniques that identify anomalies by learning a model of the normal patterns within the data, either through direct reconstruction or by modeling the data distribution to generate new, similar data points. Anomalies are detected based on the deviation from these normal patterns, which is quantified by reconstruction errors or the inability of the model to accurately generate data resembling the input. Representative works in this line of research are methods based on deep autoencoders (AEs) and Generative Adversarial Networks (GANs)~\cite{mad-gan,usad,lstm-vae, mscred,tranAD,fusagnet,grelen,chen2023adversarial}. For instance, LSTM-VAE~\cite{omnianomaly} employs LSTM as the backbone for temporal modeling and uses Variational AutoEncoder (VAE) for sequence reconstruction. 
% MAD-GAN~\cite{mad-gan} trains a GAN model on top of a reconstruction model with LSTM as the base architecture, and the outputs from both the discriminator and the reconstruction process are used to compute an anomaly score for each sample.
% DAEMON~\cite{chen2023adversarial} uses an autoencoder along with two discriminators in an adversarial training framework to learn the normal patterns of time series data. The detection of anomalies is based on the reconstruction errors, which are a measure of how well the autoencoder can reconstruct the input data. 


\subsection{Self-supervised Learning-based Methods}
\label{sec: self-supervised-learning}
self-supervised methods have garnered attention in the field of anomaly detection recently due to their ability to leverage unlabeled data, harnessing intrinsic data properties to uncover subtle anomalies. Those methods can be generally categorized into augmentation prediction-based and contrastive learning-based approaches. Augmentation prediction involves generating a set of samples by applying various data augmentation operations to each input instance and then training a model to classify the specific augmentation that a given augmented sample corresponds to~\cite{geoTransformation}~\cite{robustAndUncertainty}~\cite{inlier}. However, most of them rely on hand-crafted transformations specialized for image data, making it challenging to design such transformations for data beyond images. To overcome this challenge, NeuTral AD~\cite{neuralAD} employs learnable transformations to embed transformed data into a semantic space that maintains the similarity of the transformed data to their original form while enabling easy differentiation between different transformations via separation in the representation space. 

Contrastive learning brings together representations of data instances and their augmented versions or similar instances while pushing away negative samples. A seminal work in this field is CPC, which is tailored specifically to sequential data. Recently, quite a few works have adapted contrastive learning into TSAD~\cite{tsCPCAD}~\cite{cae-ad}~\cite{dcad}~\cite{coca}~\cite{yang2023dcdetector}. 
For example, CAE-AD~\cite{cae-ad} explores the concept of contextual contrasting, akin to CPC, to discern temporal patterns within time series data. It applies data augmentation in both the time and frequency domains, promoting similarity in the representations of augmented instances through instance-level contrast. Similarly, DCAD~\cite{dcad} leverages an attention mechanism and a position-aware convolution module to extract both global and local features from time series and their subsequences. It employs a contrastive loss to foster alignment between these global and local representations.

However, a common challenge with these methods is the selection of negative samples from the pool of training instances, which might conflict with the notion that normal samples tend to cluster together in the feature space. To address this, alternative contrastive learning strategies, such as BYOL~\cite{byol}, Simsiam~\cite{simsiam}, and VICReg~\cite{vicreg}, eliminate the need for negative samples. These approaches focus on preventing the potential collapse of the feature manifold, which could occur when only positive samples are contrasted.
VICReg, for instance, has been adapted for TSAD by COCA~\cite{coca}, which employs a contrastive learning paradigm optimized with a variance term to avoid the collapse of representations. Similarly, DCdetector~\cite{yang2023dcdetector} introduces a dual attention mechanism to learn distinct time series representations from both a patch-wise and within-patch perspective, utilizing a siamese network structure akin to Simsiam but without the need for negative samples, thereby sidestepping the manifold collapse issue.

% For instance, CAE-AD~\cite{cae-ad} implements a contextual contrasting similar to CPC capture temporal patterns within time series. It also explores data augmentation on time series in both time and frequency domains and encourages the representation of the two augmentations to be similar through an instance contrast. DCAD~\cite{dcad} uses an attention module and a position-aware convolution module to extract global and local features of the whole time series and its sub-sequence and optimize a contrastive loss that encourages the alignment between the global and local features. Those methods generally select negative samples from training instances, which may contradict the assumption that normal samples are typically clustered together in a feature space~\cite{deepSVDD}. In contrast, other
% contrastive learning approaches, such as BYOL~\cite{byol}, Simsiam~\cite{simsiam}, and VICReg~\cite{vicreg}, do not require negative samples. These methods aim to avoid the manifold collapse that arises from only contrasting positive
% samples. VICReg~\cite{vicreg} has been applied to TSAD by COCA~\cite{coca}, which adopts a contrastive learning approach for time series anomaly detection, with a contrastive loss function regularized by a variance term to prevent representation collapse. DCdetector~\cite{yang2023dcdetector} uses a dual attention structure to learn representations of time series from a patch-wise and in-patch view. It then contrasts the two views without negative samples, since it adopts a siamese model with a stopping gradient similar to Simsiam. 


==> subtexes/related_works_v2.tex <==

% \subsection{Deep Time Series Anomaly Detection}
% The mainstream deep time series anomaly detection approaches are forecasting-based and reconstruction-based methods. Forecasting-based methods predict future values and identify anomalies as data points deviating from predictions. Reconstruction-based methods reconstruct input data and identify anomalies as data points that cannot be accurately reconstructed. Existing works for forecasting-based methods generally leverage various neural network architectures like LSTMs, GRUs, TCNs, GNNs, Transformers, or hybrid combinations to capture the temporal patterns and inter-series relationships~\cite{lstm-ndt,gdn,mtad-gat,grelen,gta,tcnanomaly}. Reconstruction-based methods include deep autoencoders (AEs)~\cite{omnianomaly,grelen,anomalyTransformer,anomalybert} and Generative Adversarial Networks (GANs)~\cite{mad-gan,tanogan} with varying underlying sequence encoder architectures aiming to learn the characteristics within time series. 
% Apart from the above approaches, one-class classification methods are also widely used in anomaly detection tasks, which have the objective of learning a model of normal data and identifying anomalies as data points outside this model. One popular method in this category is DeepSVDD~\cite{deepSVDD}, which employs a deep neural network to map the input data into a high-dimensional feature space and learns a hypersphere that encapsulates the normal data. Recent works adapt the idea of DeepSVDD to time series data, either by employing advanced sequence encoders such as RNN-based and CNN-based networks~\cite{coca,couta} or incorporating additional training objectives to account for local temporal dependencies~\cite{OCPAE}. 

% \subsection{Self-supervised Learning-based Anomaly Detection}

\label{sec: self-supervised-learning}
In this section, we focus primarily on reviewing the literature of self-supervised learning-based anomaly detection methods that are directly related to our work. A brief review of general deep-learning-based time series anomaly detection methods is presented in Section 5 of the supplementary materials. Self-supervised methods under this branch can be generally divided into two categories: augmentation prediction-based and contrastive learning-based approaches. 

Augmentation prediction involves generating a set of samples by applying various data augmentation operations to each input instance and then training a model to classify the specific augmentation that a given augmented sample corresponds to~\cite{geoTransformation,robustAndUncertainty,inlier}. However, the majority of them rely on hand-crafted transformations specialized for image data, making it challenging to design such transformations for data beyond images. To overcome this challenge, NeuTral AD~\cite{neuralAD} employs learnable transformations to embed transformed data into a semantic space that maintains the similarity of the transformed data to their original form while enabling easy differentiation between different transformations via separation in the representation space. 

Contrastive learning brings together representations of data instances and their augmented versions (or similar instances) while pushing away negative samples. A seminal work in this field is CPC, which is tailored specifically to sequential data. The work~\cite{tsCPCAD} adapts the idea of CPC to time series anomaly detection, where the InfoNCE loss of each sample serves as an anomaly score. However, the negative samples used to compute the loss are all selected from normal instances of training data, which contradicts the assumption that normal samples are typically clustered together in a
feature space~\cite{deepSVDD}. In contrast, other
contrastive learning approaches, such as BYOL~\cite{byol}, Simsiam~\cite{simsiam}, and VICReg~\cite{vicreg}, do not require negative samples. These methods aim to avoid the manifold collapse that arises from only contrasting positive
samples. 
% COCA VICReg has been applied to TSAD by the work~\cite{coca}, which adopts a contrastive learning approach for time series anomaly detection, with a contrastive loss function regularized by a variance term to prevent representation collapse. 

One approach similar to our method is LNT~\cite{lnt}, which employs learnable transformations on $k$ step ahead time series values, treating these transformations and their corresponding context window as positive pairs for contrastive learning. To mitigate the representation collapse issue, they integrate the CPC objective, which contrasts $k$-step future representations against negative samples. Our method, however, offers a simpler, more efficient sequence-level contrasting technique. Moreover, we tackle the representation collapse problem by incorporating an additional contrasting layer between the input time window and its learnable transformations, which inherently bypasses the representation collapse issue without introducing negative samples.


% One approach similar to our method is LNT~\cite{lnt}, which applies learnable transformations on $k$ step ahead time series, with these transformations and their context window serving as contrastive learning's positive pairs. To circumvent the representation collapse issue, they utilize the CPC objective. In contrast, our method offers a simpler and more efficient sequence-level contrasting objective and addresses the representation collapse issue by introducing an additional contrasting layer (following~\cite{neuralAD}) between the input time window and its learnable transformations.

% These training paradigms may have limitations in certain scenarios. Forecasting-based methods may struggle when the time series is difficult to predict, such as rapidly changing or noisy sequences~\cite{lstmed}. Reconstruction-based methods may suffer from the identity mapping problem. Researchers have proposed various techniques, such as regularization and additional constraints, to address these limitations~\cite{gong2019memorizing}. One-class classification may have limitations when the distribution of normal instances is complex to be encoded with one hypersphere, especially for time series 

==> subtexes/theoretical_analysis.tex <==
In this section, we delve into a comprehensive analysis of the representation collapse issue that arises when applying solely the contextual contrastive loss, and why the integration of a discriminative contrastive loss can mitigate this problem.

First, we show that a constant feature encoder is an optimal solution for minimizing the contextual contrastive loss in Eq.~\eqref{eq. raw contextual one-class objective}. This suggests that the feature encoder might not extract meaningful semantics from the input data.
\label{sec:theoretical analysis}
\begin{proposition}
 Given the feature encoder $g(\cdot;W)$ in Section~\ref{sec: feature encoder}, there exists a choice of parameters for $W$ such that the output of $g(\cdot;W)$ is always a constant, i.e., $\exists W^*, c^* \ s.t. \ g(x; W^*) = c^*, \forall x$. In this case, $W=W^*$ is an optimal solution for minimizing the loss in Eq.~\eqref{eq. raw contextual one-class objective}.
 \label{props: constant encoder}
\end{proposition}

Proof. Following the work proposed by~\cite{deepSVDD}, there are three settings that can lead to a constant encoder solution: 1. $W=\boldsymbol{0}$; 2. When the encoder is equipped with bias terms in some hidden layers. 3. When the encoder contains bounded activations. In all cases, the loss in Eq.~\eqref{eq. raw contextual one-class objective} reaches the minimum.  \qed

Next, we show that the constant encoders do not lead to the optimal solution of minimizing the contextual discriminative contrastive loss in Eq.~\eqref{eq. contextual discriminative contrastive loss} under certain conditions.

\begin{proposition}
If there exists a choice of parameters for the feature encoder $g(\cdot)$ and the $K$ transformation networks $\{T_k(g(\cdot))\}_{k=1}^K$ such that $L_\text{dcl} < K \log K$, then the constant parameter setting $T_k(g(\cdot)) = g(\cdot) = c, \forall c \in \R^d$ is not an optimal solution for minimizing $L_{\text{cdcl}}$.
\label{props: non-constant encoder}
\end{proposition}

\textbf{Proof.} For simplicity, let $g_k(\cdot)$ denote $T_k(g(\cdot))$. First, note that when $g_k(\cdot) = g(\cdot) = c$, the contextual discriminative contrastive loss $L_{\text{cdcl}}$ is given by $K \log K$. 

Specifically, we have:
\begin{align}
L_{\text{cdcl}} & = L_{\text{cncl}} + L_{\text{dcl}}\\
& = K \| c - c \|^2_2-K\log {\frac{c'}{c'+(K-1)c'}} \\
& = K\log K
\end{align}
where $c' = h(c, c)$. 

Assuming that there exists a parameter setting such that $L_{\text{dcl}} < K \log K$, let $\epsilon = K \log K - L_{\text{cdcl}}$. Since the scoring function $h(\cdot, \cdot)$ in $L_{\text{dcl}}$ is defined as $h(g_k(\cdot), g(\cdot)) = \exp(\frac{g_k(\cdot)^Tg(\cdot)}{\tau\|g_k(\cdot)\|_2\|g(\cdot)\|_2})$, we can rescale the functions $\{g_k(\cdot)\}_{k=1}^{K}$ and $g(\cdot)$ during training such that $\| g_k(x)\|_2 \leq \frac{\epsilon}{2K}$ and $\| g(x)\|_2 \leq \frac{\epsilon}{2K}$ for all $x$. This rescaling is possible while ensuring that $h(g_k(x), g(x))$ remains the same, since cosine similarity between two vectors is invariant to their norms. Hence, we have:
\begin{align}
L_{\text{cncl}} = & \EX_{X^t\sim \D} \left[ \sum_{k=1}^K \| g_k(O^t) - g(G^t) \|^2_2 \right] \\
\leq & \EX_{X^t\sim \D}\left[  \sum_{k=1}^K (\| g_k(O^t)\|^2_2 + \| g(G^t) \|^2_2) \right]\\
< & \sum_{k=1}^K (\frac{\epsilon}{2K}+\frac{\epsilon}{2K}) =  \epsilon
\end{align}
Therefore, we have $L_{\text{cncl}} + L_{\text{dcl}} < \epsilon + L_{\text{dcl}} = \epsilon + K \log K - \epsilon = K \log K$. \qed


The intuition that $K\log K$ does not lead to the minimum solution of $L_{\text{dcl}}$ is that the objective of minimizing this loss function is to make sure that the generated transformations are diverse among themselves while preserving certain semantic similarities from a given input, which contradicts the constant encoder solution. 

Figure~\ref{fig: loss_decay} shows the loss values per epoch for our model training under purely $L_{\text{ccl}}$ loss or training under both $L_{\text{cncl}}$ and $L_{\text{dcl}}$ (the default setting). It is clear that $L_{\text{ccl}}$ decays quickly to 0 without the regularization of $L_{\text{dcl}}$. In contrast, with the additional constraints of $L_{\text{dcl}}$, $L_{\text{cncl}}$ decays much slowly compared to the former, which agrees with Proposition~\ref{props: constant encoder}. In addition, the loss value of $L_{\text{dcl}}$ quickly falls below $K\log K$, which is around 4.67 when $K=6$ (the default parameter setting used in our experiments). This verifies the assumption in Proposition ~\ref{props: non-constant encoder} is empirically applicable.

\begin{figure}[t!]
\centering
\includegraphics[height=3.5cm]{figures/neural_contrast/loss_decay.eps}  
\caption{The loss values per epoch for our model training under two scenarios on the WADI dataset. The small window is the zooming region for loss values from 20 to 30 epochs.}
\label{fig: loss_decay}
\end{figure}
















%\section{Theoretical Analysis}
% First, we prove that a constant feature encoder is an optimal solution for minimizing the contextual contrastive loss in e.q.~\ref{eq. raw contextual one-class objective}.
% \label{sec:theoretical analysis}
% \begin{proposition}
% % For some input space $\chi \in R^{N \times d}$ and output space $F \in {R^d}$,
% % Define the objective as
% % \begin{align}
% %         \min_{W}{\| g(x_1, W) - g(x_2, W)\|}^2 
% %     \label{eq. contextual one-class loss}
% % \end{align}
% % where $x_1, x_2 \in \chi$. 
%  Given the feature encoder $g(\cdot;W)$ in \ref{sec: feature encoder}, there exists a choice of parameters for $W$ such that the output of $g(\cdot;W)$ is always a constant, i.e., $\exists W^*, c^* \ s.t. \ g(x; W^*) = c^*, \forall x$. In this case, $W=W^*$ is an optimal solution for minimizing the loss in e.q.~\ref{eq. raw contextual one-class objective}.
% \end{proposition}

% Proof. Following the work~\cite{deepSVDD}, there are three settings that can lead to a constant encoder solution: 1. $W=\boldsymbol{0}$; 2. When the encoder is equipped with bias terms in some hidden layers. 3. When the encoder contains bounded activations. In all cases, the loss in eq.~\ref{eq. raw contextual one-class objective} reaches the minimum.  \qed
% % One parameter setting is to let $W=\boldsymbol{0}$, the all-zero-weights solution. In this case, $g(x;W)=0, \forall x$. As the encoder is equip-ed with bias term in some hidden layers, there exists arbitrary $c^* \in R^d$ such that $g(x; W^*) = c^*$, as proved in~\cite{deepSVDD}. In either case, the loss in eq.~\ref{eq. raw contextual one-class objective} reaches the minimum.

% Next, we show that the constant encoders do not lead to the optimal solution of minimizing the contextual discriminative contrastive loss in e.q.~\ref{eq. contextual discriminative contrastive loss}.

% % \begin{proposition}
% %  If there exists a choice of parameters for the feature encoder $g(\cdot)$ and the K transformation networks $\{T_k(g(\cdot))\}_{k=1}^K$ such that $L_\text{cdcl}<KlogK$, then the constant parameter setting, i.e., $T_k(g(\cdot))=g(\cdot)=c, \forall c \in R^d$, is not an optimal solution to minimize $L_{\text{cdcl}}$. 
% % \end{proposition}

% % Proof. For simplicity, we denote $T_k(g(\cdot))$ as $g_k(\cdot)$. First, note that the constant parameter setting results in $L_{\text{cdcl}}=KlogK$. More specifically, when $g_k(\cdot)=g(\cdot)=c, \forall c \in R^d$, the contextual discriminative contrastive loss for an input sample $X^t$ is
% % \begin{align}
% %     L^t_{\text{cdcl}} & = L^t_{\text{cncl}} + L^t_{\text{dcl}}\\
% %     & = K \| c - c \|^2_2-K\log {\frac{c'}{c'+(K-1)c'}} \\
% %     & = KlogK
% % \end{align}
% % Here, we denote $h(c, c)=c'$.
% % % $L_{\text{lnc}} = \| c - c \|^2= 0, L_{\text{ntl}} = -K\log {\frac{C}{C+(K-1)C}} = KlogK, \forall c\in R^d$. 

% % Assumming there exists a parameter setting such that $L_{\text{dcl}}<KlogK$, let $\epsilon = KlogK - L_{\text{cdcl}}$. Since the scoring function $h(\cdot, \cdot)$ in $L_{\text{dcl}}$ is defined as $h(g_k(\cdot), g(\cdot)) = \exp(\frac{g_k(\cdot)g(\cdot)}{\|g_k(\cdot)\|_2\|g(\cdot)\|_2})$, the functions $\{g_k(\cdot)\}_{k=0}^{K}$ and $g(\cdot)$ can be re-scaled during training such that $\| g_k(x)\| \leq \frac{\epsilon}{2K}$,  $\| g(x)\| \leq \frac{\epsilon}{2K}$, $\forall x$. while $h(g_k(x), g(x))$ remains the same as the cosine similarity between two vectors are invariant to their norms. Therefore, we have
% % \begin{align}
% %    L_{\text{cncl}}^t = & \sum_{k=1}^K \| g_k(O^t) - g(G^t) \|^2_2 \\
% %     \leq & \sum_{k=1}^K (\| g_k(O^t)\|^2_2 + \| g(G^t) \|^2_2) \\
% %      < &  \sum_{k=1}^K (\frac{\epsilon}{2K}+\frac{\epsilon}{2K}) \\
% %     = & \epsilon
% % \end{align}
% % Therefore, $L_{cncl}^t + L_{dcl}^t < \epsilon + L_{dcl}^t = \epsilon + KlogK - \epsilon = KlogK$, which is valid for all $X^t \in \D$.

% \begin{proposition}
% If there exists a choice of parameters for the feature encoder $g(\cdot)$ and the $K$ transformation networks $\{T_k(g(\cdot))\}_{k=1}^K$ such that $L_\text{cdcl} < K \log K$, then the constant parameter setting $T_k(g(\cdot)) = g(\cdot) = c, \forall c \in \R^d$ is not an optimal solution for minimizing $L_{\text{cdcl}}$.
% \end{proposition}

% \textbf{Proof.} For simplicity, let $g_k(\cdot)$ denote $T_k(g(\cdot))$. First, note that when $g_k(\cdot) = g(\cdot) = c$, the contextual discriminative contrastive loss $L_{\text{cdcl}}$ is given by $K \log K$. Specifically, for an input sample $X^t$, we have:
% \begin{align}
% L^t_{\text{cdcl}} & = L^t_{\text{cncl}} + L^t_{\text{dcl}}\\
% & = K \| c - c \|^2_2-K\log {\frac{c'}{c'+(K-1)c'}} \\
% & = K\log K
% \end{align}
% where $c' = h(c, c)$.

% Assuming that there exists a parameter setting such that $L_{\text{dcl}} < K \log K$, let $\epsilon = K \log K - L_{\text{cdcl}}$. Since the scoring function $h(\cdot, \cdot)$ in $L_{\text{dcl}}$ is defined as $h(g_k(\cdot), g(\cdot)) = \exp(\frac{g_k(\cdot)g(\cdot)}{\tau\|g_k(\cdot)\|_2\|g(\cdot)\|_2})$, we can rescale the functions $\{g_k(\cdot)\}_{k=0}^{K}$ and $g(\cdot)$ during training such that $| g_k(x)| \leq \frac{\epsilon}{2K}$ and $| g(x)| \leq \frac{\epsilon}{2K}$ for all $x$. This rescaling is possible while ensuring that $h(g_k(x), g(x))$ remains the same, since cosine similarity between two vectors is invariant to their norms. Hence, we have:
% \begin{align}
% L_{\text{cncl}}^t = & \sum_{k=1}^K \| g_k(O^t) - g(G^t) \|^2_2 \\
% \leq & \sum_{k=1}^K (\| g_k(O^t)\|^2_2 + \| g(G^t) \|^2_2) \\
% < & \sum_{k=1}^K (\frac{\epsilon}{2K}+\frac{\epsilon}{2K}) =  \epsilon
% \end{align}
% Therefore, we have $L_{\text{cncl}}^t + L_{\text{dcl}}^t < \epsilon + L_{\text{dcl}}^t = \epsilon + K \log K - \epsilon = K \log K$ for all $X^t \in \mathcal{D}$.  \qed


% The intuition for $KlogK$ does not lead to the minimum solution of $L_{\text{dcl}}$ is that the objective of minimizing this loss function is to make sure the generated transformations are diverse among themselves while preserving certain semantic similarities from a given input, which contradicts with the constant encoder solution. This can be easily verified empirically in our experiments. 

% % According to~\cite{qiu2021neural}, $KlogK$ is equivalent to K times the cross entropy of uniform distribution, meaning that neural trnasformation learning is performing no better than random guessing on which category among the K transformations that the input belong to. Meanwhile, the neural transformation loss can be easily achieved below $KlogK$ in our experiments. 



==> subtexes/theoretical_analysis_v2.tex <==
In this section, we delve into an analysis of the representation collapse issue that arises when applying solely the contextual contrastive loss, and why the integration of a discriminative contrastive loss can mitigate this problem. First, we show that a constant feature encoder is an optimal solution for minimizing the contextual contrastive loss in Eq.~\eqref{eq. raw contextual one-class objective}. This suggests that the feature encoder might not extract meaningful semantics from the input data.
\label{sec:theoretical analysis}
\begin{proposition}
 Given the feature encoder $g(\cdot;W)$ in Section~\ref{sec: feature encoder}, there exists a choice of parameters for $W$ such that the output of $g(\cdot;W)$ is always a constant, i.e., $\exists W^*, c^* \ s.t. \ g(x; W^*) = c^*, \forall x$. In this case, $W=W^*$ is an optimal solution for minimizing the loss in Eq.~\eqref{eq. raw contextual one-class objective}.
 \label{props: constant encoder}
\end{proposition}

Proof. Following the work proposed by~\cite{deepSVDD}, there are three settings that can lead to a constant encoder solution: 1. $W=\boldsymbol{0}$; 2. When the encoder is equipped with bias terms in some hidden layers. 3. When the encoder contains bounded activations. In all cases, the loss in Eq.~\eqref{eq. raw contextual one-class objective} reaches the minimum.  \qed

Next, we show that the constant encoders do not lead to the optimal solution of minimizing the contextual discriminative contrastive loss in Eq.~\eqref{eq. contextual discriminative contrastive loss} under certain conditions.

\begin{proposition}
If there exists a choice of parameters for the feature encoder $g(\cdot)$ and the $K$ transformation networks $\{T_k(g(\cdot))\}_{k=1}^K$ such that $L_\text{dcl} < K \log K$, then the constant parameter setting $T_k(g(\cdot)) = g(\cdot) = c, \forall c \in \R^d$ is not an optimal solution for minimizing $L_{\text{cdcl}}$.
\label{props: non-constant encoder}
\end{proposition}

\textbf{Proof.} For simplicity, let $g_k(\cdot)$ denote $T_k(g(\cdot))$. First, note that when $g_k(\cdot) = g(\cdot) = c$, the contextual discriminative contrastive loss $L_{\text{cdcl}}$ is given by $K \log K$. 

Specifically, we have:
\begin{align}
L_{\text{cdcl}} & = L_{\text{cncl}} + L_{\text{dcl}}\\
& = K \| c - c \|^2_2-K\log {\frac{c'}{c'+(K-1)c'}} \\
& = K\log K
\end{align}
where $c' = h(c, c)$. 
Assuming that there exists a parameter setting such that $L_{\text{dcl}} < K \log K$, let $\epsilon = K \log K - L_{\text{cdcl}}$. Since the scoring function $h(\cdot, \cdot)$ in $L_{\text{dcl}}$ is defined as $h(g_k(\cdot), g(\cdot)) = \exp(\frac{g_k(\cdot)^Tg(\cdot)}{\tau\|g_k(\cdot)\|_2\|g(\cdot)\|_2})$, we can rescale the functions $\{g_k(\cdot)\}_{k=1}^{K}$ and $g(\cdot)$ during training such that $\| g_k(x)\|_2 \leq \frac{\epsilon}{2K}$ and $\| g(x)\|_2 \leq \frac{\epsilon}{2K}$ for all $x$. This rescaling is possible while ensuring that $h(g_k(x), g(x))$ remains the same, since cosine similarity between two vectors is invariant to their norms. Hence, we have:
\begin{align}
L_{\text{cncl}} = & \EX_{X^t\sim \D} \left[ \sum_{k=1}^K \| g_k(O^t) - g(G^t) \|^2_2 \right] \\
\leq & \EX_{X^t\sim \D}\left[  \sum_{k=1}^K (\| g_k(O^t)\|^2_2 + \| g(G^t) \|^2_2) \right]\\
< & \sum_{k=1}^K (\frac{\epsilon}{2K}+\frac{\epsilon}{2K}) =  \epsilon
\end{align}
Therefore, we have $L_{\text{cncl}} + L_{\text{dcl}} < \epsilon + L_{\text{dcl}} = \epsilon + K \log K - \epsilon = K \log K$. \qed


The intuition that $K\log K$ does not lead to the minimum solution of $L_{\text{dcl}}$ is that the objective of minimizing this loss function is to make sure that the generated transformations are diverse among themselves while preserving certain semantic similarities from a given input, which contradicts the constant encoder solution. 

% A visual inspection of loss values in \textbf{Section 1.2} of supplementary materials shows that $L_{\text{dcl}}<K \log K$ can be easily reached empirically.







==> subtexes/theoretical_analysis_v3.tex <==
In this section, we delve into a comprehensive analysis of the representation collapse issue that arises when applying solely the contextual contrastive loss, and why the integration of a discriminative contrastive loss can mitigate this problem. First, we show that a constant feature encoder is an optimal solution for minimizing the contextual contrastive loss in Eq.~\eqref{eq. raw contextual one-class objective}.
\label{sec:theoretical analysis}
\begin{proposition}
 Given the feature encoder $g(\cdot;W)$ in Section~\ref{sec: feature encoder}, there exists a choice of parameters for $W$ such that the output of $g(\cdot;W)$ is always a constant, i.e., $\exists W^*, c^* \ s.t. \ g(x; W^*) = c^*, \forall x$. In this case, $W=W^*$ is an optimal solution for minimizing the loss in Eq.~\eqref{eq. raw contextual one-class objective}.
 \label{props: constant encoder}
\end{proposition}
The proof is shown in Section 2 of the supplementary materials. Proposition~\ref{props: constant encoder} implies that the feature encoder may have limited ability to extract meaningful semantics from the input data given that the constant solution can be easily reached. Next, we show that the constant encoders do not lead to the optimal solution of minimizing the contextual discriminative contrastive loss in Eq.~\eqref{eq. contextual discriminative contrastive loss} under certain conditions in Proposition~\ref{props: non-constant encoder}.

\begin{proposition}
If there exists a choice of parameters for the feature encoder $g(\cdot)$ and the $K$ transformation networks $\{T_k(g(\cdot))\}_{k=1}^K$ such that $L_\text{dcl} < K \log K$, then the constant parameter setting $T_k(g(\cdot)) = g(\cdot) = c, \forall c \in \R^d$ is not an optimal solution for minimizing $L_{\text{cdcl}}$.
\label{props: non-constant encoder}
\end{proposition}
The proof is shown in Section 2 of the supplementary materials. The intuition that $K\log K$ does not lead to the minimum solution of $L_{\text{dcl}}$ is that the objective of minimizing this loss function is to make sure that the generated transformations are diverse among themselves while preserving certain semantic similarities from a given input, which contradicts the constant encoder solution. 






